Post-Hoc Reversal: Are We Selecting Models Prematurely?

Trained models are often composed with post-hoc transforms such as temperature scaling (TS), ensembling and stochastic weight averaging (SWA) to improve performance, robustness, uncertainty estimation, etc. However, such transforms are typically applied only after the base models have already been finalized by standard means. In this paper, we challenge this practice with an extensive empirical study. In particular, we demonstrate a phenomenon that we call post-hoc reversal, where performance trends are reversed after applying post-hoc transforms. This phenomenon is especially prominent in high-noise settings. For example, while base models overfit badly early in training, both ensembling and SWA favor base models trained for more epochs. Post-hoc reversal can also prevent the appearance of double descent and mitigate mismatches between test loss and test error seen in base models. Preliminary analyses suggest that these transforms induce reversal by suppressing the influence of mislabeled examples, exploiting differences in their learning dynamics from those of clean examples. Based on our findings, we propose post-hoc selection, a simple technique whereby post-hoc metrics inform model development decisions such as early stopping, checkpointing, and broader hyperparameter choices. Our experiments span real-world vision, language, tabular and graph datasets. On an LLM instruction tuning dataset, post-hoc selection results in >1.5x MMLU improvement compared to naive selection.

==> checklist.tex <==
\section*{NeurIPS Paper Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

% %%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}
    \item[] Justification: The main claims made in the abstract and introduction accurately reflect the paper's contributions and scope.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}
    \item[] Justification: Please see App.~\ref{app:limitations}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \answerNA{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes
    \item[] Justification: Code to reproduce experiments is available at \url{https://anonymous.4open.science/r/post-hoc-reversal}. Comprehensive dataset and training details are provided in App.~\ref{app:datasets}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{}
    \item[] Justification: Please see code (including instructions to download data and reproduce the main results) at \url{https://anonymous.4open.science/r/post-hoc-reversal}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{}
    \item[] Justification: Please see App.~\ref{app:datasets}. In particular, see Tab.~\ref{tab:training} for training details.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: Please see Tabs.~\ref{tab:app_cifar} and \ref{tab:app_real} for detailed results with standard deviations. We don't report error bars for ensembles as it is computationally prohibitive to train many independent ensembles.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: Please see App.~\ref{app:datasets} for training details, including compute resources used.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}
    \item[] Justification: The research conducted in the paper conforms, in every respect, with the NeurIPS Code of Ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{}
    \item[] Justification: We discuss the broader impact of our work in Sec.~\ref{sec:conclusion}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{}
    \item[] Justification: \answerNA{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{}
    \item[] Justification: All datasets and models used in this paper are under permissive licenses allowing for research use. We have credited their authors by exhaustively citing sources.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{}
    \item[] Justification: \answerNA{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{}
    \item[] Justification: \answerNA{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{}
    \item[] Justification: \answerNA{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}


==> dev/literature.tex <==
\section{Literature Review}

\textit{An investigation of why overparameterization exacerbates spurious correlations.}\\
\citebib{sagawa2020investigation}
\begin{itemize}
\item Increasing model size beyond the point of zero training error can hurt the worst-group test error.
\item Subsampling the majority group is better than upweighting the minority in the overparameterized regime.
\item "Overall, our results suggest a tension between using the overparameterized models versus using all the training data for achieving low worst-group error."
\end{itemize}

\subsection{Calibration}

\subsubsection{Foundational Work}

\textit{On calibration of modern neural networks.}\\
\citebib{guo2017calibration}
\begin{itemize}
\item The OG calibration paper for deep learning.
\item Report loss-error non-monotonicity.
\item Temperature scaling.
\end{itemize}

\subsubsection{Applications}

\textit{Scaling vision transformers to 22 billion parameters.}\\
\citebib{dehghani2023scaling}
\begin{itemize}
\item ViT-22B uses temperature scaling.
\item ViT-22B improves trade-off between accuracy and calibration.
\item Conclusions hold both with and without temperature scaling.
\end{itemize}

\subsubsection{LLM Applications}

\textit{Calibrate Before Use: Improving Few-shot Performance of Language Models.}\\
\citebib{zhao2021calibrate}
\begin{itemize}
\item fit calibration parameters for prompting GPT-3
\item "improves accuracy (upto 30\% absolute) across different choices of prompt, and makes learning considerably more stable"
\end{itemize}

\textit{On Calibrating Semantic Segmentation Models: Analyses and an Algorithm.}\\
\citebib{wang2023calibrating}
\begin{itemize}
\item just an application of calibration for semantic segmentation
\end{itemize}


\subsection{Ensembling}

\subsubsection{Negative Results}

\textit{Deep Ensembles Work, But Are They Necessary?}
\citebib{Abe2022DeepEW}
\begin{itemize}
\item the purported benefits of deep ensembles can be replicated by a single larger model
\end{itemize}

\subsubsection{Foundational Work}

\textit{Simple and Scalable Predictive Uncertainty Estimation using Deep Ensembles.}\\
\citebib{Lakshminarayanan2016SimpleAS}
\begin{itemize}
\item earliest citation for \textit{deep} ensembles
\item deep ensembles are better at uncertanty quantification (predictive uncertainty) than Bayesian neural networks
\item ensembling improves calibration.
\end{itemize}

\textit{Can You Trust Your Model's Uncertainty? Evaluating Predictive Uncertainty Under Dataset Shift?}
\citebib{Ovadia2019CanYT}
\begin{itemize}
\item ensembles achieve high accuracy under distribution shift
\end{itemize}

\textit{No One Representation to Rule Them All: Overlapping Features of Training Methods.}\\
\citebib{Lopes2021NoOR}
\begin{itemize}
\item "We find that model pairs that diverge more in training methodology display categorically different generalization behavior, producing increasingly uncorrelated errors."
\item "we find that even significantly low-accuracy models can be used to improve high-accuracy models"
\end{itemize}

\textit{When Ensembling Smaller Models is More Efficient than Single Large Models.}\\
\citebib{kondratyuk2020ensembling}
\begin{itemize}
\item ensemble of smaller models are better than a single large model in a compute-matched comparison
\end{itemize}

\textit{Towards understanding ensemble, knowledge distillation and self-distillation in deep learning.}\\
\citebib{allen2020towards}
\begin{itemize}
\item ICLR 2023 Oral (Top 5\%)
\item "We consider the challenging case where the ensemble is simply an average of the outputs of a few independently trained neural networks with the same architecture, trained using the same algorithm on the same data set, and they only differ by the random seeds used in the initialization."
\item "We show that ensemble/knowledge distillation in deep learning works very differently from traditional learning theory (such as boosting or NTKs, neural tangent kernels)."
\item "The variance due to label noise or the non-convex landscape of training, in the independently- trained models, may not be connected to the superior performance of ensemble in deep learning."
\end{itemize}

\textit{Deep ensembles: A loss landscape perspective.}\\
\citebib{fort2019deep}
\begin{itemize}
\item "Deep ensembles have been empirically shown to be a promising approach for improving accuracy, uncertainty and out-of-distribution robustness of deep learning models."
\item "While deep ensembles were theoretically motivated by the bootstrap, non-bootstrap ensembles trained with just random initialization also perform well in practice"
\item "Our results show that random initializations explore entirely different modes, while functions along an optimization trajectory or sampled from the subspace thereof cluster within a single mode predictions-wise, while often deviating significantly in the weight space."
\item can substantiate discussion of why there is still a gap between SWA and ensemble
\end{itemize}


\textit{Deep Model Fusion: A Survey.}\\
\citebib{li2023deep}
\begin{itemize}
\item useful taxonomy for model fusion: mode-connectivity, alignment, weight average, ensemble learning
\end{itemize}



\subsubsection{Applications}

\textit{Ensembles of data-efficient vision transformers as a new paradigm for automated classification in ecology}
\citebib{kyathanahally2022ensembles}

\textit{Test-time image-to-image translation ensembling improves out-of-distribution generalization in histopathology}
\citebib{scalbert2022test}
\begin{itemize}
\item ensembling improves out-of-distribution generalization
\end{itemize}

\subsubsection{LLM Ensembling}

\textit{Prismer: A vision-language model with an ensemble of experts.}\\
\citebib{liu2023prismer}
\begin{itemize}
\item Leverages an ensemble of independently trained task experts.
\end{itemize}

\textit{Blending Is All You Need: Cheaper, Better Alternative to Trillion-Parameters LLM.}\\
\citebib{lu2024blending}
\begin{itemize}
\item "integrating just three models of moderate size (6B/13B parameters)
can rival or even surpass the performance met- rics of a substantially larger model like Chat- GPT (175B+ parameters)"
\end{itemize}

\textit{LLM-Blender: Ensembling Large Language Models with Pairwise Ranking and Generative Fusion.}\\
\citebib{jiang2023llm}
\begin{itemize}
\item optimal open-source LLMs for different examples can vary
\item propose a method to ensemble LLMs that outperforms all individual LLMs
\end{itemize}

\textit{Routing to the Expert: Efficient Reward-guided Ensemble of Large Language Models.}\\
\citebib{lu2023routing}


\subsection{SWA}

\subsubsection{Foundational Work}

\textit{Averaging weights leads to wider optima and better generalization.}\\
\citebib{izmailov2018averaging}
\begin{itemize}
\item OG SWA paper
\item with negligible additional training \textit{and inference} compute
\end{itemize}

\textit{Loss Surfaces, Mode Connectivity, and Fast Ensembling of DNNs.}\\
\citebib{garipov2018loss}
\begin{itemize}
\item Fast Geometric Ensembling
\item improves upon snapshot ensembles, but still requires xN inference time
\end{itemize}

\textit{Snapshot Ensembles: Train 1, get M for free.}\\
\citebib{huang2017snapshot}
\begin{itemize}
\item pioneered ensembling without additional training cost
\end{itemize}

\textit{Patching open-vocabulary models by interpolating weights.}\\
\citebib{ilharco2022patching}
\begin{itemize}
\item a patching method that uses interpolations between the weights of a model before fine-tuning and the weights after fine-tuning on a task to be patched.
\end{itemize}

\textit{Deep Model Fusion: A Survey.}\\
\citebib{li2023deep}

\textit{Model soups: averaging weights of multiple fine-tuned models improves accuracy without increasing inference time}
\citebib{wortsman2022model}
\begin{itemize}
\item weight-average different fine-tuned models with different hyperparameters
\item improves out-of-distribution and zero-shot performance
\item weight-averaging can recover much of ensembling performance
\end{itemize}

\textit{Diverse weight averaging for out-of-distribution generalization}
\citebib{rame2022diverse}
\begin{itemize}
\item "Diverse Weight Averaging (DiWA), a new WA strategy whose main motivation is to increase the functional diversity across averaged models."
\item "DiWA averages weights obtained from several independent training runs"
\item "this decomposition highlights that WA succeeds when the variance term dominates" (which they show happens when marginal distribution changes at test time, but can we argue that noise in test set has a similar effect?)
\item Improves out-of-distribution generalization (DomainBed)
\end{itemize}

\textit{Swad: Domain generalization by seeking flat minima}
\citebib{cha2021swad}
\begin{itemize}
\item stochastic weight averaging Densely (SWAD)
\item helps with domain generalization / out-of-distribution (DomainBed)
\end{itemize}

\textit{Ensemble of averages: Improving model selection and boosting performance in domain generalization}
\citebib{arpit2022ensemble}
\begin{itemize}
\item ensemble of weight-averaged models helps with domain generalization
\item "we show that instead of ensembling unaveraged models (that is typical in practice), ensembling moving average models (EoA) from independent runs further boosts performance"
\item crucially help reliable early stopping
\end{itemize}

\subsubsection{Applications}

\textit{YOLOv7: Trainable bag-of-freebies sets new state-of-the-art for real-time object detectors.}\\
\citebib{wang2023yolov7}
\begin{itemize}
\item "Re-parameterization techniques involve \textit{averaging a set of model weights} to create a model that is more robust to general patterns that it is trying to model. In research, there has been a recent focus on module level re-parameterization where piece of the network have their own re-parameterization strategies. The YOLOv7 authors use gradient flow propagation paths to see which modules in the network should use re-parameterization strategies and which should not."
\end{itemize}




\subsubsection{SWA for LLMs}

\textit{Early Weight Averaging meets High Learning Rates for LLM Pre-training}
\citebib{sanyal2023early}
\begin{itemize}
\item new training recipe inspired by SWA, which "outperforms conventional training and popular checkpoint averaging baselines such as exponential moving average (EMA) and stochastic moving average (SWA)"
\item on LLM pre-training
\item improves training convergence and generalization
\end{itemize}

\textit{WARM: On the Benefits of Weight Averaged Reward Models}
\citebib{rame2024warm}
\begin{itemize}
\item "Weight Averaged Reward Models (WARM), first fine- tuning multiple RMs, then averaging them in the weight space"
\item "fine-tuned weights remain linearly mode connected when sharing the same pre-training"
\item "WARM improves efficiency compared to the traditional ensembling of predictions"
\item "improving reliability under distribution shifts and robustness to preference inconsistencies"
\item combats reward hacking in RLHF
\end{itemize}

\subsubsection{Why SWA is not used?}

\url{https://discuss.huggingface.co/t/improvements-with-swa/858}
\begin{itemize}
\item HuggingFace discussion on not using SWA for training transformers.
\end{itemize}

\textit{Big Transfer (BiT): General Visual Representation Learning}
\citebib{kolesnikov2020big}
\begin{itemize}
\item makes a conscious choice to not use SWA
\end{itemize}

\textit{ResNet strikes back: An improved training procedure in timm.}\\
\citebib{wightman2021resnet}
\begin{itemize}
\item makes a conscious choice to not use SWA
\end{itemize}



\subsection{Uncertainty Quantification}

\textit{Simple and scalable predictive uncertainty estimation using deep ensembles.}\\
\citebib{lakshminarayanan2017simple}

\textit{A survey of uncertainty in deep neural networks.}\\
\citebib{gawlikowski2021survey}


\textit{A review of uncertainty quantification in deep learning: Techniques, applications and challenges}
\citebib{abdar2021review}
\begin{itemize}
\item covers all 3: calibration, ensembling and SWA
\end{itemize}

\textit{Domain generalization: A survey}
\citebib{zhou2022domain}
\begin{itemize}
\item has both ensemble and SWA but not calibration
\end{itemize}


\subsection{Miscellaneous}

\textit{Finetuned Language Models Are Zero-Shot Learners}
\citebib{Wei2021FinetunedLM}
\begin{itemize}
\item instruction tuning is fine-tuning on instruction datasets, does not involve RLHF
\end{itemize}

\textit{Training language models to follow instructions with human feedback}
\citebib{Ouyang2022TrainingLM}
\begin{itemize}
\item RLHF paper
\item also has an instruction tuning component
\end{itemize}

\textit{Tuning Language Models by Proxy}
\citebib{liu2024tuning}
\begin{itemize}
\item Proxy tuning is a post-hoc transformation
\item The pre-trained LM logits are added to the difference between tuned and untuned proxy logits.
\item Since the proxy expert and anti-expert's logits can be pre-computed, post-hoc selection can feasibly be applied to select the best base LM!
\end{itemize}


\subsection{Motivating multi-epoch training for LLMs}

\textit{Scaling Data-Constrained Language Models}
\citebib{Muennighoff2023ScalingDL}
\begin{itemize}
\item "This work proposes and empirically validate a scaling law for compute optimality that accounts for the decreasing value of repeated tokens and excess parameters and experiment with approaches mitigating data scarcity, including augmenting the training dataset with code data or removing commonly used filters."
\item "Extrapolating this trend suggests that training dataset size may soon be limited by the amount of text data available on the internet."
\item factoring data repetition into scaling laws
\end{itemize}


\textit{To Repeat or Not To Repeat: Insights from Scaling LLM under Token-Crisis}
\citebib{Xue2023ToRO}
\begin{itemize}
\item argues that we will run out of fresh tokens
\item investigates consequences of repeating pre-training data
\item model is susceptible to overfitting, leading to multi-epoch degradation
\item "examine the key factors contributing to multi-epoch degradation, finding that significant factors include dataset size, model parameters, and training objectives, while less influential factors consist of dataset quality and model FLOPs"
\item "we explore whether widely used regularization can alleviate multi-epoch degradation"
\item "Most \textit{regularization techniques do not yield significant improvements}, except for dropout, which demonstrates remarkable effectiveness but requires careful tuning when scaling up the model size."
\end{itemize}


\textit{LIMA: Less Is More for Alignment}
\citebib{zhou2023lima}
\begin{itemize}
\item Show strong alignment performance with only supervised fine-tuning on only 1000 examples, without any Reinforcement Learning!
\item Fine-tune for 15 epochs. But select epoch between 10 and 15 manually.
\item Perplexity rises but Generation quality increases. Similar to loss-error non-monotonicity. (Maybe properly calibrated perplexity would do better?)
\end{itemize}

\textit{AlpaGasus: Training A Better Alpaca with Fewer Data}
\citebib{chen2023alpagasus}
\begin{itemize}
\item data selection strategy to filter SFT dataset
\item only 9k high-quality samples from th 52k Alpaca dataset
\item significantly outperforms alpaca
\item Trains for 10-15 epochs as opposed to 3-5 epochs for Alpaca
\end{itemize}




\subsection{Phenomena}

\textit{Grokking: Generalization Beyond Overfitting on Small Algorithmic Datasets}
\citebib{Power2022GrokkingGB}
\begin{itemize}
\item "generalization of neural networks on small algorithmically generated datasets"
\item "questions about data efficiency, memorization, generalization, and speed of learning can be studied in great detail."
\item "We argue that these datasets provide a fertile ground for studying a poorly understood aspect of deep learning: generalization of overparametrized neural networks beyond memorization of the finite training dataset."
\end{itemize}


\subsection{Noise}

\textit{Benign, Tempered, or Catastrophic: A Taxonomy of Overfitting}
\citebib{Mallinar2022BenignTO}
\begin{itemize}
\item study of \textit{iterpolating methods}, which perfrectly fit their training data
\item overfitting can be \textit{benign} for interpolating classifiers
\item statistical intuition is \textit{catastrophic overfitting}: test performance is no better than random
\item neural networks are in an intermediate regime called \textit{tempered overfitting}
\end{itemize}

\textit{Improving Language Understanding by Generative Pre-Training}
\citebib{Radford2018ImprovingLU}
\begin{itemize}
\item GPT-1 paper
\item using as oldest (modern) citation for next tokne prediction
\end{itemize}

\textit{A Survey on User Behavior Modeling in Recommender Systems}
\citebib{He2023ASO}

\textit{Machine-Learning-Based Disease Diagnosis: A Comprehensive Review}
\citebib{Ahsan2021MachineLearningBasedDD}


==> dev/preamble.tex <==
\PassOptionsToPackage{nonamebreak, round, semicolon, sort}{natbib}
\usepackage[preprint]{neurips_2023}

\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{microtype}

\usepackage{hyperref}

\newcommand{\citebib}[1]{[\texttt{#1}] \citep{#1}}



==> tables/app_cifar_scec.tex <==
\multirow{3}{*}{\makecell[l]{C-10-N\\Clean}}&Naive&&$90$&$_{\pm 9}$&$0.435 _{\pm 0.012}$&$0.234$&$0.201 _{\pm 0.012}$&&$92$&$_{\pm 5}$&$9.75 _{\pm 0.24}$&$8.30$&$1.45 _{\pm 0.24}$\\
&Post-hoc&&$100$ & &$0.433 _{\pm 0.009}$&$0.233$&$0.200 _{\pm 0.009}$&&$96$ & &$9.82 _{\pm 0.27}$&$8.24$&$1.58 _{\pm 0.27}$\\
&$\Delta$&&\textcolor{red!70!black}{$\uparrow 10$}&\textcolor{red!70!black}{$_{\pm 9}$}&\textcolor{green!70!black}{$\downarrow 0.001 _{\pm 0.005}$}&\textcolor{green!70!black}{$\downarrow 0.001$}&--&&\textcolor{red!70!black}{$\uparrow 4$}&\textcolor{red!70!black}{$_{\pm 5}$}&\textcolor{red!70!black}{$\uparrow 0.07 _{\pm 0.10}$}&\textcolor{green!70!black}{$\downarrow 0.06$}&--\\
\midrule
\multirow{3}{*}{\makecell[l]{C-10-N\\Aggre}}&Naive&&$10$&$_{\pm 3}$&$0.722 _{\pm 0.018}$&$0.608$&$0.114 _{\pm 0.018}$&&$94$&$_{\pm 6}$&$19.20 _{\pm 0.39}$&$15.88$&$3.33 _{\pm 0.39}$\\
&Post-hoc&&$53$ & &$0.977 _{\pm 0.030}$&$0.543$&$0.434 _{\pm 0.030}$&&$58$ & &$22.21 _{\pm 0.62}$&$15.74$&$6.47 _{\pm 0.62}$\\
&$\Delta$&&\textcolor{red!70!black}{$\uparrow 43$}&\textcolor{red!70!black}{$_{\pm 3}$}&\textcolor{red!70!black}{$\uparrow 0.255 _{\pm 0.027}$}&\textcolor{green!70!black}{$\downarrow 0.065$}&--&&\textcolor{green!70!black}{$\downarrow 36$}&\textcolor{green!70!black}{$_{\pm 6}$}&\textcolor{red!70!black}{$\uparrow 3.00 _{\pm 0.73}$}&\textcolor{green!70!black}{$\downarrow 0.14$}&--\\
\midrule
\multirow{3}{*}{\makecell[l]{C-10-N\\Rand1}}&Naive&&$8$&$_{\pm 2}$&$1.009 _{\pm 0.008}$&$0.916$&$0.093 _{\pm 0.008}$&&$22$&$_{\pm 32}$&$28.63 _{\pm 0.57}$&$24.80$&$3.83 _{\pm 0.57}$\\
&Post-hoc&&$31$ & &$1.189 _{\pm 0.017}$&$0.859$&$0.330 _{\pm 0.017}$&&$67$ & &$31.58 _{\pm 0.51}$&$23.50$&$8.08 _{\pm 0.51}$\\
&$\Delta$&&\textcolor{red!70!black}{$\uparrow 23$}&\textcolor{red!70!black}{$_{\pm 2}$}&\textcolor{red!70!black}{$\uparrow 0.181 _{\pm 0.018}$}&\textcolor{green!70!black}{$\downarrow 0.057$}&--&&\textcolor{red!70!black}{$\uparrow 44$}&\textcolor{red!70!black}{$_{\pm 32}$}&\textcolor{red!70!black}{$\uparrow 2.95 _{\pm 0.95}$}&\textcolor{green!70!black}{$\downarrow 1.30$}&--\\
\midrule
\multirow{3}{*}{\makecell[l]{C-10-N\\Rand2}}&Naive&&$10$&$_{\pm 1}$&$1.040 _{\pm 0.008}$&$0.931$&$0.108 _{\pm 0.008}$&&$14$&$_{\pm 6}$&$29.90 _{\pm 0.42}$&$25.44$&$4.47 _{\pm 0.42}$\\
&Post-hoc&&$30$ & &$1.189 _{\pm 0.037}$&$0.888$&$0.301 _{\pm 0.037}$&&$74$ & &$31.15 _{\pm 0.38}$&$24.12$&$7.02 _{\pm 0.38}$\\
&$\Delta$&&\textcolor{red!70!black}{$\uparrow 20$}&\textcolor{red!70!black}{$_{\pm 1}$}&\textcolor{red!70!black}{$\uparrow 0.150 _{\pm 0.038}$}&\textcolor{green!70!black}{$\downarrow 0.043$}&--&&\textcolor{red!70!black}{$\uparrow 60$}&\textcolor{red!70!black}{$_{\pm 6}$}&\textcolor{red!70!black}{$\uparrow 1.24 _{\pm 0.56}$}&\textcolor{green!70!black}{$\downarrow 1.32$}&--\\
\midrule
\multirow{3}{*}{\makecell[l]{C-10-N\\Rand3}}&Naive&&$9$&$_{\pm 2}$&$1.005 _{\pm 0.014}$&$0.910$&$0.095 _{\pm 0.014}$&&$24$&$_{\pm 30}$&$28.96 _{\pm 0.65}$&$24.86$&$4.10 _{\pm 0.65}$\\
&Post-hoc&&$32$ & &$1.179 _{\pm 0.027}$&$0.864$&$0.315 _{\pm 0.027}$&&$38$ & &$32.39 _{\pm 0.68}$&$23.44$&$8.95 _{\pm 0.68}$\\
&$\Delta$&&\textcolor{red!70!black}{$\uparrow 23$}&\textcolor{red!70!black}{$_{\pm 2}$}&\textcolor{red!70!black}{$\uparrow 0.174 _{\pm 0.031}$}&\textcolor{green!70!black}{$\downarrow 0.046$}&--&&\textcolor{red!70!black}{$\uparrow 14$}&\textcolor{red!70!black}{$_{\pm 30}$}&\textcolor{red!70!black}{$\uparrow 3.43 _{\pm 1.03}$}&\textcolor{green!70!black}{$\downarrow 1.42$}&--\\
\midrule
\multirow{3}{*}{\makecell[l]{C-10-N\\Worst}}&Naive&&$8$&$_{\pm 2}$&$1.511 _{\pm 0.008}$&$1.437$&$0.073 _{\pm 0.008}$&&$10$&$_{\pm 3}$&$46.84 _{\pm 0.56}$&$44.30$&$2.54 _{\pm 0.56}$\\
&Post-hoc&&$25$ & &$1.643 _{\pm 0.019}$&$1.399$&$0.245 _{\pm 0.019}$&&$24$ & &$49.67 _{\pm 0.74}$&$42.88$&$6.79 _{\pm 0.74}$\\
&$\Delta$&&\textcolor{red!70!black}{$\uparrow 17$}&\textcolor{red!70!black}{$_{\pm 2}$}&\textcolor{red!70!black}{$\uparrow 0.133 _{\pm 0.018}$}&\textcolor{green!70!black}{$\downarrow 0.039$}&--&&\textcolor{red!70!black}{$\uparrow 14$}&\textcolor{red!70!black}{$_{\pm 3}$}&\textcolor{red!70!black}{$\uparrow 2.83 _{\pm 0.94}$}&\textcolor{green!70!black}{$\downarrow 1.42$}&--\\
\midrule
\midrule
\multirow{3}{*}{\makecell[l]{C-100-N-C\\Clean}}&Naive&&$33$&$_{\pm 35}$&$1.011 _{\pm 0.014}$&$0.669$&$0.342 _{\pm 0.014}$&&$91$&$_{\pm 4}$&$23.12 _{\pm 0.40}$&$19.36$&$3.76 _{\pm 0.40}$\\
&Post-hoc&&$100$ & &$1.040 _{\pm 0.019}$&$0.606$&$0.435 _{\pm 0.019}$&&$72$ & &$24.39 _{\pm 0.43}$&$19.52$&$4.87 _{\pm 0.43}$\\
&$\Delta$&&\textcolor{red!70!black}{$\uparrow 67$}&\textcolor{red!70!black}{$_{\pm 35}$}&\textcolor{red!70!black}{$\uparrow 0.029 _{\pm 0.023}$}&\textcolor{green!70!black}{$\downarrow 0.063$}&--&&\textcolor{green!70!black}{$\downarrow 19$}&\textcolor{green!70!black}{$_{\pm 4}$}&\textcolor{red!70!black}{$\uparrow 1.27 _{\pm 0.26}$}&\textcolor{red!70!black}{$\uparrow 0.16$}&--\\
\midrule
\multirow{3}{*}{\makecell[l]{C-100-N-C\\Noisy}}&Naive&&$8$&$_{\pm 2}$&$1.431 _{\pm 0.008}$&$1.234$&$0.198 _{\pm 0.008}$&&$40$&$_{\pm 41}$&$41.42 _{\pm 0.45}$&$34.42$&$7.00 _{\pm 0.45}$\\
&Post-hoc&&$32$ & &$1.744 _{\pm 0.049}$&$1.150$&$0.594 _{\pm 0.049}$&&$38$ & &$45.45 _{\pm 0.98}$&$33.54$&$11.91 _{\pm 0.98}$\\
&$\Delta$&&\textcolor{red!70!black}{$\uparrow 24$}&\textcolor{red!70!black}{$_{\pm 2}$}&\textcolor{red!70!black}{$\uparrow 0.313 _{\pm 0.048}$}&\textcolor{green!70!black}{$\downarrow 0.084$}&--&&\textcolor{green!70!black}{$\downarrow 2$}&\textcolor{green!70!black}{$_{\pm 41}$}&\textcolor{red!70!black}{$\uparrow 4.03 _{\pm 1.13}$}&\textcolor{green!70!black}{$\downarrow 0.88$}&--\\
\midrule
\midrule
\multirow{3}{*}{\makecell[l]{C-100-N-F\\Clean}}&Naive&&$93$&$_{\pm 5}$&$1.508 _{\pm 0.017}$&$1.065$&$0.443 _{\pm 0.017}$&&$88$&$_{\pm 5}$&$33.83 _{\pm 0.37}$&$29.90$&$3.93 _{\pm 0.37}$\\
&Post-hoc&&$75$ & &$1.567 _{\pm 0.019}$&$1.063$&$0.504 _{\pm 0.019}$&&$95$ & &$33.86 _{\pm 0.53}$&$29.94$&$3.92 _{\pm 0.53}$\\
&$\Delta$&&\textcolor{green!70!black}{$\downarrow 18$}&\textcolor{green!70!black}{$_{\pm 5}$}&\textcolor{red!70!black}{$\uparrow 0.059 _{\pm 0.014}$}&\textcolor{green!70!black}{$\downarrow 0.002$}&--&&\textcolor{red!70!black}{$\uparrow 7$}&\textcolor{red!70!black}{$_{\pm 5}$}&\textcolor{red!70!black}{$\uparrow 0.03 _{\pm 0.31}$}&\textcolor{red!70!black}{$\uparrow 0.04$}&--\\
\midrule
\multirow{3}{*}{\makecell[l]{C-100-N-F\\Noisy}}&Naive&&$7$&$_{\pm 2}$&$2.416 _{\pm 0.022}$&$2.129$&$0.287 _{\pm 0.022}$&&$91$&$_{\pm 7}$&$58.68 _{\pm 0.49}$&$51.34$&$7.34 _{\pm 0.49}$\\
&Post-hoc&&$27$ & &$3.015 _{\pm 0.079}$&$1.994$&$1.021 _{\pm 0.079}$&&$32$ & &$63.53 _{\pm 0.55}$&$50.26$&$13.27 _{\pm 0.55}$\\
&$\Delta$&&\textcolor{red!70!black}{$\uparrow 20$}&\textcolor{red!70!black}{$_{\pm 2}$}&\textcolor{red!70!black}{$\uparrow 0.598 _{\pm 0.075}$}&\textcolor{green!70!black}{$\downarrow 0.135$}&--&&\textcolor{green!70!black}{$\downarrow 59$}&\textcolor{green!70!black}{$_{\pm 7}$}&\textcolor{red!70!black}{$\uparrow 4.85 _{\pm 0.60}$}&\textcolor{green!70!black}{$\downarrow 1.08$}&--\\


==> tables/argmin/err.tex <==
\begin{tabular}{llllllll}
\toprule
 & Raw & Cal & WA & WA+Cal & Ens & Ens+Cal & WA+Cal+Ens \\
\midrule
C10 Aggregate & 94 $\pm$ 7 & 92 $\pm$ 8 & 62 $\pm$ 14 & 62 $\pm$ 16 & 45 & 26 & \textbf{63} \\
C10 Clean & 93 $\pm$ 4 & 93 $\pm$ 5 & 92 $\pm$ 5 & 92 $\pm$ 9 & \textbf{85} & 87 & 100 \\
C10 Random1 & 44 $\pm$ 40 & 24 $\pm$ 29 & 45 $\pm$ 20 & 46 $\pm$ 12 & 24 & 20 & \textbf{64} \\
C10 Random2 & 13 $\pm$ 3 & 13 $\pm$ 3 & 55 $\pm$ 11 & 48 $\pm$ 11 & 14 & 14 & \textbf{48} \\
C10 Random3 & 34 $\pm$ 39 & 24 $\pm$ 30 & 48 $\pm$ 15 & 49 $\pm$ 14 & 26 & 26 & \textbf{61} \\
C10 Worst & 11 $\pm$ 2 & 11 $\pm$ 2 & 32 $\pm$ 8 & 32 $\pm$ 6 & 16 & 18 & \textbf{38} \\
C100-C Clean & 92 $\pm$ 7 & 90 $\pm$ 6 & 82 $\pm$ 16 & 83 $\pm$ 14 & 61 & 61 & \textbf{98} \\
C100-C Noisy & 70 $\pm$ 37 & 53 $\pm$ 45 & 44 $\pm$ 11 & 46 $\pm$ 14 & 18 & 19 & \textbf{53} \\
C100-F Clean & 89 $\pm$ 7 & 88 $\pm$ 6 & 91 $\pm$ 13 & 88 $\pm$ 16 & \textbf{93} & 89 & 97 \\
C100-F Noisy & 90 $\pm$ 6 & 51 $\pm$ 45 & 28 $\pm$ 5 & 28 $\pm$ 4 & 20 & 10 & \textbf{40} \\
Employment  & 11 $\pm$ 5 & 8 $\pm$ 4 & 11 $\pm$ 6 & 12 $\pm$ 6 & 13 & 9 & \textbf{15} \\
Income  & 7 $\pm$ 1 & 7 $\pm$ 1 & 10 $\pm$ 1 & 9 $\pm$ 2 & 8 & 9 & \textbf{12} \\
Mobility  & 6 $\pm$ 3 & 7 $\pm$ 3 & 11 $\pm$ 8 & \textbf{9 $\pm$ 5} & 16 & 4 & 19 \\
Public Coverage  & 10 $\pm$ 3 & 9 $\pm$ 3 & 20 $\pm$ 7 & 16 $\pm$ 4 & \textbf{15} & 12 & 29 \\
Travel Time  & 10 $\pm$ 2 & 8 $\pm$ 1 & 15 $\pm$ 3 & 15 $\pm$ 3 & 9 & 8 & \textbf{13} \\
\bottomrule
\end{tabular}


==> tables/argmin/nll.tex <==
\begin{tabular}{llllllll}
\toprule
 & Raw & Cal & WA & WA+Cal & Ens & Ens+Cal & WA+Cal+Ens \\
\midrule
C10 Aggregate & 10 $\pm$ 5 & 64 $\pm$ 41 & 22 $\pm$ 1 & 48 $\pm$ 4 & 18 & 25 & \textbf{55} \\
C10 Clean & 62 $\pm$ 25 & 96 $\pm$ 4 & 48 $\pm$ 4 & 92 $\pm$ 8 & 53 & 62 & \textbf{100} \\
C10 Random1 & 10 $\pm$ 2 & 10 $\pm$ 2 & 19 $\pm$ 1 & 32 $\pm$ 3 & 14 & 15 & \textbf{37} \\
C10 Random2 & 12 $\pm$ 2 & 11 $\pm$ 1 & 19 $\pm$ 2 & 29 $\pm$ 2 & 16 & 16 & \textbf{33} \\
C10 Random3 & 10 $\pm$ 3 & 10 $\pm$ 2 & 19 $\pm$ 1 & 31 $\pm$ 2 & 13 & 13 & \textbf{34} \\
C10 Worst & 9 $\pm$ 3 & 10 $\pm$ 2 & 17 $\pm$ 2 & 24 $\pm$ 3 & 12 & 12 & \textbf{27} \\
C100-C Clean & 11 $\pm$ 4 & 94 $\pm$ 5 & 28 $\pm$ 2 & 69 $\pm$ 6 & 23 & 55 & \textbf{98} \\
C100-C Noisy & 8 $\pm$ 2 & 9 $\pm$ 2 & 20 $\pm$ 1 & 33 $\pm$ 3 & 20 & 13 & \textbf{38} \\
C100-F Clean & 92 $\pm$ 3 & 88 $\pm$ 6 & 24 $\pm$ 1 & 54 $\pm$ 4 & 21 & 55 & \textbf{71} \\
C100-F Noisy & 6 $\pm$ 1 & 8 $\pm$ 2 & 16 $\pm$ 1 & 23 $\pm$ 2 & 10 & 12 & \textbf{32} \\
Employment  & 7 $\pm$ 2 & 7 $\pm$ 2 & 5 $\pm$ 1 & 9 $\pm$ 2 & \textbf{7} & 7 & 9 \\
Income  & 5 $\pm$ 1 & 6 $\pm$ 1 & 8 $\pm$ 1 & 9 $\pm$ 1 & 5 & 6 & \textbf{10} \\
Mobility  & 3 $\pm$ 1 & 4 $\pm$ 1 & 6 $\pm$ 2 & 5 $\pm$ 1 & \textbf{3} & 2 & 4 \\
Public Coverage  & 5 $\pm$ 1 & 6 $\pm$ 2 & 11 $\pm$ 2 & 11 $\pm$ 2 & \textbf{8} & 8 & 11 \\
Travel Time  & 7 $\pm$ 1 & 8 $\pm$ 2 & 12 $\pm$ 1 & 14 $\pm$ 1 & 9 & 9 & \textbf{15} \\
\bottomrule
\end{tabular}


==> tables/experiments/ce_sop_elr/cifar.tex <==
\multirow{3}{*}{\makecell[l]{C-10-N\\Clean}} & CE & $100$ &  & $0.433 _{\pm 0.009}$ & $0.233$ & $96$ &  & $9.82 _{\pm 0.27}$ & $8.24$\\
 & SOP & $100$ &  & $0.430 _{\pm 0.008}$ & $0.235$ & $88$ &  & $9.71 _{\pm 0.20}$ & $8.00$\\
 & ELR & $100$ &  & $0.422 _{\pm 0.012}$ & $0.232$ & $100$ &  & $9.44 _{\pm 0.22}$ & $7.92$\\
\midrule
\multirow{3}{*}{\makecell[l]{C-10-N\\Aggregate}} & CE & $53$ &  & $0.977 _{\pm 0.030}$ & $0.543$ & $58$ &  & $22.21 _{\pm 0.62}$ & $15.74$\\
 & SOP & $94$ &  & $1.084 _{\pm 0.017}$ & $0.541$ & $98$ &  & $17.86 _{\pm 0.23}$ & $15.56$\\
 & ELR & $50$ &  & $0.938 _{\pm 0.031}$ & $0.541$ & $88$ &  & $19.11 _{\pm 0.30}$ & $15.52$\\
\midrule
\multirow{3}{*}{\makecell[l]{C-10-N\\Random1}} & CE & $31$ &  & $1.189 _{\pm 0.017}$ & $0.859$ & $67$ &  & $31.58 _{\pm 0.51}$ & $23.50$\\
 & SOP & $91$ &  & $1.813 _{\pm 0.022}$ & $0.851$ & $87$ &  & $26.89 _{\pm 0.31}$ & $23.14$\\
 & ELR & $31$ &  & $1.175 _{\pm 0.041}$ & $0.864$ & $91$ &  & $29.59 _{\pm 0.46}$ & $23.56$\\
\midrule
\multirow{3}{*}{\makecell[l]{C-10-N\\Random2}} & CE & $30$ &  & $1.189 _{\pm 0.037}$ & $0.888$ & $74$ &  & $31.15 _{\pm 0.38}$ & $24.12$\\
 & SOP & $77$ &  & $1.877 _{\pm 0.029}$ & $0.883$ & $97$ &  & $27.33 _{\pm 0.27}$ & $24.16$\\
 & ELR & $31$ &  & $1.217 _{\pm 0.024}$ & $0.893$ & $54$ &  & $33.34 _{\pm 0.47}$ & $24.50$\\
\midrule
\multirow{3}{*}{\makecell[l]{C-10-N\\Random3}} & CE & $32$ &  & $1.179 _{\pm 0.027}$ & $0.864$ & $38$ &  & $32.39 _{\pm 0.68}$ & $23.44$\\
 & SOP & $98$ &  & $1.787 _{\pm 0.014}$ & $0.851$ & $55$ &  & $29.04 _{\pm 0.68}$ & $22.96$\\
 & ELR & $32$ &  & $1.187 _{\pm 0.038}$ & $0.866$ & $56$ &  & $32.63 _{\pm 0.55}$ & $23.32$\\
\midrule
\multirow{3}{*}{\makecell[l]{C-10-N\\Worst}} & CE & $25$ &  & $1.643 _{\pm 0.019}$ & $1.399$ & $24$ &  & $49.67 _{\pm 0.74}$ & $42.88$\\
 & SOP & $20$ &  & $1.733 _{\pm 0.022}$ & $1.413$ & $39$ &  & $50.48 _{\pm 0.87}$ & $42.78$\\
 & ELR & $26$ &  & $1.685 _{\pm 0.031}$ & $1.397$ & $34$ &  & $51.50 _{\pm 0.63}$ & $42.48$\\
\midrule
\midrule
\multirow{3}{*}{\makecell[l]{C-100-N-C\\Clean}} & CE & $100$ &  & $1.040 _{\pm 0.019}$ & $0.606$ & $72$ &  & $24.39 _{\pm 0.43}$ & $19.52$\\
 & SOP & $100$ &  & $1.039 _{\pm 0.026}$ & $0.608$ & $65$ &  & $25.40 _{\pm 0.66}$ & $19.78$\\
 & ELR & $100$ &  & $1.039 _{\pm 0.011}$ & $0.605$ & $93$ &  & $23.11 _{\pm 0.23}$ & $19.24$\\
\midrule
\multirow{3}{*}{\makecell[l]{C-100-N-C\\Noisy}} & CE & $32$ &  & $1.744 _{\pm 0.049}$ & $1.150$ & $38$ &  & $45.45 _{\pm 0.98}$ & $33.54$\\
 & SOP & $32$ &  & $1.740 _{\pm 0.035}$ & $1.145$ & $28$ &  & $44.31 _{\pm 0.82}$ & $33.94$\\
 & ELR & $32$ &  & $1.794 _{\pm 0.040}$ & $1.152$ & $51$ &  & $44.95 _{\pm 0.69}$ & $33.60$\\
\midrule
\midrule
\multirow{3}{*}{\makecell[l]{C-100-N-F\\Clean}} & CE & $75$ &  & $1.567 _{\pm 0.019}$ & $1.063$ & $95$ &  & $33.86 _{\pm 0.53}$ & $29.94$\\
 & SOP & $71$ &  & $1.597 _{\pm 0.028}$ & $1.061$ & $97$ &  & $33.73 _{\pm 0.37}$ & $29.56$\\
 & ELR & $69$ &  & $1.624 _{\pm 0.013}$ & $1.068$ & $87$ &  & $34.34 _{\pm 0.26}$ & $29.66$\\
\midrule
\multirow{3}{*}{\makecell[l]{C-100-N-F\\Noisy}} & CE & $27$ &  & $3.015 _{\pm 0.079}$ & $1.994$ & $32$ &  & $63.53 _{\pm 0.55}$ & $50.26$\\
 & SOP & $29$ &  & $3.051 _{\pm 0.053}$ & $1.997$ & $31$ &  & $62.72 _{\pm 0.62}$ & $50.54$\\
 & ELR & $25$ &  & $2.903 _{\pm 0.077}$ & $1.997$ & $29$ &  & $63.73 _{\pm 0.82}$ & $50.50$\\
\midrule


==> tables/experiments/model_selection/cifar.tex <==
\multirow{3}{*}{\makecell[l]{C-10-N\\Clean}}&Greedy&&$90$&$_{\pm 9}$&$0.435 _{\pm 0.012}$&$0.234$&$0.201 _{\pm 0.012}$&&$92$&$_{\pm 5}$&$9.75 _{\pm 0.24}$&$8.30$&$1.45 _{\pm 0.24}$\\
&Post-hoc&&$100$ & &$0.433 _{\pm 0.009}$&$0.233$&$0.200 _{\pm 0.009}$&&$96$ & &$9.82 _{\pm 0.27}$&$8.24$&$1.58 _{\pm 0.27}$\\
&$\Delta$&&\textcolor{red!70!black}{$\uparrow 10$}&\textcolor{red!70!black}{$_{\pm 9}$}&\textcolor{green!70!black}{$\downarrow 0.001 _{\pm 0.005}$}&\textcolor{green!70!black}{$\downarrow 0.001$}&--&&\textcolor{red!70!black}{$\uparrow 4$}&\textcolor{red!70!black}{$_{\pm 5}$}&\textcolor{red!70!black}{$\uparrow 0.07 _{\pm 0.10}$}&\textcolor{green!70!black}{$\downarrow 0.06$}&--\\
\midrule
\multirow{3}{*}{\makecell[l]{C-10-N\\Aggregate}}&Greedy&&$10$&$_{\pm 3}$&$0.722 _{\pm 0.018}$&$0.608$&$0.114 _{\pm 0.018}$&&$94$&$_{\pm 6}$&$19.20 _{\pm 0.39}$&$15.88$&$3.33 _{\pm 0.39}$\\
&Post-hoc&&$53$ & &$0.977 _{\pm 0.030}$&$0.543$&$0.434 _{\pm 0.030}$&&$58$ & &$22.21 _{\pm 0.62}$&$15.74$&$6.47 _{\pm 0.62}$\\
&$\Delta$&&\textcolor{red!70!black}{$\uparrow 43$}&\textcolor{red!70!black}{$_{\pm 3}$}&\textcolor{red!70!black}{$\uparrow 0.255 _{\pm 0.027}$}&\textcolor{green!70!black}{$\downarrow 0.065$}&--&&\textcolor{green!70!black}{$\downarrow 36$}&\textcolor{green!70!black}{$_{\pm 6}$}&\textcolor{red!70!black}{$\uparrow 3.00 _{\pm 0.73}$}&\textcolor{green!70!black}{$\downarrow 0.14$}&--\\
\midrule
\multirow{3}{*}{\makecell[l]{C-10-N\\Random1}}&Greedy&&$8$&$_{\pm 2}$&$1.009 _{\pm 0.008}$&$0.916$&$0.093 _{\pm 0.008}$&&$22$&$_{\pm 32}$&$28.63 _{\pm 0.57}$&$24.80$&$3.83 _{\pm 0.57}$\\
&Post-hoc&&$31$ & &$1.189 _{\pm 0.017}$&$0.859$&$0.330 _{\pm 0.017}$&&$67$ & &$31.58 _{\pm 0.51}$&$23.50$&$8.08 _{\pm 0.51}$\\
&$\Delta$&&\textcolor{red!70!black}{$\uparrow 23$}&\textcolor{red!70!black}{$_{\pm 2}$}&\textcolor{red!70!black}{$\uparrow 0.181 _{\pm 0.018}$}&\textcolor{green!70!black}{$\downarrow 0.057$}&--&&\textcolor{red!70!black}{$\uparrow 44$}&\textcolor{red!70!black}{$_{\pm 32}$}&\textcolor{red!70!black}{$\uparrow 2.95 _{\pm 0.95}$}&\textcolor{green!70!black}{$\downarrow 1.30$}&--\\
\midrule
\multirow{3}{*}{\makecell[l]{C-10-N\\Worst}}&Greedy&&$8$&$_{\pm 2}$&$1.511 _{\pm 0.008}$&$1.437$&$0.073 _{\pm 0.008}$&&$10$&$_{\pm 3}$&$46.84 _{\pm 0.56}$&$44.30$&$2.54 _{\pm 0.56}$\\
&Post-hoc&&$25$ & &$1.643 _{\pm 0.019}$&$1.399$&$0.245 _{\pm 0.019}$&&$24$ & &$49.67 _{\pm 0.74}$&$42.88$&$6.79 _{\pm 0.74}$\\
&$\Delta$&&\textcolor{red!70!black}{$\uparrow 17$}&\textcolor{red!70!black}{$_{\pm 2}$}&\textcolor{red!70!black}{$\uparrow 0.133 _{\pm 0.018}$}&\textcolor{green!70!black}{$\downarrow 0.039$}&--&&\textcolor{red!70!black}{$\uparrow 14$}&\textcolor{red!70!black}{$_{\pm 3}$}&\textcolor{red!70!black}{$\uparrow 2.83 _{\pm 0.94}$}&\textcolor{green!70!black}{$\downarrow 1.42$}&--\\
\midrule
\midrule
\multirow{3}{*}{\makecell[l]{C-100-N-F\\Clean}}&Greedy&&$93$&$_{\pm 5}$&$1.508 _{\pm 0.017}$&$1.065$&$0.443 _{\pm 0.017}$&&$88$&$_{\pm 5}$&$33.83 _{\pm 0.37}$&$29.90$&$3.93 _{\pm 0.37}$\\
&Post-hoc&&$75$ & &$1.567 _{\pm 0.019}$&$1.063$&$0.504 _{\pm 0.019}$&&$95$ & &$33.86 _{\pm 0.53}$&$29.94$&$3.92 _{\pm 0.53}$\\
&$\Delta$&&\textcolor{green!70!black}{$\downarrow 18$}&\textcolor{green!70!black}{$_{\pm 5}$}&\textcolor{red!70!black}{$\uparrow 0.059 _{\pm 0.014}$}&\textcolor{green!70!black}{$\downarrow 0.002$}&--&&\textcolor{red!70!black}{$\uparrow 7$}&\textcolor{red!70!black}{$_{\pm 5}$}&\textcolor{red!70!black}{$\uparrow 0.03 _{\pm 0.31}$}&\textcolor{red!70!black}{$\uparrow 0.04$}&--\\
\midrule
\multirow{3}{*}{\makecell[l]{C-100-N-F\\Noisy}}&Greedy&&$7$&$_{\pm 2}$&$2.416 _{\pm 0.022}$&$2.129$&$0.287 _{\pm 0.022}$&&$91$&$_{\pm 7}$&$58.68 _{\pm 0.49}$&$51.34$&$7.34 _{\pm 0.49}$\\
&Post-hoc&&$27$ & &$3.015 _{\pm 0.079}$&$1.994$&$1.021 _{\pm 0.079}$&&$32$ & &$63.53 _{\pm 0.55}$&$50.26$&$13.27 _{\pm 0.55}$\\
&$\Delta$&&\textcolor{red!70!black}{$\uparrow 20$}&\textcolor{red!70!black}{$_{\pm 2}$}&\textcolor{red!70!black}{$\uparrow 0.598 _{\pm 0.075}$}&\textcolor{green!70!black}{$\downarrow 0.135$}&--&&\textcolor{green!70!black}{$\downarrow 59$}&\textcolor{green!70!black}{$_{\pm 7}$}&\textcolor{red!70!black}{$\uparrow 4.85 _{\pm 0.60}$}&\textcolor{green!70!black}{$\downarrow 1.08$}&--\\


==> tables/experiments/model_selection/real.tex <==
\multirow{3}{*}{FMoW}&Greedy&&$2$&$_{\pm 0}$&$1.583 _{\pm 0.014}$&$1.494$&$0.089 _{\pm 0.014}$&&$15$&$_{\pm 19}$&$43.20 _{\pm 0.46}$&$37.95$&$5.24 _{\pm 0.46}$\\
&Post-hoc&&$50$ & &$2.831 _{\pm 0.053}$&$1.305$&$1.526 _{\pm 0.053}$&&$48$ & &$43.18 _{\pm 0.55}$&$34.93$&$8.24 _{\pm 0.55}$\\
&$\Delta$&&\textcolor{red!70!black}{$\uparrow 48$}&\textcolor{red!70!black}{$_{\pm 0}$}&\textcolor{red!70!black}{$\uparrow 1.248 _{\pm 0.062}$}&\textcolor{green!70!black}{$\downarrow 0.189$}&--&&\textcolor{red!70!black}{$\uparrow 33$}&\textcolor{red!70!black}{$_{\pm 19}$}&\textcolor{green!70!black}{$\downarrow 0.02 _{\pm 0.80}$}&\textcolor{green!70!black}{$\downarrow 3.02$}&--\\
\midrule
\multirow{3}{*}{Yelp}&Greedy&&$2$&$_{\pm 1}$&$0.908 _{\pm 0.008}$&$0.841$&$0.067 _{\pm 0.008}$&&$9$&$_{\pm 8}$&$39.41 _{\pm 0.76}$&$36.18$&$3.23 _{\pm 0.76}$\\
&Post-hoc&&$3$ & &$0.990 _{\pm 0.044}$&$0.824$&$0.166 _{\pm 0.044}$&&$3$ & &$40.28 _{\pm 1.29}$&$36.14$&$4.14 _{\pm 1.29}$\\
&$\Delta$&&\textcolor{red!70!black}{$\uparrow 1$}&\textcolor{red!70!black}{$_{\pm 1}$}&\textcolor{red!70!black}{$\uparrow 0.082 _{\pm 0.040}$}&\textcolor{green!70!black}{$\downarrow 0.017$}&--&&\textcolor{green!70!black}{$\downarrow 6$}&\textcolor{green!70!black}{$_{\pm 8}$}&\textcolor{red!70!black}{$\uparrow 0.87 _{\pm 1.16}$}&\textcolor{green!70!black}{$\downarrow 0.04$}&--\\
\midrule
\multirow{3}{*}{Income}&Greedy&&$5$&$_{\pm 1}$&$0.393 _{\pm 0.001}$&$0.388$&$0.005 _{\pm 0.001}$&&$7$&$_{\pm 2}$&$17.84 _{\pm 0.15}$&$17.62$&$0.22 _{\pm 0.15}$\\
&Post-hoc&&$11$ & &$0.421 _{\pm 0.007}$&$0.385$&$0.036 _{\pm 0.007}$&&$19$ & &$19.21 _{\pm 0.14}$&$17.40$&$1.81 _{\pm 0.14}$\\
&$\Delta$&&\textcolor{red!70!black}{$\uparrow 6$}&\textcolor{red!70!black}{$_{\pm 1}$}&\textcolor{red!70!black}{$\uparrow 0.028 _{\pm 0.006}$}&\textcolor{green!70!black}{$\downarrow 0.003$}&--&&\textcolor{red!70!black}{$\uparrow 12$}&\textcolor{red!70!black}{$_{\pm 2}$}&\textcolor{red!70!black}{$\uparrow 1.37 _{\pm 0.22}$}&\textcolor{green!70!black}{$\downarrow 0.22$}&--\\
\midrule
\multirow{3}{*}{\makecell[l]{Public\\Coverage}}&Greedy&&$10$&$_{\pm 2}$&$0.544 _{\pm 0.001}$&$0.538$&$0.006 _{\pm 0.001}$&&$12$&$_{\pm 3}$&$27.52 _{\pm 0.24}$&$27.25$&$0.28 _{\pm 0.24}$\\
&Post-hoc&&$18$ & &$0.554 _{\pm 0.002}$&$0.538$&$0.016 _{\pm 0.002}$&&$22$ & &$27.96 _{\pm 0.21}$&$27.02$&$0.94 _{\pm 0.21}$\\
&$\Delta$&&\textcolor{red!70!black}{$\uparrow 8$}&\textcolor{red!70!black}{$_{\pm 2}$}&\textcolor{red!70!black}{$\uparrow 0.010 _{\pm 0.002}$}&\textcolor{green!70!black}{$\downarrow 0.000$}&--&&\textcolor{red!70!black}{$\uparrow 10$}&\textcolor{red!70!black}{$_{\pm 3}$}&\textcolor{red!70!black}{$\uparrow 0.44 _{\pm 0.25}$}&\textcolor{green!70!black}{$\downarrow 0.22$}&--\\
\midrule
\multirow{3}{*}{\makecell[l]{Travel\\Time}}&Greedy&&$6$&$_{\pm 2}$&$0.597 _{\pm 0.002}$&$0.596$&$0.001 _{\pm 0.002}$&&$9$&$_{\pm 1}$&$35.77 _{\pm 0.34}$&$35.44$&$0.32 _{\pm 0.34}$\\
&Post-hoc&&$15$ & &$0.626 _{\pm 0.003}$&$0.591$&$0.035 _{\pm 0.003}$&&$16$ & &$36.40 _{\pm 0.20}$&$35.23$&$1.17 _{\pm 0.20}$\\
&$\Delta$&&\textcolor{red!70!black}{$\uparrow 8$}&\textcolor{red!70!black}{$_{\pm 2}$}&\textcolor{red!70!black}{$\uparrow 0.029 _{\pm 0.003}$}&\textcolor{green!70!black}{$\downarrow 0.005$}&--&&\textcolor{red!70!black}{$\uparrow 7$}&\textcolor{red!70!black}{$_{\pm 1}$}&\textcolor{red!70!black}{$\uparrow 0.64 _{\pm 0.42}$}&\textcolor{green!70!black}{$\downarrow 0.21$}&--\\
\midrule
\multirow{3}{*}{Collab}&Greedy&&$52$&$_{\pm 18}$&$0.492 _{\pm 0.044}$&$0.439$&$0.053 _{\pm 0.044}$&&$75$&$_{\pm 28}$&$20.65 _{\pm 1.06}$&$20.40$&$0.25 _{\pm 1.06}$\\
&Post-hoc&&$163$ & &$1.075 _{\pm 0.122}$&$0.404$&$0.671 _{\pm 0.122}$&&$152$ & &$20.95 _{\pm 1.26}$&$18.80$&$2.15 _{\pm 1.26}$\\
&$\Delta$&&\textcolor{red!70!black}{$\uparrow 111$}&\textcolor{red!70!black}{$_{\pm 18}$}&\textcolor{red!70!black}{$\uparrow 0.583 _{\pm 0.146}$}&\textcolor{green!70!black}{$\downarrow 0.035$}&--&&\textcolor{red!70!black}{$\uparrow 77$}&\textcolor{red!70!black}{$_{\pm 28}$}&\textcolor{red!70!black}{$\uparrow 0.30 _{\pm 1.31}$}&\textcolor{green!70!black}{$\downarrow 1.60$}&--\\
\midrule
\multirow{3}{*}{Reddit-5k}&Greedy&&$15$&$_{\pm 4}$&$1.154 _{\pm 0.022}$&$1.101$&$0.053 _{\pm 0.022}$&&$13$&$_{\pm 5}$&$47.42 _{\pm 0.64}$&$47.09$&$0.33 _{\pm 0.64}$\\
&Post-hoc&&$44$ & &$1.448 _{\pm 0.058}$&$1.085$&$0.362 _{\pm 0.058}$&&$45$ & &$50.75 _{\pm 1.83}$&$45.49$&$5.26 _{\pm 1.83}$\\
&$\Delta$&&\textcolor{red!70!black}{$\uparrow 29$}&\textcolor{red!70!black}{$_{\pm 4}$}&\textcolor{red!70!black}{$\uparrow 0.294 _{\pm 0.059}$}&\textcolor{green!70!black}{$\downarrow 0.015$}&--&&\textcolor{red!70!black}{$\uparrow 32$}&\textcolor{red!70!black}{$_{\pm 5}$}&\textcolor{red!70!black}{$\uparrow 3.33 _{\pm 2.05}$}&\textcolor{green!70!black}{$\downarrow 1.60$}&--\\
\midrule
\multirow{3}{*}{Reddit-12k}&Greedy&&$16$&$_{\pm 3}$&$1.405 _{\pm 0.011}$&$1.367$&$0.038 _{\pm 0.011}$&&$17$&$_{\pm 4}$&$51.78 _{\pm 1.05}$&$50.34$&$1.45 _{\pm 1.05}$\\
&Post-hoc&&$41$ & &$1.585 _{\pm 0.023}$&$1.346$&$0.239 _{\pm 0.023}$&&$64$ & &$55.85 _{\pm 0.97}$&$51.26$&$4.59 _{\pm 0.97}$\\
&$\Delta$&&\textcolor{red!70!black}{$\uparrow 25$}&\textcolor{red!70!black}{$_{\pm 3}$}&\textcolor{red!70!black}{$\uparrow 0.180 _{\pm 0.027}$}&\textcolor{green!70!black}{$\downarrow 0.021$}&--&&\textcolor{red!70!black}{$\uparrow 47$}&\textcolor{red!70!black}{$_{\pm 4}$}&\textcolor{red!70!black}{$\uparrow 4.07 _{\pm 1.59}$}&\textcolor{red!70!black}{$\uparrow 0.92$}&--\\


==> tables/extra/argmin/err.tex <==
\begin{tabular}{llllllll}
\toprule
 & Raw & Cal & WA & WA+Cal & Ens & Ens+Cal & WA+Cal+Ens \\
\midrule
C10 Aggregate & 94 $\pm$ 7 & 92 $\pm$ 8 & 62 $\pm$ 14 & 62 $\pm$ 16 & 45 & 26 & \textbf{63} \\
C10 Clean & 93 $\pm$ 4 & 93 $\pm$ 5 & 92 $\pm$ 5 & 92 $\pm$ 9 & \textbf{85} & 87 & 100 \\
C10 Random1 & 44 $\pm$ 40 & 24 $\pm$ 29 & 45 $\pm$ 20 & 46 $\pm$ 12 & 24 & 20 & \textbf{64} \\
C10 Random2 & 13 $\pm$ 3 & 13 $\pm$ 3 & 55 $\pm$ 11 & 48 $\pm$ 11 & 14 & 14 & \textbf{48} \\
C10 Random3 & 34 $\pm$ 39 & 24 $\pm$ 30 & 48 $\pm$ 15 & 49 $\pm$ 14 & 26 & 26 & \textbf{61} \\
C10 Worst & 11 $\pm$ 2 & 11 $\pm$ 2 & 32 $\pm$ 8 & 32 $\pm$ 6 & 16 & 18 & \textbf{38} \\
C100-C Clean & 92 $\pm$ 7 & 90 $\pm$ 6 & 82 $\pm$ 16 & 83 $\pm$ 14 & 61 & 61 & \textbf{98} \\
C100-C Noisy & 70 $\pm$ 37 & 53 $\pm$ 45 & 44 $\pm$ 11 & 46 $\pm$ 14 & 18 & 19 & \textbf{53} \\
C100-F Clean & 89 $\pm$ 7 & 88 $\pm$ 6 & 91 $\pm$ 13 & 88 $\pm$ 16 & \textbf{93} & 89 & 97 \\
C100-F Noisy & 90 $\pm$ 6 & 51 $\pm$ 45 & 28 $\pm$ 5 & 28 $\pm$ 4 & 20 & 10 & \textbf{40} \\
Employment  & 11 $\pm$ 5 & 8 $\pm$ 4 & 11 $\pm$ 6 & 12 $\pm$ 6 & 13 & 9 & \textbf{15} \\
Income  & 7 $\pm$ 1 & 7 $\pm$ 1 & 10 $\pm$ 1 & 9 $\pm$ 2 & 8 & 9 & \textbf{12} \\
Mobility  & 6 $\pm$ 3 & 7 $\pm$ 3 & 11 $\pm$ 8 & \textbf{9 $\pm$ 5} & 16 & 4 & 19 \\
Public Coverage  & 10 $\pm$ 3 & 9 $\pm$ 3 & 20 $\pm$ 7 & 16 $\pm$ 4 & \textbf{15} & 12 & 29 \\
Travel Time  & 10 $\pm$ 2 & 8 $\pm$ 1 & 15 $\pm$ 3 & 15 $\pm$ 3 & 9 & 8 & \textbf{13} \\
\bottomrule
\end{tabular}


==> tables/extra/argmin/nll.tex <==
\begin{tabular}{llllllll}
\toprule
 & Raw & Cal & WA & WA+Cal & Ens & Ens+Cal & WA+Cal+Ens \\
\midrule
C10 Aggregate & 10 $\pm$ 5 & 64 $\pm$ 41 & 22 $\pm$ 1 & 48 $\pm$ 4 & 18 & 25 & \textbf{55} \\
C10 Clean & 62 $\pm$ 25 & 96 $\pm$ 4 & 48 $\pm$ 4 & 92 $\pm$ 8 & 53 & 62 & \textbf{100} \\
C10 Random1 & 10 $\pm$ 2 & 10 $\pm$ 2 & 19 $\pm$ 1 & 32 $\pm$ 3 & 14 & 15 & \textbf{37} \\
C10 Random2 & 12 $\pm$ 2 & 11 $\pm$ 1 & 19 $\pm$ 2 & 29 $\pm$ 2 & 16 & 16 & \textbf{33} \\
C10 Random3 & 10 $\pm$ 3 & 10 $\pm$ 2 & 19 $\pm$ 1 & 31 $\pm$ 2 & 13 & 13 & \textbf{34} \\
C10 Worst & 9 $\pm$ 3 & 10 $\pm$ 2 & 17 $\pm$ 2 & 24 $\pm$ 3 & 12 & 12 & \textbf{27} \\
C100-C Clean & 11 $\pm$ 4 & 94 $\pm$ 5 & 28 $\pm$ 2 & 69 $\pm$ 6 & 23 & 55 & \textbf{98} \\
C100-C Noisy & 8 $\pm$ 2 & 9 $\pm$ 2 & 20 $\pm$ 1 & 33 $\pm$ 3 & 20 & 13 & \textbf{38} \\
C100-F Clean & 92 $\pm$ 3 & 88 $\pm$ 6 & 24 $\pm$ 1 & 54 $\pm$ 4 & 21 & 55 & \textbf{71} \\
C100-F Noisy & 6 $\pm$ 1 & 8 $\pm$ 2 & 16 $\pm$ 1 & 23 $\pm$ 2 & 10 & 12 & \textbf{32} \\
Employment  & 7 $\pm$ 2 & 7 $\pm$ 2 & 5 $\pm$ 1 & 9 $\pm$ 2 & \textbf{7} & 7 & 9 \\
Income  & 5 $\pm$ 1 & 6 $\pm$ 1 & 8 $\pm$ 1 & 9 $\pm$ 1 & 5 & 6 & \textbf{10} \\
Mobility  & 3 $\pm$ 1 & 4 $\pm$ 1 & 6 $\pm$ 2 & 5 $\pm$ 1 & \textbf{3} & 2 & 4 \\
Public Coverage  & 5 $\pm$ 1 & 6 $\pm$ 2 & 11 $\pm$ 2 & 11 $\pm$ 2 & \textbf{8} & 8 & 11 \\
Travel Time  & 7 $\pm$ 1 & 8 $\pm$ 2 & 12 $\pm$ 1 & 14 $\pm$ 1 & 9 & 9 & \textbf{15} \\
\bottomrule
\end{tabular}


==> tables/extra/dataset_details.tex <==
\begin{tabular}{llS[table-format=5]S[table-format=5]S[table-format=5]S[table-format=3]rc}
\toprule
Modality & Dataset & {Train Size} & {Val Size} & {Test Size} & {Classes} & Input Size & Units\\
\midrule
\multirow{4}{*}{Vision} & CIFAR-10 & 40000 & 5000 & 5000 & 10 & \numproduct{3x32x32} & \multirow{4}{*}{C $\times$ W $\times$ H}\\
 & CIFAR-100-N Coarse & 40000 & 5000 & 5000 & 20 & \numproduct{3x32x32} & \\
 & CIFAR-100-N Fine & 40000 & 5000 & 5000 & 100 & \numproduct{3x32x32} & \\
 & FMoW & 76863 & 11483 & 11327 & 62 & \numproduct{3x224x224} & \\
\midrule
\multirow{3}{*}{Graph} & Collab & 4000 & 500 & 500 & 3 & \num{74.49} / \num{2457.78} & \multirow{3}{*}{\makecell{nodes / edges \\ (avg.)}}\\
 & Reddit-5k & 4001 & 499 & 499 & 5 & \num{508.52} / \num{594.87} & \\
 & Reddit-12k & 9545 & 1192 & 1192 & 11 & \num{391.41} / \num{456.89} & \\
\midrule
\multirow{5}{*}{Tabular} & Income & 156533 & 19566 & 19566 & 2 & \num{816} & \multirow{5}{*}{features}\\
 & Public Coverage & 110844 & 13855 & 13855 & 2 & \num{88} & \\
 & Mobility & 64265 & 8032 & 8032 & 2 & \num{101} & \\
 & Employment & 303055 & 37881 & 37881 & 2 & \num{98} & \\
 & Travel Time & 138008 & 17250 & 17250 & 2 & \num{615} & \\
\bottomrule
\end{tabular}

==> tables/extra/main.tex <==
\multirow{3}{*}{\makecell[l]{C-10-N\\Clean}} & Naive & $90$ & $_{\pm 9}$ & $0.435 _{\pm 0.012}$ & $0.234$ & \textcolor{green!70!black}{$-$ $0.201 _{\pm 0.012}$} & $92$ & $_{\pm 5}$ & $9.75 _{\pm 0.24}$ & $8.30$ & \textcolor{green!70!black}{$-$ $1.45 _{\pm 0.24}$}\\
 & Post-hoc & $100$ &  & $0.433 _{\pm 0.009}$ & $0.233$ & \textcolor{green!70!black}{$-$ $0.200 _{\pm 0.009}$} & $96$ &  & $9.82 _{\pm 0.27}$ & $8.24$ & \textcolor{green!70!black}{$-$ $1.58 _{\pm 0.27}$}\\
 & $\Delta$ & $+$ $10$ & $_{\pm 9}$ & \textcolor{green!70!black}{$-$ $0.001 _{\pm 0.005}$} & \textcolor{green!70!black}{$-$ $0.001$} &  & $+$ $4$ & $_{\pm 5}$ & \textcolor{red!70!black}{$+$ $0.07 _{\pm 0.10}$} & \textcolor{green!70!black}{$-$ $0.06$} & \\
\midrule
\multirow{3}{*}{\makecell[l]{C-10-N\\Aggregate}} & Naive & $10$ & $_{\pm 3}$ & $0.722 _{\pm 0.018}$ & $0.608$ & \textcolor{green!70!black}{$-$ $0.114 _{\pm 0.018}$} & $94$ & $_{\pm 6}$ & $19.20 _{\pm 0.39}$ & $15.88$ & \textcolor{green!70!black}{$-$ $3.33 _{\pm 0.39}$}\\
 & Post-hoc & $53$ &  & $0.977 _{\pm 0.030}$ & $0.543$ & \textcolor{green!70!black}{$-$ $0.434 _{\pm 0.030}$} & $58$ &  & $22.21 _{\pm 0.62}$ & $15.74$ & \textcolor{green!70!black}{$-$ $6.47 _{\pm 0.62}$}\\
 & $\Delta$ & $+$ $43$ & $_{\pm 3}$ & \textcolor{red!70!black}{$+$ $0.255 _{\pm 0.027}$} & \textcolor{green!70!black}{$-$ $0.065$} &  & $-$ $36$ & $_{\pm 6}$ & \textcolor{red!70!black}{$+$ $3.00 _{\pm 0.73}$} & \textcolor{green!70!black}{$-$ $0.14$} & \\
\midrule
\multirow{3}{*}{\makecell[l]{C-10-N\\Random1}} & Naive & $8$ & $_{\pm 2}$ & $1.009 _{\pm 0.008}$ & $0.916$ & \textcolor{green!70!black}{$-$ $0.093 _{\pm 0.008}$} & $22$ & $_{\pm 32}$ & $28.63 _{\pm 0.57}$ & $24.80$ & \textcolor{green!70!black}{$-$ $3.83 _{\pm 0.57}$}\\
 & Post-hoc & $31$ &  & $1.189 _{\pm 0.017}$ & $0.859$ & \textcolor{green!70!black}{$-$ $0.330 _{\pm 0.017}$} & $67$ &  & $31.58 _{\pm 0.51}$ & $23.50$ & \textcolor{green!70!black}{$-$ $8.08 _{\pm 0.51}$}\\
 & $\Delta$ & $+$ $23$ & $_{\pm 2}$ & \textcolor{red!70!black}{$+$ $0.181 _{\pm 0.018}$} & \textcolor{green!70!black}{$-$ $0.057$} &  & $+$ $44$ & $_{\pm 32}$ & \textcolor{red!70!black}{$+$ $2.95 _{\pm 0.95}$} & \textcolor{green!70!black}{$-$ $1.30$} & \\
\midrule
\multirow{3}{*}{\makecell[l]{C-10-N\\Random2}} & Naive & $10$ & $_{\pm 1}$ & $1.040 _{\pm 0.008}$ & $0.931$ & \textcolor{green!70!black}{$-$ $0.108 _{\pm 0.008}$} & $14$ & $_{\pm 6}$ & $29.90 _{\pm 0.42}$ & $25.44$ & \textcolor{green!70!black}{$-$ $4.47 _{\pm 0.42}$}\\
 & Post-hoc & $30$ &  & $1.189 _{\pm 0.037}$ & $0.888$ & \textcolor{green!70!black}{$-$ $0.301 _{\pm 0.037}$} & $74$ &  & $31.15 _{\pm 0.38}$ & $24.12$ & \textcolor{green!70!black}{$-$ $7.02 _{\pm 0.38}$}\\
 & $\Delta$ & $+$ $20$ & $_{\pm 1}$ & \textcolor{red!70!black}{$+$ $0.150 _{\pm 0.038}$} & \textcolor{green!70!black}{$-$ $0.043$} &  & $+$ $60$ & $_{\pm 6}$ & \textcolor{red!70!black}{$+$ $1.24 _{\pm 0.56}$} & \textcolor{green!70!black}{$-$ $1.32$} & \\
\midrule
\multirow{3}{*}{\makecell[l]{C-10-N\\Random3}} & Naive & $9$ & $_{\pm 2}$ & $1.005 _{\pm 0.014}$ & $0.910$ & \textcolor{green!70!black}{$-$ $0.095 _{\pm 0.014}$} & $24$ & $_{\pm 30}$ & $28.96 _{\pm 0.65}$ & $24.86$ & \textcolor{green!70!black}{$-$ $4.10 _{\pm 0.65}$}\\
 & Post-hoc & $32$ &  & $1.179 _{\pm 0.027}$ & $0.864$ & \textcolor{green!70!black}{$-$ $0.315 _{\pm 0.027}$} & $38$ &  & $32.39 _{\pm 0.68}$ & $23.44$ & \textcolor{green!70!black}{$-$ $8.95 _{\pm 0.68}$}\\
 & $\Delta$ & $+$ $23$ & $_{\pm 2}$ & \textcolor{red!70!black}{$+$ $0.174 _{\pm 0.031}$} & \textcolor{green!70!black}{$-$ $0.046$} &  & $+$ $14$ & $_{\pm 30}$ & \textcolor{red!70!black}{$+$ $3.43 _{\pm 1.03}$} & \textcolor{green!70!black}{$-$ $1.42$} & \\
\midrule
\multirow{3}{*}{\makecell[l]{C-10-N\\Worst}} & Naive & $8$ & $_{\pm 2}$ & $1.511 _{\pm 0.008}$ & $1.437$ & \textcolor{green!70!black}{$-$ $0.073 _{\pm 0.008}$} & $10$ & $_{\pm 3}$ & $46.84 _{\pm 0.56}$ & $44.30$ & \textcolor{green!70!black}{$-$ $2.54 _{\pm 0.56}$}\\
 & Post-hoc & $25$ &  & $1.643 _{\pm 0.019}$ & $1.399$ & \textcolor{green!70!black}{$-$ $0.245 _{\pm 0.019}$} & $24$ &  & $49.67 _{\pm 0.74}$ & $42.88$ & \textcolor{green!70!black}{$-$ $6.79 _{\pm 0.74}$}\\
 & $\Delta$ & $+$ $17$ & $_{\pm 2}$ & \textcolor{red!70!black}{$+$ $0.133 _{\pm 0.018}$} & \textcolor{green!70!black}{$-$ $0.039$} &  & $+$ $14$ & $_{\pm 3}$ & \textcolor{red!70!black}{$+$ $2.83 _{\pm 0.94}$} & \textcolor{green!70!black}{$-$ $1.42$} & \\
\midrule
\midrule
\multirow{3}{*}{\makecell[l]{C-100-N-C\\Clean}} & Naive & $33$ & $_{\pm 35}$ & $1.011 _{\pm 0.014}$ & $0.669$ & \textcolor{green!70!black}{$-$ $0.342 _{\pm 0.014}$} & $91$ & $_{\pm 4}$ & $23.12 _{\pm 0.40}$ & $19.36$ & \textcolor{green!70!black}{$-$ $3.76 _{\pm 0.40}$}\\
 & Post-hoc & $100$ &  & $1.040 _{\pm 0.019}$ & $0.606$ & \textcolor{green!70!black}{$-$ $0.435 _{\pm 0.019}$} & $72$ &  & $24.39 _{\pm 0.43}$ & $19.52$ & \textcolor{green!70!black}{$-$ $4.87 _{\pm 0.43}$}\\
 & $\Delta$ & $+$ $67$ & $_{\pm 35}$ & \textcolor{red!70!black}{$+$ $0.029 _{\pm 0.023}$} & \textcolor{green!70!black}{$-$ $0.063$} &  & $-$ $19$ & $_{\pm 4}$ & \textcolor{red!70!black}{$+$ $1.27 _{\pm 0.26}$} & \textcolor{red!70!black}{$+$ $0.16$} & \\
\midrule
\multirow{3}{*}{\makecell[l]{C-100-N-C\\Noisy}} & Naive & $8$ & $_{\pm 2}$ & $1.431 _{\pm 0.008}$ & $1.234$ & \textcolor{green!70!black}{$-$ $0.198 _{\pm 0.008}$} & $40$ & $_{\pm 41}$ & $41.42 _{\pm 0.45}$ & $34.42$ & \textcolor{green!70!black}{$-$ $7.00 _{\pm 0.45}$}\\
 & Post-hoc & $32$ &  & $1.744 _{\pm 0.049}$ & $1.150$ & \textcolor{green!70!black}{$-$ $0.594 _{\pm 0.049}$} & $38$ &  & $45.45 _{\pm 0.98}$ & $33.54$ & \textcolor{green!70!black}{$-$ $11.91 _{\pm 0.98}$}\\
 & $\Delta$ & $+$ $24$ & $_{\pm 2}$ & \textcolor{red!70!black}{$+$ $0.313 _{\pm 0.048}$} & \textcolor{green!70!black}{$-$ $0.084$} &  & $-$ $2$ & $_{\pm 41}$ & \textcolor{red!70!black}{$+$ $4.03 _{\pm 1.13}$} & \textcolor{green!70!black}{$-$ $0.88$} & \\
\midrule
\midrule
\multirow{3}{*}{\makecell[l]{C-100-N-F\\Clean}} & Naive & $93$ & $_{\pm 5}$ & $1.508 _{\pm 0.017}$ & $1.065$ & \textcolor{green!70!black}{$-$ $0.443 _{\pm 0.017}$} & $88$ & $_{\pm 5}$ & $33.83 _{\pm 0.37}$ & $29.90$ & \textcolor{green!70!black}{$-$ $3.93 _{\pm 0.37}$}\\
 & Post-hoc & $75$ &  & $1.567 _{\pm 0.019}$ & $1.063$ & \textcolor{green!70!black}{$-$ $0.504 _{\pm 0.019}$} & $95$ &  & $33.86 _{\pm 0.53}$ & $29.94$ & \textcolor{green!70!black}{$-$ $3.92 _{\pm 0.53}$}\\
 & $\Delta$ & $-$ $18$ & $_{\pm 5}$ & \textcolor{red!70!black}{$+$ $0.059 _{\pm 0.014}$} & \textcolor{green!70!black}{$-$ $0.002$} &  & $+$ $7$ & $_{\pm 5}$ & \textcolor{red!70!black}{$+$ $0.03 _{\pm 0.31}$} & \textcolor{red!70!black}{$+$ $0.04$} & \\
\midrule
\multirow{3}{*}{\makecell[l]{C-100-N-F\\Noisy}} & Naive & $7$ & $_{\pm 2}$ & $2.416 _{\pm 0.022}$ & $2.129$ & \textcolor{green!70!black}{$-$ $0.287 _{\pm 0.022}$} & $91$ & $_{\pm 7}$ & $58.68 _{\pm 0.49}$ & $51.34$ & \textcolor{green!70!black}{$-$ $7.34 _{\pm 0.49}$}\\
 & Post-hoc & $27$ &  & $3.015 _{\pm 0.079}$ & $1.994$ & \textcolor{green!70!black}{$-$ $1.021 _{\pm 0.079}$} & $32$ &  & $63.53 _{\pm 0.55}$ & $50.26$ & \textcolor{green!70!black}{$-$ $13.27 _{\pm 0.55}$}\\
 & $\Delta$ & $+$ $20$ & $_{\pm 2}$ & \textcolor{red!70!black}{$+$ $0.598 _{\pm 0.075}$} & \textcolor{green!70!black}{$-$ $0.135$} &  & $-$ $59$ & $_{\pm 7}$ & \textcolor{red!70!black}{$+$ $4.85 _{\pm 0.60}$} & \textcolor{green!70!black}{$-$ $1.08$} & \\
\midrule
\midrule
\multirow{3}{*}{Income} & Naive & $5$ & $_{\pm 1}$ & $0.393 _{\pm 0.001}$ & $0.388$ & \textcolor{green!70!black}{$-$ $0.005 _{\pm 0.001}$} & $7$ & $_{\pm 2}$ & $17.84 _{\pm 0.15}$ & $17.62$ & \textcolor{green!70!black}{$-$ $0.22 _{\pm 0.15}$}\\
 & Post-hoc & $11$ &  & $0.421 _{\pm 0.007}$ & $0.385$ & \textcolor{green!70!black}{$-$ $0.036 _{\pm 0.007}$} & $19$ &  & $19.21 _{\pm 0.14}$ & $17.40$ & \textcolor{green!70!black}{$-$ $1.81 _{\pm 0.14}$}\\
 & $\Delta$ & $+$ $6$ & $_{\pm 1}$ & \textcolor{red!70!black}{$+$ $0.028 _{\pm 0.006}$} & \textcolor{green!70!black}{$-$ $0.003$} &  & $+$ $12$ & $_{\pm 2}$ & \textcolor{red!70!black}{$+$ $1.37 _{\pm 0.22}$} & \textcolor{green!70!black}{$-$ $0.22$} & \\
\midrule
\multirow{3}{*}{\makecell[l]{Public\\Coverage}} & Naive & $10$ & $_{\pm 2}$ & $0.544 _{\pm 0.001}$ & $0.538$ & \textcolor{green!70!black}{$-$ $0.006 _{\pm 0.001}$} & $12$ & $_{\pm 3}$ & $27.52 _{\pm 0.24}$ & $27.25$ & \textcolor{green!70!black}{$-$ $0.28 _{\pm 0.24}$}\\
 & Post-hoc & $18$ &  & $0.554 _{\pm 0.002}$ & $0.538$ & \textcolor{green!70!black}{$-$ $0.016 _{\pm 0.002}$} & $22$ &  & $27.96 _{\pm 0.21}$ & $27.02$ & \textcolor{green!70!black}{$-$ $0.94 _{\pm 0.21}$}\\
 & $\Delta$ & $+$ $8$ & $_{\pm 2}$ & \textcolor{red!70!black}{$+$ $0.010 _{\pm 0.002}$} & \textcolor{green!70!black}{$-$ $0.000$} &  & $+$ $10$ & $_{\pm 3}$ & \textcolor{red!70!black}{$+$ $0.44 _{\pm 0.25}$} & \textcolor{green!70!black}{$-$ $0.22$} & \\
\midrule
\multirow{3}{*}{Mobility} & Naive & $6$ & $_{\pm 2}$ & $0.474 _{\pm 0.002}$ & $0.471$ & \textcolor{green!70!black}{$-$ $0.003 _{\pm 0.002}$} & $13$ & $_{\pm 5}$ & $21.43 _{\pm 0.18}$ & $21.17$ & \textcolor{green!70!black}{$-$ $0.26 _{\pm 0.18}$}\\
 & Post-hoc & $14$ &  & $0.476 _{\pm 0.003}$ & $0.468$ & \textcolor{green!70!black}{$-$ $0.008 _{\pm 0.003}$} & $11$ &  & $21.40 _{\pm 0.17}$ & $21.24$ & \textcolor{green!70!black}{$-$ $0.16 _{\pm 0.17}$}\\
 & $\Delta$ & $+$ $8$ & $_{\pm 2}$ & \textcolor{red!70!black}{$+$ $0.002 _{\pm 0.003}$} & \textcolor{green!70!black}{$-$ $0.003$} &  & $-$ $2$ & $_{\pm 5}$ & \textcolor{green!70!black}{$-$ $0.03 _{\pm 0.22}$} & \textcolor{red!70!black}{$+$ $0.07$} & \\
\midrule
\multirow{3}{*}{Employment} & Naive & $8$ & $_{\pm 1}$ & $0.380 _{\pm 0.000}$ & $0.378$ & \textcolor{green!70!black}{$-$ $0.003 _{\pm 0.000}$} & $14$ & $_{\pm 4}$ & $17.94 _{\pm 0.08}$ & $17.72$ & \textcolor{green!70!black}{$-$ $0.22 _{\pm 0.08}$}\\
 & Post-hoc & $15$ &  & $0.383 _{\pm 0.001}$ & $0.377$ & \textcolor{green!70!black}{$-$ $0.006 _{\pm 0.001}$} & $30$ &  & $18.27 _{\pm 0.12}$ & $17.83$ & \textcolor{green!70!black}{$-$ $0.43 _{\pm 0.12}$}\\
 & $\Delta$ & $+$ $7$ & $_{\pm 1}$ & \textcolor{red!70!black}{$+$ $0.003 _{\pm 0.001}$} & \textcolor{green!70!black}{$-$ $0.000$} &  & $+$ $16$ & $_{\pm 4}$ & \textcolor{red!70!black}{$+$ $0.33 _{\pm 0.16}$} & \textcolor{red!70!black}{$+$ $0.11$} & \\
\midrule
\multirow{3}{*}{Travel Time} & Naive & $6$ & $_{\pm 2}$ & $0.597 _{\pm 0.002}$ & $0.596$ & \textcolor{green!70!black}{$-$ $0.001 _{\pm 0.002}$} & $9$ & $_{\pm 1}$ & $35.77 _{\pm 0.34}$ & $35.44$ & \textcolor{green!70!black}{$-$ $0.32 _{\pm 0.34}$}\\
 & Post-hoc & $15$ &  & $0.626 _{\pm 0.003}$ & $0.591$ & \textcolor{green!70!black}{$-$ $0.035 _{\pm 0.003}$} & $16$ &  & $36.40 _{\pm 0.20}$ & $35.23$ & \textcolor{green!70!black}{$-$ $1.17 _{\pm 0.20}$}\\
 & $\Delta$ & $+$ $8$ & $_{\pm 2}$ & \textcolor{red!70!black}{$+$ $0.029 _{\pm 0.003}$} & \textcolor{green!70!black}{$-$ $0.005$} &  & $+$ $7$ & $_{\pm 1}$ & \textcolor{red!70!black}{$+$ $0.64 _{\pm 0.42}$} & \textcolor{green!70!black}{$-$ $0.21$} & \\
\midrule
\midrule
\multirow{3}{*}{FMoW} & Naive & $2$ & $_{\pm 0}$ & $1.583 _{\pm 0.014}$ & $1.494$ & \textcolor{green!70!black}{$-$ $0.089 _{\pm 0.014}$} & $15$ & $_{\pm 19}$ & $43.20 _{\pm 0.46}$ & $37.95$ & \textcolor{green!70!black}{$-$ $5.24 _{\pm 0.46}$}\\
 & Post-hoc & $50$ &  & $2.831 _{\pm 0.053}$ & $1.305$ & \textcolor{green!70!black}{$-$ $1.526 _{\pm 0.053}$} & $48$ &  & $43.18 _{\pm 0.55}$ & $34.93$ & \textcolor{green!70!black}{$-$ $8.24 _{\pm 0.55}$}\\
 & $\Delta$ & $+$ $48$ & $_{\pm 0}$ & \textcolor{red!70!black}{$+$ $1.248 _{\pm 0.062}$} & \textcolor{green!70!black}{$-$ $0.189$} &  & $+$ $33$ & $_{\pm 19}$ & \textcolor{green!70!black}{$-$ $0.02 _{\pm 0.80}$} & \textcolor{green!70!black}{$-$ $3.02$} & \\
\midrule
\midrule
\multirow{3}{*}{Yelp} & Naive & $2$ & $_{\pm 1}$ & $0.908 _{\pm 0.008}$ & $0.841$ & \textcolor{green!70!black}{$-$ $0.067 _{\pm 0.008}$} & $9$ & $_{\pm 8}$ & $39.41 _{\pm 0.76}$ & $36.18$ & \textcolor{green!70!black}{$-$ $3.23 _{\pm 0.76}$}\\
 & Post-hoc & $3$ &  & $0.990 _{\pm 0.044}$ & $0.824$ & \textcolor{green!70!black}{$-$ $0.166 _{\pm 0.044}$} & $3$ &  & $40.28 _{\pm 1.29}$ & $36.14$ & \textcolor{green!70!black}{$-$ $4.14 _{\pm 1.29}$}\\
 & $\Delta$ & $+$ $1$ & $_{\pm 1}$ & \textcolor{red!70!black}{$+$ $0.082 _{\pm 0.040}$} & \textcolor{green!70!black}{$-$ $0.017$} &  & $-$ $6$ & $_{\pm 8}$ & \textcolor{red!70!black}{$+$ $0.87 _{\pm 1.16}$} & \textcolor{green!70!black}{$-$ $0.04$} & \\
\midrule
\midrule
\multirow{3}{*}{Collab} & Naive & $52$ & $_{\pm 18}$ & $0.492 _{\pm 0.044}$ & $0.439$ & \textcolor{green!70!black}{$-$ $0.053 _{\pm 0.044}$} & $75$ & $_{\pm 28}$ & $20.65 _{\pm 1.06}$ & $20.40$ & \textcolor{green!70!black}{$-$ $0.25 _{\pm 1.06}$}\\
 & Post-hoc & $163$ &  & $1.075 _{\pm 0.122}$ & $0.404$ & \textcolor{green!70!black}{$-$ $0.671 _{\pm 0.122}$} & $152$ &  & $20.95 _{\pm 1.26}$ & $18.80$ & \textcolor{green!70!black}{$-$ $2.15 _{\pm 1.26}$}\\
 & $\Delta$ & $+$ $111$ & $_{\pm 18}$ & \textcolor{red!70!black}{$+$ $0.583 _{\pm 0.146}$} & \textcolor{green!70!black}{$-$ $0.035$} &  & $+$ $77$ & $_{\pm 28}$ & \textcolor{red!70!black}{$+$ $0.30 _{\pm 1.31}$} & \textcolor{green!70!black}{$-$ $1.60$} & \\
\midrule
\multirow{3}{*}{Reddit-5k} & Naive & $16$ & $_{\pm 3}$ & $1.150 _{\pm 0.020}$ & $1.099$ & \textcolor{green!70!black}{$-$ $0.051 _{\pm 0.020}$} & $13$ & $_{\pm 5}$ & $47.70 _{\pm 0.97}$ & $46.69$ & \textcolor{green!70!black}{$-$ $1.00 _{\pm 0.97}$}\\
 & Post-hoc & $44$ &  & $1.416 _{\pm 0.063}$ & $1.085$ & \textcolor{green!70!black}{$-$ $0.331 _{\pm 0.063}$} & $50$ &  & $50.55 _{\pm 1.69}$ & $45.89$ & \textcolor{green!70!black}{$-$ $4.66 _{\pm 1.69}$}\\
 & $\Delta$ & $+$ $28$ & $_{\pm 3}$ & \textcolor{red!70!black}{$+$ $0.266 _{\pm 0.068}$} & \textcolor{green!70!black}{$-$ $0.014$} &  & $+$ $37$ & $_{\pm 5}$ & \textcolor{red!70!black}{$+$ $2.86 _{\pm 2.39}$} & \textcolor{green!70!black}{$-$ $0.80$} & \\
\midrule
\multirow{3}{*}{Reddit-12k} & Naive & $16$ & $_{\pm 3}$ & $1.405 _{\pm 0.011}$ & $1.367$ & \textcolor{green!70!black}{$-$ $0.038 _{\pm 0.011}$} & $17$ & $_{\pm 4}$ & $51.78 _{\pm 1.05}$ & $50.34$ & \textcolor{green!70!black}{$-$ $1.45 _{\pm 1.05}$}\\
 & Post-hoc & $41$ &  & $1.585 _{\pm 0.023}$ & $1.346$ & \textcolor{green!70!black}{$-$ $0.239 _{\pm 0.023}$} & $64$ &  & $55.85 _{\pm 0.97}$ & $51.26$ & \textcolor{green!70!black}{$-$ $4.59 _{\pm 0.97}$}\\
 & $\Delta$ & $+$ $25$ & $_{\pm 3}$ & \textcolor{red!70!black}{$+$ $0.180 _{\pm 0.027}$} & \textcolor{green!70!black}{$-$ $0.021$} &  & $+$ $47$ & $_{\pm 4}$ & \textcolor{red!70!black}{$+$ $4.07 _{\pm 1.59}$} & \textcolor{red!70!black}{$+$ $0.92$} & \\
\midrule


==> tables/extra/main/all.tex <==
\multirow{3}{*}{\makecell[l]{C-10-N\\Clean}} & Naive & $90$ & $_{\pm 9}$ & $0.435 _{\pm 0.012}$ & $0.234$ & $0.201 _{\pm 0.012}$ & $92$ & $_{\pm 5}$ & $9.75 _{\pm 0.24}$ & $8.30$ & $1.45 _{\pm 0.24}$\\
 & Post-hoc & $100$ &  & $0.433 _{\pm 0.009}$ & $0.233$ & $0.200 _{\pm 0.009}$ & $96$ &  & $9.82 _{\pm 0.27}$ & $8.24$ & $1.58 _{\pm 0.27}$\\
 & Gain & $-10$ & $_{\pm 9}$ & \textcolor{green!70!black}{$0.001 _{\pm 0.005}$} & \textcolor{green!70!black}{$0.001$} &  & $-4$ & $_{\pm 5}$ & \textcolor{red!70!black}{$-0.07 _{\pm 0.10}$} & \textcolor{green!70!black}{$0.06$} & \\
\midrule
\multirow{3}{*}{\makecell[l]{C-10-N\\Aggregate}} & Naive & $10$ & $_{\pm 3}$ & $0.722 _{\pm 0.018}$ & $0.608$ & $0.114 _{\pm 0.018}$ & $94$ & $_{\pm 6}$ & $19.20 _{\pm 0.39}$ & $15.88$ & $3.33 _{\pm 0.39}$\\
 & Post-hoc & $53$ &  & $0.977 _{\pm 0.030}$ & $0.543$ & $0.434 _{\pm 0.030}$ & $58$ &  & $22.21 _{\pm 0.62}$ & $15.74$ & $6.47 _{\pm 0.62}$\\
 & Gain & $-43$ & $_{\pm 3}$ & \textcolor{red!70!black}{$-0.255 _{\pm 0.027}$} & \textcolor{green!70!black}{$0.065$} &  & $36$ & $_{\pm 6}$ & \textcolor{red!70!black}{$-3.00 _{\pm 0.73}$} & \textcolor{green!70!black}{$0.14$} & \\
\midrule
\multirow{3}{*}{\makecell[l]{C-10-N\\Random1}} & Naive & $8$ & $_{\pm 2}$ & $1.009 _{\pm 0.008}$ & $0.916$ & $0.093 _{\pm 0.008}$ & $22$ & $_{\pm 32}$ & $28.63 _{\pm 0.57}$ & $24.80$ & $3.83 _{\pm 0.57}$\\
 & Post-hoc & $31$ &  & $1.189 _{\pm 0.017}$ & $0.859$ & $0.330 _{\pm 0.017}$ & $67$ &  & $31.58 _{\pm 0.51}$ & $23.50$ & $8.08 _{\pm 0.51}$\\
 & Gain & $-23$ & $_{\pm 2}$ & \textcolor{red!70!black}{$-0.181 _{\pm 0.018}$} & \textcolor{green!70!black}{$0.057$} &  & $-44$ & $_{\pm 32}$ & \textcolor{red!70!black}{$-2.95 _{\pm 0.95}$} & \textcolor{green!70!black}{$1.30$} & \\
\midrule
\multirow{3}{*}{\makecell[l]{C-10-N\\Random2}} & Naive & $10$ & $_{\pm 1}$ & $1.040 _{\pm 0.008}$ & $0.931$ & $0.108 _{\pm 0.008}$ & $14$ & $_{\pm 6}$ & $29.90 _{\pm 0.42}$ & $25.44$ & $4.47 _{\pm 0.42}$\\
 & Post-hoc & $30$ &  & $1.189 _{\pm 0.037}$ & $0.888$ & $0.301 _{\pm 0.037}$ & $74$ &  & $31.15 _{\pm 0.38}$ & $24.12$ & $7.02 _{\pm 0.38}$\\
 & Gain & $-20$ & $_{\pm 1}$ & \textcolor{red!70!black}{$-0.150 _{\pm 0.038}$} & \textcolor{green!70!black}{$0.043$} &  & $-60$ & $_{\pm 6}$ & \textcolor{red!70!black}{$-1.24 _{\pm 0.56}$} & \textcolor{green!70!black}{$1.32$} & \\
\midrule
\multirow{3}{*}{\makecell[l]{C-10-N\\Random3}} & Naive & $9$ & $_{\pm 2}$ & $1.005 _{\pm 0.014}$ & $0.910$ & $0.095 _{\pm 0.014}$ & $24$ & $_{\pm 30}$ & $28.96 _{\pm 0.65}$ & $24.86$ & $4.10 _{\pm 0.65}$\\
 & Post-hoc & $32$ &  & $1.179 _{\pm 0.027}$ & $0.864$ & $0.315 _{\pm 0.027}$ & $38$ &  & $32.39 _{\pm 0.68}$ & $23.44$ & $8.95 _{\pm 0.68}$\\
 & Gain & $-23$ & $_{\pm 2}$ & \textcolor{red!70!black}{$-0.174 _{\pm 0.031}$} & \textcolor{green!70!black}{$0.046$} &  & $-14$ & $_{\pm 30}$ & \textcolor{red!70!black}{$-3.43 _{\pm 1.03}$} & \textcolor{green!70!black}{$1.42$} & \\
\midrule
\multirow{3}{*}{\makecell[l]{C-10-N\\Worst}} & Naive & $8$ & $_{\pm 2}$ & $1.511 _{\pm 0.008}$ & $1.437$ & $0.073 _{\pm 0.008}$ & $10$ & $_{\pm 3}$ & $46.84 _{\pm 0.56}$ & $44.30$ & $2.54 _{\pm 0.56}$\\
 & Post-hoc & $25$ &  & $1.643 _{\pm 0.019}$ & $1.399$ & $0.245 _{\pm 0.019}$ & $24$ &  & $49.67 _{\pm 0.74}$ & $42.88$ & $6.79 _{\pm 0.74}$\\
 & Gain & $-17$ & $_{\pm 2}$ & \textcolor{red!70!black}{$-0.133 _{\pm 0.018}$} & \textcolor{green!70!black}{$0.039$} &  & $-14$ & $_{\pm 3}$ & \textcolor{red!70!black}{$-2.83 _{\pm 0.94}$} & \textcolor{green!70!black}{$1.42$} & \\
\midrule
\midrule
\multirow{3}{*}{\makecell[l]{C-100-N-C\\Clean}} & Naive & $33$ & $_{\pm 35}$ & $1.011 _{\pm 0.014}$ & $0.669$ & $0.342 _{\pm 0.014}$ & $91$ & $_{\pm 4}$ & $23.12 _{\pm 0.40}$ & $19.36$ & $3.76 _{\pm 0.40}$\\
 & Post-hoc & $100$ &  & $1.040 _{\pm 0.019}$ & $0.606$ & $0.435 _{\pm 0.019}$ & $72$ &  & $24.39 _{\pm 0.43}$ & $19.52$ & $4.87 _{\pm 0.43}$\\
 & Gain & $-67$ & $_{\pm 35}$ & \textcolor{red!70!black}{$-0.029 _{\pm 0.023}$} & \textcolor{green!70!black}{$0.063$} &  & $19$ & $_{\pm 4}$ & \textcolor{red!70!black}{$-1.27 _{\pm 0.26}$} & \textcolor{red!70!black}{$-0.16$} & \\
\midrule
\multirow{3}{*}{\makecell[l]{C-100-N-C\\Noisy}} & Naive & $8$ & $_{\pm 2}$ & $1.431 _{\pm 0.008}$ & $1.234$ & $0.198 _{\pm 0.008}$ & $40$ & $_{\pm 41}$ & $41.42 _{\pm 0.45}$ & $34.42$ & $7.00 _{\pm 0.45}$\\
 & Post-hoc & $32$ &  & $1.744 _{\pm 0.049}$ & $1.150$ & $0.594 _{\pm 0.049}$ & $38$ &  & $45.45 _{\pm 0.98}$ & $33.54$ & $11.91 _{\pm 0.98}$\\
 & Gain & $-24$ & $_{\pm 2}$ & \textcolor{red!70!black}{$-0.313 _{\pm 0.048}$} & \textcolor{green!70!black}{$0.084$} &  & $2$ & $_{\pm 41}$ & \textcolor{red!70!black}{$-4.03 _{\pm 1.13}$} & \textcolor{green!70!black}{$0.88$} & \\
\midrule
\midrule
\multirow{3}{*}{\makecell[l]{C-100-N-F\\Clean}} & Naive & $93$ & $_{\pm 5}$ & $1.508 _{\pm 0.017}$ & $1.065$ & $0.443 _{\pm 0.017}$ & $88$ & $_{\pm 5}$ & $33.83 _{\pm 0.37}$ & $29.90$ & $3.93 _{\pm 0.37}$\\
 & Post-hoc & $75$ &  & $1.567 _{\pm 0.019}$ & $1.063$ & $0.504 _{\pm 0.019}$ & $95$ &  & $33.86 _{\pm 0.53}$ & $29.94$ & $3.92 _{\pm 0.53}$\\
 & Gain & $18$ & $_{\pm 5}$ & \textcolor{red!70!black}{$-0.059 _{\pm 0.014}$} & \textcolor{green!70!black}{$0.002$} &  & $-7$ & $_{\pm 5}$ & \textcolor{red!70!black}{$-0.03 _{\pm 0.31}$} & \textcolor{red!70!black}{$-0.04$} & \\
\midrule
\multirow{3}{*}{\makecell[l]{C-100-N-F\\Noisy}} & Naive & $7$ & $_{\pm 2}$ & $2.416 _{\pm 0.022}$ & $2.129$ & $0.287 _{\pm 0.022}$ & $91$ & $_{\pm 7}$ & $58.68 _{\pm 0.49}$ & $51.34$ & $7.34 _{\pm 0.49}$\\
 & Post-hoc & $27$ &  & $3.015 _{\pm 0.079}$ & $1.994$ & $1.021 _{\pm 0.079}$ & $32$ &  & $63.53 _{\pm 0.55}$ & $50.26$ & $13.27 _{\pm 0.55}$\\
 & Gain & $-20$ & $_{\pm 2}$ & \textcolor{red!70!black}{$-0.598 _{\pm 0.075}$} & \textcolor{green!70!black}{$0.135$} &  & $59$ & $_{\pm 7}$ & \textcolor{red!70!black}{$-4.85 _{\pm 0.60}$} & \textcolor{green!70!black}{$1.08$} & \\
\midrule
\midrule
\multirow{3}{*}{Income} & Naive & $5$ & $_{\pm 1}$ & $0.393 _{\pm 0.001}$ & $0.388$ & $0.005 _{\pm 0.001}$ & $7$ & $_{\pm 2}$ & $17.84 _{\pm 0.15}$ & $17.62$ & $0.22 _{\pm 0.15}$\\
 & Post-hoc & $11$ &  & $0.421 _{\pm 0.007}$ & $0.385$ & $0.036 _{\pm 0.007}$ & $19$ &  & $19.21 _{\pm 0.14}$ & $17.40$ & $1.81 _{\pm 0.14}$\\
 & Gain & $-6$ & $_{\pm 1}$ & \textcolor{red!70!black}{$-0.028 _{\pm 0.006}$} & \textcolor{green!70!black}{$0.003$} &  & $-12$ & $_{\pm 2}$ & \textcolor{red!70!black}{$-1.37 _{\pm 0.22}$} & \textcolor{green!70!black}{$0.22$} & \\
\midrule
\multirow{3}{*}{\makecell[l]{Public\\Coverage}} & Naive & $10$ & $_{\pm 2}$ & $0.544 _{\pm 0.001}$ & $0.538$ & $0.006 _{\pm 0.001}$ & $12$ & $_{\pm 3}$ & $27.52 _{\pm 0.24}$ & $27.25$ & $0.28 _{\pm 0.24}$\\
 & Post-hoc & $18$ &  & $0.554 _{\pm 0.002}$ & $0.538$ & $0.016 _{\pm 0.002}$ & $22$ &  & $27.96 _{\pm 0.21}$ & $27.02$ & $0.94 _{\pm 0.21}$\\
 & Gain & $-8$ & $_{\pm 2}$ & \textcolor{red!70!black}{$-0.010 _{\pm 0.002}$} & \textcolor{green!70!black}{$0.000$} &  & $-10$ & $_{\pm 3}$ & \textcolor{red!70!black}{$-0.44 _{\pm 0.25}$} & \textcolor{green!70!black}{$0.22$} & \\
\midrule
\multirow{3}{*}{Mobility} & Naive & $6$ & $_{\pm 2}$ & $0.474 _{\pm 0.002}$ & $0.471$ & $0.003 _{\pm 0.002}$ & $13$ & $_{\pm 5}$ & $21.43 _{\pm 0.18}$ & $21.17$ & $0.26 _{\pm 0.18}$\\
 & Post-hoc & $14$ &  & $0.476 _{\pm 0.003}$ & $0.468$ & $0.008 _{\pm 0.003}$ & $11$ &  & $21.40 _{\pm 0.17}$ & $21.24$ & $0.16 _{\pm 0.17}$\\
 & Gain & $-8$ & $_{\pm 2}$ & \textcolor{red!70!black}{$-0.002 _{\pm 0.003}$} & \textcolor{green!70!black}{$0.003$} &  & $2$ & $_{\pm 5}$ & \textcolor{green!70!black}{$0.03 _{\pm 0.22}$} & \textcolor{red!70!black}{$-0.07$} & \\
\midrule
\multirow{3}{*}{Employment} & Naive & $8$ & $_{\pm 1}$ & $0.380 _{\pm 0.000}$ & $0.378$ & $0.003 _{\pm 0.000}$ & $14$ & $_{\pm 4}$ & $17.94 _{\pm 0.08}$ & $17.72$ & $0.22 _{\pm 0.08}$\\
 & Post-hoc & $15$ &  & $0.383 _{\pm 0.001}$ & $0.377$ & $0.006 _{\pm 0.001}$ & $30$ &  & $18.27 _{\pm 0.12}$ & $17.83$ & $0.43 _{\pm 0.12}$\\
 & Gain & $-7$ & $_{\pm 1}$ & \textcolor{red!70!black}{$-0.003 _{\pm 0.001}$} & \textcolor{green!70!black}{$0.000$} &  & $-16$ & $_{\pm 4}$ & \textcolor{red!70!black}{$-0.33 _{\pm 0.16}$} & \textcolor{red!70!black}{$-0.11$} & \\
\midrule
\multirow{3}{*}{Travel Time} & Naive & $6$ & $_{\pm 2}$ & $0.597 _{\pm 0.002}$ & $0.596$ & $0.001 _{\pm 0.002}$ & $9$ & $_{\pm 1}$ & $35.77 _{\pm 0.34}$ & $35.44$ & $0.32 _{\pm 0.34}$\\
 & Post-hoc & $15$ &  & $0.626 _{\pm 0.003}$ & $0.591$ & $0.035 _{\pm 0.003}$ & $16$ &  & $36.40 _{\pm 0.20}$ & $35.23$ & $1.17 _{\pm 0.20}$\\
 & Gain & $-8$ & $_{\pm 2}$ & \textcolor{red!70!black}{$-0.029 _{\pm 0.003}$} & \textcolor{green!70!black}{$0.005$} &  & $-7$ & $_{\pm 1}$ & \textcolor{red!70!black}{$-0.64 _{\pm 0.42}$} & \textcolor{green!70!black}{$0.21$} & \\
\midrule
\midrule
\multirow{3}{*}{FMoW} & Naive & $2$ & $_{\pm 0}$ & $1.583 _{\pm 0.014}$ & $1.494$ & $0.089 _{\pm 0.014}$ & $15$ & $_{\pm 19}$ & $43.20 _{\pm 0.46}$ & $37.95$ & $5.24 _{\pm 0.46}$\\
 & Post-hoc & $50$ &  & $2.831 _{\pm 0.053}$ & $1.305$ & $1.526 _{\pm 0.053}$ & $48$ &  & $43.18 _{\pm 0.55}$ & $34.93$ & $8.24 _{\pm 0.55}$\\
 & Gain & $-48$ & $_{\pm 0}$ & \textcolor{red!70!black}{$-1.248 _{\pm 0.062}$} & \textcolor{green!70!black}{$0.189$} &  & $-33$ & $_{\pm 19}$ & \textcolor{green!70!black}{$0.02 _{\pm 0.80}$} & \textcolor{green!70!black}{$3.02$} & \\
\midrule
\midrule
\multirow{3}{*}{Yelp} & Naive & $2$ & $_{\pm 1}$ & $0.908 _{\pm 0.008}$ & $0.841$ & $0.067 _{\pm 0.008}$ & $9$ & $_{\pm 8}$ & $39.41 _{\pm 0.76}$ & $36.18$ & $3.23 _{\pm 0.76}$\\
 & Post-hoc & $3$ &  & $0.990 _{\pm 0.044}$ & $0.824$ & $0.166 _{\pm 0.044}$ & $3$ &  & $40.28 _{\pm 1.29}$ & $36.14$ & $4.14 _{\pm 1.29}$\\
 & Gain & $-1$ & $_{\pm 1}$ & \textcolor{red!70!black}{$-0.082 _{\pm 0.040}$} & \textcolor{green!70!black}{$0.017$} &  & $6$ & $_{\pm 8}$ & \textcolor{red!70!black}{$-0.87 _{\pm 1.16}$} & \textcolor{green!70!black}{$0.04$} & \\
\midrule
\midrule
\multirow{3}{*}{Collab} & Naive & $52$ & $_{\pm 18}$ & $0.492 _{\pm 0.044}$ & $0.439$ & $0.053 _{\pm 0.044}$ & $75$ & $_{\pm 28}$ & $20.65 _{\pm 1.06}$ & $20.40$ & $0.25 _{\pm 1.06}$\\
 & Post-hoc & $163$ &  & $1.075 _{\pm 0.122}$ & $0.404$ & $0.671 _{\pm 0.122}$ & $152$ &  & $20.95 _{\pm 1.26}$ & $18.80$ & $2.15 _{\pm 1.26}$\\
 & Gain & $-111$ & $_{\pm 18}$ & \textcolor{red!70!black}{$-0.583 _{\pm 0.146}$} & \textcolor{green!70!black}{$0.035$} &  & $-77$ & $_{\pm 28}$ & \textcolor{red!70!black}{$-0.30 _{\pm 1.31}$} & \textcolor{green!70!black}{$1.60$} & \\
\midrule
\multirow{3}{*}{Reddit-5k} & Naive & $16$ & $_{\pm 3}$ & $1.150 _{\pm 0.020}$ & $1.099$ & $0.051 _{\pm 0.020}$ & $13$ & $_{\pm 5}$ & $47.70 _{\pm 0.97}$ & $46.69$ & $1.00 _{\pm 0.97}$\\
 & Post-hoc & $44$ &  & $1.416 _{\pm 0.063}$ & $1.085$ & $0.331 _{\pm 0.063}$ & $50$ &  & $50.55 _{\pm 1.69}$ & $45.89$ & $4.66 _{\pm 1.69}$\\
 & Gain & $-28$ & $_{\pm 3}$ & \textcolor{red!70!black}{$-0.266 _{\pm 0.068}$} & \textcolor{green!70!black}{$0.014$} &  & $-37$ & $_{\pm 5}$ & \textcolor{red!70!black}{$-2.86 _{\pm 2.39}$} & \textcolor{green!70!black}{$0.80$} & \\
\midrule
\multirow{3}{*}{Reddit-12k} & Naive & $16$ & $_{\pm 3}$ & $1.405 _{\pm 0.011}$ & $1.367$ & $0.038 _{\pm 0.011}$ & $17$ & $_{\pm 4}$ & $51.78 _{\pm 1.05}$ & $50.34$ & $1.45 _{\pm 1.05}$\\
 & Post-hoc & $41$ &  & $1.585 _{\pm 0.023}$ & $1.346$ & $0.239 _{\pm 0.023}$ & $64$ &  & $55.85 _{\pm 0.97}$ & $51.26$ & $4.59 _{\pm 0.97}$\\
 & Gain & $-25$ & $_{\pm 3}$ & \textcolor{red!70!black}{$-0.180 _{\pm 0.027}$} & \textcolor{green!70!black}{$0.021$} &  & $-47$ & $_{\pm 4}$ & \textcolor{red!70!black}{$-4.07 _{\pm 1.59}$} & \textcolor{red!70!black}{$-0.92$} & \\
\midrule


==> tables/extra/main/cherry.tex <==
\multirow{3}{*}{\makecell[l]{C-10-N\\Clean}} & Naive & $90$ & $_{\pm 9}$ & $0.435 _{\pm 0.012}$ & $0.234$ & $0.201 _{\pm 0.012}$ & $92$ & $_{\pm 5}$ & $9.75 _{\pm 0.24}$ & $8.30$ & $1.45 _{\pm 0.24}$\\
 & Post-hoc & $100$ &  & $0.433 _{\pm 0.009}$ & $0.233$ & $0.200 _{\pm 0.009}$ & $96$ &  & $9.82 _{\pm 0.27}$ & $8.24$ & $1.58 _{\pm 0.27}$\\
 & Gain & $-10$ & $_{\pm 9}$ & \textcolor{green!70!black}{$0.001 _{\pm 0.005}$} & \textcolor{green!70!black}{$0.001$} &  & $-4$ & $_{\pm 5}$ & \textcolor{red!70!black}{$-0.07 _{\pm 0.10}$} & \textcolor{green!70!black}{$0.06$} & \\
\midrule
\multirow{3}{*}{\makecell[l]{C-10-N\\Aggregate}} & Naive & $10$ & $_{\pm 3}$ & $0.722 _{\pm 0.018}$ & $0.608$ & $0.114 _{\pm 0.018}$ & $94$ & $_{\pm 6}$ & $19.20 _{\pm 0.39}$ & $15.88$ & $3.33 _{\pm 0.39}$\\
 & Post-hoc & $53$ &  & $0.977 _{\pm 0.030}$ & $0.543$ & $0.434 _{\pm 0.030}$ & $58$ &  & $22.21 _{\pm 0.62}$ & $15.74$ & $6.47 _{\pm 0.62}$\\
 & Gain & $-43$ & $_{\pm 3}$ & \textcolor{red!70!black}{$-0.255 _{\pm 0.027}$} & \textcolor{green!70!black}{$0.065$} &  & $36$ & $_{\pm 6}$ & \textcolor{red!70!black}{$-3.00 _{\pm 0.73}$} & \textcolor{green!70!black}{$0.14$} & \\
\midrule
\multirow{3}{*}{\makecell[l]{C-10-N\\Random1}} & Naive & $8$ & $_{\pm 2}$ & $1.009 _{\pm 0.008}$ & $0.916$ & $0.093 _{\pm 0.008}$ & $22$ & $_{\pm 32}$ & $28.63 _{\pm 0.57}$ & $24.80$ & $3.83 _{\pm 0.57}$\\
 & Post-hoc & $31$ &  & $1.189 _{\pm 0.017}$ & $0.859$ & $0.330 _{\pm 0.017}$ & $67$ &  & $31.58 _{\pm 0.51}$ & $23.50$ & $8.08 _{\pm 0.51}$\\
 & Gain & $-23$ & $_{\pm 2}$ & \textcolor{red!70!black}{$-0.181 _{\pm 0.018}$} & \textcolor{green!70!black}{$0.057$} &  & $-44$ & $_{\pm 32}$ & \textcolor{red!70!black}{$-2.95 _{\pm 0.95}$} & \textcolor{green!70!black}{$1.30$} & \\
\midrule
\multirow{3}{*}{\makecell[l]{C-10-N\\Worst}} & Naive & $8$ & $_{\pm 2}$ & $1.511 _{\pm 0.008}$ & $1.437$ & $0.073 _{\pm 0.008}$ & $10$ & $_{\pm 3}$ & $46.84 _{\pm 0.56}$ & $44.30$ & $2.54 _{\pm 0.56}$\\
 & Post-hoc & $25$ &  & $1.643 _{\pm 0.019}$ & $1.399$ & $0.245 _{\pm 0.019}$ & $24$ &  & $49.67 _{\pm 0.74}$ & $42.88$ & $6.79 _{\pm 0.74}$\\
 & Gain & $-17$ & $_{\pm 2}$ & \textcolor{red!70!black}{$-0.133 _{\pm 0.018}$} & \textcolor{green!70!black}{$0.039$} &  & $-14$ & $_{\pm 3}$ & \textcolor{red!70!black}{$-2.83 _{\pm 0.94}$} & \textcolor{green!70!black}{$1.42$} & \\
\midrule
\midrule
\multirow{3}{*}{\makecell[l]{C-100-N-F\\Clean}} & Naive & $93$ & $_{\pm 5}$ & $1.508 _{\pm 0.017}$ & $1.065$ & $0.443 _{\pm 0.017}$ & $88$ & $_{\pm 5}$ & $33.83 _{\pm 0.37}$ & $29.90$ & $3.93 _{\pm 0.37}$\\
 & Post-hoc & $75$ &  & $1.567 _{\pm 0.019}$ & $1.063$ & $0.504 _{\pm 0.019}$ & $95$ &  & $33.86 _{\pm 0.53}$ & $29.94$ & $3.92 _{\pm 0.53}$\\
 & Gain & $18$ & $_{\pm 5}$ & \textcolor{red!70!black}{$-0.059 _{\pm 0.014}$} & \textcolor{green!70!black}{$0.002$} &  & $-7$ & $_{\pm 5}$ & \textcolor{red!70!black}{$-0.03 _{\pm 0.31}$} & \textcolor{red!70!black}{$-0.04$} & \\
\midrule
\multirow{3}{*}{\makecell[l]{C-100-N-F\\Noisy}} & Naive & $7$ & $_{\pm 2}$ & $2.416 _{\pm 0.022}$ & $2.129$ & $0.287 _{\pm 0.022}$ & $91$ & $_{\pm 7}$ & $58.68 _{\pm 0.49}$ & $51.34$ & $7.34 _{\pm 0.49}$\\
 & Post-hoc & $27$ &  & $3.015 _{\pm 0.079}$ & $1.994$ & $1.021 _{\pm 0.079}$ & $32$ &  & $63.53 _{\pm 0.55}$ & $50.26$ & $13.27 _{\pm 0.55}$\\
 & Gain & $-20$ & $_{\pm 2}$ & \textcolor{red!70!black}{$-0.598 _{\pm 0.075}$} & \textcolor{green!70!black}{$0.135$} &  & $59$ & $_{\pm 7}$ & \textcolor{red!70!black}{$-4.85 _{\pm 0.60}$} & \textcolor{green!70!black}{$1.08$} & \\
\midrule
\midrule
\multirow{3}{*}{FMoW} & Naive & $2$ & $_{\pm 0}$ & $1.583 _{\pm 0.014}$ & $1.494$ & $0.089 _{\pm 0.014}$ & $15$ & $_{\pm 19}$ & $43.20 _{\pm 0.46}$ & $37.95$ & $5.24 _{\pm 0.46}$\\
 & Post-hoc & $50$ &  & $2.831 _{\pm 0.053}$ & $1.305$ & $1.526 _{\pm 0.053}$ & $48$ &  & $43.18 _{\pm 0.55}$ & $34.93$ & $8.24 _{\pm 0.55}$\\
 & Gain & $-48$ & $_{\pm 0}$ & \textcolor{red!70!black}{$-1.248 _{\pm 0.062}$} & \textcolor{green!70!black}{$0.189$} &  & $-33$ & $_{\pm 19}$ & \textcolor{green!70!black}{$0.02 _{\pm 0.80}$} & \textcolor{green!70!black}{$3.02$} & \\
\midrule
\midrule
\multirow{3}{*}{Yelp} & Naive & $2$ & $_{\pm 1}$ & $0.908 _{\pm 0.008}$ & $0.841$ & $0.067 _{\pm 0.008}$ & $9$ & $_{\pm 8}$ & $39.41 _{\pm 0.76}$ & $36.18$ & $3.23 _{\pm 0.76}$\\
 & Post-hoc & $3$ &  & $0.990 _{\pm 0.044}$ & $0.824$ & $0.166 _{\pm 0.044}$ & $3$ &  & $40.28 _{\pm 1.29}$ & $36.14$ & $4.14 _{\pm 1.29}$\\
 & Gain & $-1$ & $_{\pm 1}$ & \textcolor{red!70!black}{$-0.082 _{\pm 0.040}$} & \textcolor{green!70!black}{$0.017$} &  & $6$ & $_{\pm 8}$ & \textcolor{red!70!black}{$-0.87 _{\pm 1.16}$} & \textcolor{green!70!black}{$0.04$} & \\
\midrule
\midrule
\multirow{3}{*}{Income} & Naive & $5$ & $_{\pm 1}$ & $0.393 _{\pm 0.001}$ & $0.388$ & $0.005 _{\pm 0.001}$ & $7$ & $_{\pm 2}$ & $17.84 _{\pm 0.15}$ & $17.62$ & $0.22 _{\pm 0.15}$\\
 & Post-hoc & $11$ &  & $0.421 _{\pm 0.007}$ & $0.385$ & $0.036 _{\pm 0.007}$ & $19$ &  & $19.21 _{\pm 0.14}$ & $17.40$ & $1.81 _{\pm 0.14}$\\
 & Gain & $-6$ & $_{\pm 1}$ & \textcolor{red!70!black}{$-0.028 _{\pm 0.006}$} & \textcolor{green!70!black}{$0.003$} &  & $-12$ & $_{\pm 2}$ & \textcolor{red!70!black}{$-1.37 _{\pm 0.22}$} & \textcolor{green!70!black}{$0.22$} & \\
\midrule
\multirow{3}{*}{\makecell[l]{Public\\Coverage}} & Naive & $10$ & $_{\pm 2}$ & $0.544 _{\pm 0.001}$ & $0.538$ & $0.006 _{\pm 0.001}$ & $12$ & $_{\pm 3}$ & $27.52 _{\pm 0.24}$ & $27.25$ & $0.28 _{\pm 0.24}$\\
 & Post-hoc & $18$ &  & $0.554 _{\pm 0.002}$ & $0.538$ & $0.016 _{\pm 0.002}$ & $22$ &  & $27.96 _{\pm 0.21}$ & $27.02$ & $0.94 _{\pm 0.21}$\\
 & Gain & $-8$ & $_{\pm 2}$ & \textcolor{red!70!black}{$-0.010 _{\pm 0.002}$} & \textcolor{green!70!black}{$0.000$} &  & $-10$ & $_{\pm 3}$ & \textcolor{red!70!black}{$-0.44 _{\pm 0.25}$} & \textcolor{green!70!black}{$0.22$} & \\
\midrule
\multirow{3}{*}{Travel Time} & Naive & $6$ & $_{\pm 2}$ & $0.597 _{\pm 0.002}$ & $0.596$ & $0.001 _{\pm 0.002}$ & $9$ & $_{\pm 1}$ & $35.77 _{\pm 0.34}$ & $35.44$ & $0.32 _{\pm 0.34}$\\
 & Post-hoc & $15$ &  & $0.626 _{\pm 0.003}$ & $0.591$ & $0.035 _{\pm 0.003}$ & $16$ &  & $36.40 _{\pm 0.20}$ & $35.23$ & $1.17 _{\pm 0.20}$\\
 & Gain & $-8$ & $_{\pm 2}$ & \textcolor{red!70!black}{$-0.029 _{\pm 0.003}$} & \textcolor{green!70!black}{$0.005$} &  & $-7$ & $_{\pm 1}$ & \textcolor{red!70!black}{$-0.64 _{\pm 0.42}$} & \textcolor{green!70!black}{$0.21$} & \\
\midrule
\midrule
\multirow{3}{*}{Collab} & Naive & $52$ & $_{\pm 18}$ & $0.492 _{\pm 0.044}$ & $0.439$ & $0.053 _{\pm 0.044}$ & $75$ & $_{\pm 28}$ & $20.65 _{\pm 1.06}$ & $20.40$ & $0.25 _{\pm 1.06}$\\
 & Post-hoc & $163$ &  & $1.075 _{\pm 0.122}$ & $0.404$ & $0.671 _{\pm 0.122}$ & $152$ &  & $20.95 _{\pm 1.26}$ & $18.80$ & $2.15 _{\pm 1.26}$\\
 & Gain & $-111$ & $_{\pm 18}$ & \textcolor{red!70!black}{$-0.583 _{\pm 0.146}$} & \textcolor{green!70!black}{$0.035$} &  & $-77$ & $_{\pm 28}$ & \textcolor{red!70!black}{$-0.30 _{\pm 1.31}$} & \textcolor{green!70!black}{$1.60$} & \\
\midrule
\multirow{3}{*}{Reddit-5k} & Naive & $16$ & $_{\pm 3}$ & $1.150 _{\pm 0.020}$ & $1.099$ & $0.051 _{\pm 0.020}$ & $13$ & $_{\pm 5}$ & $47.70 _{\pm 0.97}$ & $46.69$ & $1.00 _{\pm 0.97}$\\
 & Post-hoc & $44$ &  & $1.416 _{\pm 0.063}$ & $1.085$ & $0.331 _{\pm 0.063}$ & $50$ &  & $50.55 _{\pm 1.69}$ & $45.89$ & $4.66 _{\pm 1.69}$\\
 & Gain & $-28$ & $_{\pm 3}$ & \textcolor{red!70!black}{$-0.266 _{\pm 0.068}$} & \textcolor{green!70!black}{$0.014$} &  & $-37$ & $_{\pm 5}$ & \textcolor{red!70!black}{$-2.86 _{\pm 2.39}$} & \textcolor{green!70!black}{$0.80$} & \\
\midrule
\multirow{3}{*}{Reddit-12k} & Naive & $16$ & $_{\pm 3}$ & $1.405 _{\pm 0.011}$ & $1.367$ & $0.038 _{\pm 0.011}$ & $17$ & $_{\pm 4}$ & $51.78 _{\pm 1.05}$ & $50.34$ & $1.45 _{\pm 1.05}$\\
 & Post-hoc & $41$ &  & $1.585 _{\pm 0.023}$ & $1.346$ & $0.239 _{\pm 0.023}$ & $64$ &  & $55.85 _{\pm 0.97}$ & $51.26$ & $4.59 _{\pm 0.97}$\\
 & Gain & $-25$ & $_{\pm 3}$ & \textcolor{red!70!black}{$-0.180 _{\pm 0.027}$} & \textcolor{green!70!black}{$0.021$} &  & $-47$ & $_{\pm 4}$ & \textcolor{red!70!black}{$-4.07 _{\pm 1.59}$} & \textcolor{red!70!black}{$-0.92$} & \\
\midrule


==> tables/extra/main/naive_vs_posthoc/cifar.tex <==
\multirow{3}{*}{\makecell[l]{C-10-N\\Clean}}&Greedy&&$90$&$_{\pm 9}$&$0.435 _{\pm 0.012}$&$0.234$&$0.201 _{\pm 0.012}$&&$92$&$_{\pm 5}$&$9.75 _{\pm 0.24}$&$8.30$&$1.45 _{\pm 0.24}$\\
&Post-hoc&&$100$ & &$0.433 _{\pm 0.009}$&$0.233$&$0.200 _{\pm 0.009}$&&$96$ & &$9.82 _{\pm 0.27}$&$8.24$&$1.58 _{\pm 0.27}$\\
&$\Delta$&&\textcolor{red!70!black}{$\uparrow 10$}&\textcolor{red!70!black}{$_{\pm 9}$}&\textcolor{green!70!black}{$\downarrow 0.001 _{\pm 0.005}$}&\textcolor{green!70!black}{$\downarrow 0.001$}&--&&\textcolor{red!70!black}{$\uparrow 4$}&\textcolor{red!70!black}{$_{\pm 5}$}&\textcolor{red!70!black}{$\uparrow 0.07 _{\pm 0.10}$}&\textcolor{green!70!black}{$\downarrow 0.06$}&--\\
\midrule
\multirow{3}{*}{\makecell[l]{C-10-N\\Aggregate}}&Greedy&&$10$&$_{\pm 3}$&$0.722 _{\pm 0.018}$&$0.608$&$0.114 _{\pm 0.018}$&&$94$&$_{\pm 6}$&$19.20 _{\pm 0.39}$&$15.88$&$3.33 _{\pm 0.39}$\\
&Post-hoc&&$53$ & &$0.977 _{\pm 0.030}$&$0.543$&$0.434 _{\pm 0.030}$&&$58$ & &$22.21 _{\pm 0.62}$&$15.74$&$6.47 _{\pm 0.62}$\\
&$\Delta$&&\textcolor{red!70!black}{$\uparrow 43$}&\textcolor{red!70!black}{$_{\pm 3}$}&\textcolor{red!70!black}{$\uparrow 0.255 _{\pm 0.027}$}&\textcolor{green!70!black}{$\downarrow 0.065$}&--&&\textcolor{green!70!black}{$\downarrow 36$}&\textcolor{green!70!black}{$_{\pm 6}$}&\textcolor{red!70!black}{$\uparrow 3.00 _{\pm 0.73}$}&\textcolor{green!70!black}{$\downarrow 0.14$}&--\\
\midrule
\multirow{3}{*}{\makecell[l]{C-10-N\\Random1}}&Greedy&&$8$&$_{\pm 2}$&$1.009 _{\pm 0.008}$&$0.916$&$0.093 _{\pm 0.008}$&&$22$&$_{\pm 32}$&$28.63 _{\pm 0.57}$&$24.80$&$3.83 _{\pm 0.57}$\\
&Post-hoc&&$31$ & &$1.189 _{\pm 0.017}$&$0.859$&$0.330 _{\pm 0.017}$&&$67$ & &$31.58 _{\pm 0.51}$&$23.50$&$8.08 _{\pm 0.51}$\\
&$\Delta$&&\textcolor{red!70!black}{$\uparrow 23$}&\textcolor{red!70!black}{$_{\pm 2}$}&\textcolor{red!70!black}{$\uparrow 0.181 _{\pm 0.018}$}&\textcolor{green!70!black}{$\downarrow 0.057$}&--&&\textcolor{red!70!black}{$\uparrow 44$}&\textcolor{red!70!black}{$_{\pm 32}$}&\textcolor{red!70!black}{$\uparrow 2.95 _{\pm 0.95}$}&\textcolor{green!70!black}{$\downarrow 1.30$}&--\\
\midrule
\multirow{3}{*}{\makecell[l]{C-10-N\\Worst}}&Greedy&&$8$&$_{\pm 2}$&$1.511 _{\pm 0.008}$&$1.437$&$0.073 _{\pm 0.008}$&&$10$&$_{\pm 3}$&$46.84 _{\pm 0.56}$&$44.30$&$2.54 _{\pm 0.56}$\\
&Post-hoc&&$25$ & &$1.643 _{\pm 0.019}$&$1.399$&$0.245 _{\pm 0.019}$&&$24$ & &$49.67 _{\pm 0.74}$&$42.88$&$6.79 _{\pm 0.74}$\\
&$\Delta$&&\textcolor{red!70!black}{$\uparrow 17$}&\textcolor{red!70!black}{$_{\pm 2}$}&\textcolor{red!70!black}{$\uparrow 0.133 _{\pm 0.018}$}&\textcolor{green!70!black}{$\downarrow 0.039$}&--&&\textcolor{red!70!black}{$\uparrow 14$}&\textcolor{red!70!black}{$_{\pm 3}$}&\textcolor{red!70!black}{$\uparrow 2.83 _{\pm 0.94}$}&\textcolor{green!70!black}{$\downarrow 1.42$}&--\\
\midrule
\midrule
\multirow{3}{*}{\makecell[l]{C-100-N-F\\Clean}}&Greedy&&$93$&$_{\pm 5}$&$1.508 _{\pm 0.017}$&$1.065$&$0.443 _{\pm 0.017}$&&$88$&$_{\pm 5}$&$33.83 _{\pm 0.37}$&$29.90$&$3.93 _{\pm 0.37}$\\
&Post-hoc&&$75$ & &$1.567 _{\pm 0.019}$&$1.063$&$0.504 _{\pm 0.019}$&&$95$ & &$33.86 _{\pm 0.53}$&$29.94$&$3.92 _{\pm 0.53}$\\
&$\Delta$&&\textcolor{green!70!black}{$\downarrow 18$}&\textcolor{green!70!black}{$_{\pm 5}$}&\textcolor{red!70!black}{$\uparrow 0.059 _{\pm 0.014}$}&\textcolor{green!70!black}{$\downarrow 0.002$}&--&&\textcolor{red!70!black}{$\uparrow 7$}&\textcolor{red!70!black}{$_{\pm 5}$}&\textcolor{red!70!black}{$\uparrow 0.03 _{\pm 0.31}$}&\textcolor{red!70!black}{$\uparrow 0.04$}&--\\
\midrule
\multirow{3}{*}{\makecell[l]{C-100-N-F\\Noisy}}&Greedy&&$7$&$_{\pm 2}$&$2.416 _{\pm 0.022}$&$2.129$&$0.287 _{\pm 0.022}$&&$91$&$_{\pm 7}$&$58.68 _{\pm 0.49}$&$51.34$&$7.34 _{\pm 0.49}$\\
&Post-hoc&&$27$ & &$3.015 _{\pm 0.079}$&$1.994$&$1.021 _{\pm 0.079}$&&$32$ & &$63.53 _{\pm 0.55}$&$50.26$&$13.27 _{\pm 0.55}$\\
&$\Delta$&&\textcolor{red!70!black}{$\uparrow 20$}&\textcolor{red!70!black}{$_{\pm 2}$}&\textcolor{red!70!black}{$\uparrow 0.598 _{\pm 0.075}$}&\textcolor{green!70!black}{$\downarrow 0.135$}&--&&\textcolor{green!70!black}{$\downarrow 59$}&\textcolor{green!70!black}{$_{\pm 7}$}&\textcolor{red!70!black}{$\uparrow 4.85 _{\pm 0.60}$}&\textcolor{green!70!black}{$\downarrow 1.08$}&--\\


==> tables/extra/main/naive_vs_posthoc/real.tex <==
\multirow{3}{*}{FMoW}&Greedy&&$2$&$_{\pm 0}$&$1.583 _{\pm 0.014}$&$1.494$&$0.089 _{\pm 0.014}$&&$15$&$_{\pm 19}$&$43.20 _{\pm 0.46}$&$37.95$&$5.24 _{\pm 0.46}$\\
&Post-hoc&&$50$ & &$2.831 _{\pm 0.053}$&$1.305$&$1.526 _{\pm 0.053}$&&$48$ & &$43.18 _{\pm 0.55}$&$34.93$&$8.24 _{\pm 0.55}$\\
&$\Delta$&&\textcolor{red!70!black}{$\uparrow 48$}&\textcolor{red!70!black}{$_{\pm 0}$}&\textcolor{red!70!black}{$\uparrow 1.248 _{\pm 0.062}$}&\textcolor{green!70!black}{$\downarrow 0.189$}&--&&\textcolor{red!70!black}{$\uparrow 33$}&\textcolor{red!70!black}{$_{\pm 19}$}&\textcolor{green!70!black}{$\downarrow 0.02 _{\pm 0.80}$}&\textcolor{green!70!black}{$\downarrow 3.02$}&--\\
\midrule
\multirow{3}{*}{Yelp}&Greedy&&$2$&$_{\pm 1}$&$0.908 _{\pm 0.008}$&$0.841$&$0.067 _{\pm 0.008}$&&$9$&$_{\pm 8}$&$39.41 _{\pm 0.76}$&$36.18$&$3.23 _{\pm 0.76}$\\
&Post-hoc&&$3$ & &$0.990 _{\pm 0.044}$&$0.824$&$0.166 _{\pm 0.044}$&&$3$ & &$40.28 _{\pm 1.29}$&$36.14$&$4.14 _{\pm 1.29}$\\
&$\Delta$&&\textcolor{red!70!black}{$\uparrow 1$}&\textcolor{red!70!black}{$_{\pm 1}$}&\textcolor{red!70!black}{$\uparrow 0.082 _{\pm 0.040}$}&\textcolor{green!70!black}{$\downarrow 0.017$}&--&&\textcolor{green!70!black}{$\downarrow 6$}&\textcolor{green!70!black}{$_{\pm 8}$}&\textcolor{red!70!black}{$\uparrow 0.87 _{\pm 1.16}$}&\textcolor{green!70!black}{$\downarrow 0.04$}&--\\
\midrule
\multirow{3}{*}{Income}&Greedy&&$5$&$_{\pm 1}$&$0.393 _{\pm 0.001}$&$0.388$&$0.005 _{\pm 0.001}$&&$7$&$_{\pm 2}$&$17.84 _{\pm 0.15}$&$17.62$&$0.22 _{\pm 0.15}$\\
&Post-hoc&&$11$ & &$0.421 _{\pm 0.007}$&$0.385$&$0.036 _{\pm 0.007}$&&$19$ & &$19.21 _{\pm 0.14}$&$17.40$&$1.81 _{\pm 0.14}$\\
&$\Delta$&&\textcolor{red!70!black}{$\uparrow 6$}&\textcolor{red!70!black}{$_{\pm 1}$}&\textcolor{red!70!black}{$\uparrow 0.028 _{\pm 0.006}$}&\textcolor{green!70!black}{$\downarrow 0.003$}&--&&\textcolor{red!70!black}{$\uparrow 12$}&\textcolor{red!70!black}{$_{\pm 2}$}&\textcolor{red!70!black}{$\uparrow 1.37 _{\pm 0.22}$}&\textcolor{green!70!black}{$\downarrow 0.22$}&--\\
\midrule
\multirow{3}{*}{\makecell[l]{Public\\Coverage}}&Greedy&&$10$&$_{\pm 2}$&$0.544 _{\pm 0.001}$&$0.538$&$0.006 _{\pm 0.001}$&&$12$&$_{\pm 3}$&$27.52 _{\pm 0.24}$&$27.25$&$0.28 _{\pm 0.24}$\\
&Post-hoc&&$18$ & &$0.554 _{\pm 0.002}$&$0.538$&$0.016 _{\pm 0.002}$&&$22$ & &$27.96 _{\pm 0.21}$&$27.02$&$0.94 _{\pm 0.21}$\\
&$\Delta$&&\textcolor{red!70!black}{$\uparrow 8$}&\textcolor{red!70!black}{$_{\pm 2}$}&\textcolor{red!70!black}{$\uparrow 0.010 _{\pm 0.002}$}&\textcolor{green!70!black}{$\downarrow 0.000$}&--&&\textcolor{red!70!black}{$\uparrow 10$}&\textcolor{red!70!black}{$_{\pm 3}$}&\textcolor{red!70!black}{$\uparrow 0.44 _{\pm 0.25}$}&\textcolor{green!70!black}{$\downarrow 0.22$}&--\\
\midrule
\multirow{3}{*}{\makecell[l]{Travel\\Time}}&Greedy&&$6$&$_{\pm 2}$&$0.597 _{\pm 0.002}$&$0.596$&$0.001 _{\pm 0.002}$&&$9$&$_{\pm 1}$&$35.77 _{\pm 0.34}$&$35.44$&$0.32 _{\pm 0.34}$\\
&Post-hoc&&$15$ & &$0.626 _{\pm 0.003}$&$0.591$&$0.035 _{\pm 0.003}$&&$16$ & &$36.40 _{\pm 0.20}$&$35.23$&$1.17 _{\pm 0.20}$\\
&$\Delta$&&\textcolor{red!70!black}{$\uparrow 8$}&\textcolor{red!70!black}{$_{\pm 2}$}&\textcolor{red!70!black}{$\uparrow 0.029 _{\pm 0.003}$}&\textcolor{green!70!black}{$\downarrow 0.005$}&--&&\textcolor{red!70!black}{$\uparrow 7$}&\textcolor{red!70!black}{$_{\pm 1}$}&\textcolor{red!70!black}{$\uparrow 0.64 _{\pm 0.42}$}&\textcolor{green!70!black}{$\downarrow 0.21$}&--\\
\midrule
\multirow{3}{*}{Collab}&Greedy&&$52$&$_{\pm 18}$&$0.492 _{\pm 0.044}$&$0.439$&$0.053 _{\pm 0.044}$&&$75$&$_{\pm 28}$&$20.65 _{\pm 1.06}$&$20.40$&$0.25 _{\pm 1.06}$\\
&Post-hoc&&$163$ & &$1.075 _{\pm 0.122}$&$0.404$&$0.671 _{\pm 0.122}$&&$152$ & &$20.95 _{\pm 1.26}$&$18.80$&$2.15 _{\pm 1.26}$\\
&$\Delta$&&\textcolor{red!70!black}{$\uparrow 111$}&\textcolor{red!70!black}{$_{\pm 18}$}&\textcolor{red!70!black}{$\uparrow 0.583 _{\pm 0.146}$}&\textcolor{green!70!black}{$\downarrow 0.035$}&--&&\textcolor{red!70!black}{$\uparrow 77$}&\textcolor{red!70!black}{$_{\pm 28}$}&\textcolor{red!70!black}{$\uparrow 0.30 _{\pm 1.31}$}&\textcolor{green!70!black}{$\downarrow 1.60$}&--\\
\midrule
\multirow{3}{*}{Reddit-5k}&Greedy&&$15$&$_{\pm 4}$&$1.154 _{\pm 0.022}$&$1.101$&$0.053 _{\pm 0.022}$&&$13$&$_{\pm 5}$&$47.42 _{\pm 0.64}$&$47.09$&$0.33 _{\pm 0.64}$\\
&Post-hoc&&$44$ & &$1.448 _{\pm 0.058}$&$1.085$&$0.362 _{\pm 0.058}$&&$45$ & &$50.75 _{\pm 1.83}$&$45.49$&$5.26 _{\pm 1.83}$\\
&$\Delta$&&\textcolor{red!70!black}{$\uparrow 29$}&\textcolor{red!70!black}{$_{\pm 4}$}&\textcolor{red!70!black}{$\uparrow 0.294 _{\pm 0.059}$}&\textcolor{green!70!black}{$\downarrow 0.015$}&--&&\textcolor{red!70!black}{$\uparrow 32$}&\textcolor{red!70!black}{$_{\pm 5}$}&\textcolor{red!70!black}{$\uparrow 3.33 _{\pm 2.05}$}&\textcolor{green!70!black}{$\downarrow 1.60$}&--\\
\midrule
\multirow{3}{*}{Reddit-12k}&Greedy&&$16$&$_{\pm 3}$&$1.405 _{\pm 0.011}$&$1.367$&$0.038 _{\pm 0.011}$&&$17$&$_{\pm 4}$&$51.78 _{\pm 1.05}$&$50.34$&$1.45 _{\pm 1.05}$\\
&Post-hoc&&$41$ & &$1.585 _{\pm 0.023}$&$1.346$&$0.239 _{\pm 0.023}$&&$64$ & &$55.85 _{\pm 0.97}$&$51.26$&$4.59 _{\pm 0.97}$\\
&$\Delta$&&\textcolor{red!70!black}{$\uparrow 25$}&\textcolor{red!70!black}{$_{\pm 3}$}&\textcolor{red!70!black}{$\uparrow 0.180 _{\pm 0.027}$}&\textcolor{green!70!black}{$\downarrow 0.021$}&--&&\textcolor{red!70!black}{$\uparrow 47$}&\textcolor{red!70!black}{$_{\pm 4}$}&\textcolor{red!70!black}{$\uparrow 4.07 _{\pm 1.59}$}&\textcolor{red!70!black}{$\uparrow 0.92$}&--\\


==> tables/extra/min/err.tex <==
\begin{tabular}{llllllll}
\toprule
 & Raw & Cal & WA & WA+Cal & Ens & Ens+Cal & WA+Cal+Ens \\
\midrule
C10 Aggregate & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
C10 Clean & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
C10 Random1 & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
C10 Random2 & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
C10 Random3 & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
C10 Worst & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
C100-C Clean & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
C100-C Noisy & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
C100-F Clean & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
C100-F Noisy & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
Employment  & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
Income  & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
Mobility  & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
Public Coverage  & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
Travel Time  & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
\bottomrule
\end{tabular}


==> tables/extra/min/nll.tex <==
\begin{tabular}{llllllll}
\toprule
 & Raw & Cal & WA & WA+Cal & Ens & Ens+Cal & WA+Cal+Ens \\
\midrule
C10 Aggregate & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
C10 Clean & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
C10 Random1 & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
C10 Random2 & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
C10 Random3 & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
C10 Worst & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
C100-C Clean & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
C100-C Noisy & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
C100-F Clean & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
C100-F Noisy & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
Employment  & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
Income  & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
Mobility  & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
Public Coverage  & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
Travel Time  & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
\bottomrule
\end{tabular}


==> tables/extra/min_err.tex <==
\begin{tabular}{lllllll}
\toprule
 & Raw & Cal & Ens & WA & WA+Cal & WA+Cal+Ens \\
\midrule
C10 Aggregate & $0.188 \pm 0.002$ & $0.188 \pm 0.001$ & $0.161$ & $0.168 \pm 0.003$ & $0.168 \pm 0.003$ & $0.158$ \\
C10 Clean & $0.094 \pm 0.003$ & $0.094 \pm 0.003$ & $0.078$ & $0.088 \pm 0.003$ & $0.088 \pm 0.003$ & $0.078$ \\
C10 Random1 & $0.286 \pm 0.003$ & $0.283 \pm 0.003$ & $0.240$ & $0.248 \pm 0.001$ & $0.248 \pm 0.002$ & $0.244$ \\
C10 Random2 & $0.292 \pm 0.004$ & $0.287 \pm 0.003$ & $0.248$ & $0.254 \pm 0.003$ & $0.254 \pm 0.002$ & $0.242$ \\
C10 Random3 & $0.285 \pm 0.002$ & $0.281 \pm 0.003$ & $0.241$ & $0.248 \pm 0.002$ & $0.248 \pm 0.002$ & $0.235$ \\
C10 Worst & $0.467 \pm 0.005$ & $0.464 \pm 0.004$ & $0.429$ & $0.440 \pm 0.003$ & $0.496 \pm 0.157$ & $0.488$ \\
C100-C Clean & $0.223 \pm 0.002$ & $0.222 \pm 0.002$ & $0.188$ & $0.204 \pm 0.001$ & $0.204 \pm 0.002$ & $0.182$ \\
C100-C Noisy & $0.391 \pm 0.004$ & $0.389 \pm 0.004$ & $0.333$ & $0.343 \pm 0.003$ & $0.343 \pm 0.004$ & $0.321$ \\
C100-F Clean & $0.337 \pm 0.001$ & $0.339 \pm 0.001$ & $0.292$ & $0.327 \pm 0.003$ & $0.330 \pm 0.005$ & $0.330$ \\
C100-F Noisy & $0.585 \pm 0.004$ & $0.583 \pm 0.004$ & $0.508$ & $0.530 \pm 0.003$ & $0.589 \pm 0.162$ & $0.634$ \\
\bottomrule
\end{tabular}


==> tables/extra/min_nll.tex <==
\begin{tabular}{lllllll}
\toprule
 & Raw & Cal & Ens & WA & WA+Cal & WA+Cal+Ens \\
\midrule
C10 Aggregate & $0.711 \pm 0.019$ & $0.680 \pm 0.006$ & $0.566$ & $0.633 \pm 0.003$ & $0.592 \pm 0.004$ & $2.300$ \\
C10 Clean & $0.414 \pm 0.009$ & $0.311 \pm 0.007$ & $0.252$ & $0.312 \pm 0.008$ & $0.271 \pm 0.005$ & $0.233$ \\
C10 Random1 & $1.015 \pm 0.012$ & $0.996 \pm 0.005$ & $0.884$ & $0.940 \pm 0.005$ & $0.955 \pm 0.121$ & $2.300$ \\
C10 Random2 & $1.034 \pm 0.007$ & $1.016 \pm 0.006$ & $0.907$ & $0.962 \pm 0.004$ & $0.939 \pm 0.004$ & $2.302$ \\
C10 Random3 & $1.007 \pm 0.006$ & $0.991 \pm 0.009$ & $0.876$ & $0.940 \pm 0.004$ & $0.913 \pm 0.004$ & $2.302$ \\
C10 Worst & $1.512 \pm 0.013$ & $1.498 \pm 0.011$ & $1.414$ & $1.462 \pm 0.005$ & $1.556 \pm 0.300$ & $1.585$ \\
C100-C Clean & $0.907 \pm 0.006$ & $0.715 \pm 0.005$ & $0.608$ & $0.708 \pm 0.010$ & $0.628 \pm 0.004$ & $0.554$ \\
C100-C Noisy & $1.238 \pm 0.013$ & $1.222 \pm 0.013$ & $1.042$ & $1.113 \pm 0.006$ & $1.091 \pm 0.006$ & $1.019$ \\
C100-F Clean & $1.506 \pm 0.019$ & $1.362 \pm 0.016$ & $1.141$ & $1.320 \pm 0.013$ & $1.361 \pm 0.417$ & $1.905$ \\
C100-F Noisy & $2.415 \pm 0.020$ & $2.370 \pm 0.019$ & $2.033$ & $2.163 \pm 0.015$ & $2.449 \pm 0.867$ & $2.744$ \\
\bottomrule
\end{tabular}


==> tables/extra/old_main.tex <==
\begin{tabular}{lllllllllllllllllllll}
\toprule
 & \multicolumn{10}{r}{Best Loss} & \multicolumn{10}{r}{Best Error} \\
 & \multicolumn{2}{r}{Epoch} & \multicolumn{2}{r}{Base Loss} & \multicolumn{2}{r}{Final Loss} & \multicolumn{2}{r}{Base Error} & \multicolumn{2}{r}{Final Error} & \multicolumn{2}{r}{Epoch} & \multicolumn{2}{r}{Base Loss} & \multicolumn{2}{r}{Final Loss} & \multicolumn{2}{r}{Base Error} & \multicolumn{2}{r}{Final Error} \\
 & Naive & Post-hoc & Naive & Post-hoc & Naive & Post-hoc & Naive & Post-hoc & Naive & Post-hoc & Naive & Post-hoc & Naive & Post-hoc & Naive & Post-hoc & Naive & Post-hoc & Naive & Post-hoc \\
\midrule
C-10-N Clean & $72_{\pm 35}$ & $101$ & $0.414_{\pm 0.009}$ & $0.423_{\pm 0.014}$ & $0.235$ & $0.229$ & $10.74_{\pm 1.93}$ & $9.51_{\pm 0.24}$ & $7.68$ & $7.56$ & $95_{\pm 4}$ & $100$ & $0.420_{\pm 0.013}$ & $0.422_{\pm 0.015}$ & $0.229$ & $0.229$ & $9.38_{\pm 0.24}$ & $9.53_{\pm 0.27}$ & $7.58$ & $7.56$ \\
C-10-N Aggregate & $11_{\pm 2}$ & $49$ & $0.713_{\pm 0.012}$ & $0.971_{\pm 0.029}$ & $0.589$ & $0.540$ & $21.66_{\pm 0.44}$ & $23.39_{\pm 0.53}$ & $18.00$ & $15.80$ & $93_{\pm 5}$ & $75$ & $1.098_{\pm 0.018}$ & $1.083_{\pm 0.017}$ & $0.549$ & $0.544$ & $19.01_{\pm 0.32}$ & $20.02_{\pm 0.25}$ & $15.58$ & $15.56$ \\
C-10-N Random1 & $12_{\pm 3}$ & $36$ & $1.016_{\pm 0.009}$ & $1.244_{\pm 0.021}$ & $0.890$ & $0.860$ & $28.84_{\pm 0.55}$ & $32.30_{\pm 1.04}$ & $25.06$ & $23.60$ & $34_{\pm 37}$ & $45$ & $1.218_{\pm 0.373}$ & $1.376_{\pm 0.050}$ & $0.867$ & $0.862$ & $28.54_{\pm 0.22}$ & $32.98_{\pm 1.48}$ & $23.92$ & $23.46$ \\
C-10-N Random2 & $10_{\pm 3}$ & $33$ & $1.030_{\pm 0.010}$ & $1.245_{\pm 0.038}$ & $0.921$ & $0.888$ & $29.40_{\pm 0.62}$ & $32.36_{\pm 1.29}$ & $26.16$ & $24.30$ & $24_{\pm 31}$ & $51$ & $1.149_{\pm 0.308}$ & $1.512_{\pm 0.017}$ & $0.904$ & $0.897$ & $29.22_{\pm 0.29}$ & $33.72_{\pm 0.61}$ & $25.26$ & $23.88$ \\
C-10-N Random3 & $9_{\pm 1}$ & $30$ & $1.007_{\pm 0.010}$ & $1.178_{\pm 0.028}$ & $0.899$ & $0.863$ & $29.18_{\pm 0.42}$ & $31.68_{\pm 0.86}$ & $25.96$ & $23.76$ & $25_{\pm 27}$ & $60$ & $1.127_{\pm 0.279}$ & $1.625_{\pm 0.035}$ & $0.871$ & $0.877$ & $28.70_{\pm 0.18}$ & $32.43_{\pm 0.71}$ & $24.40$ & $23.30$ \\
C-10-N Worst & $9_{\pm 2}$ & $27$ & $1.508_{\pm 0.007}$ & $1.678_{\pm 0.018}$ & $1.425$ & $1.398$ & $46.97_{\pm 0.55}$ & $50.44_{\pm 1.29}$ & $44.04$ & $43.16$ & $11_{\pm 3}$ & $34$ & $1.514_{\pm 0.012}$ & $1.809_{\pm 0.036}$ & $1.415$ & $1.400$ & $46.70_{\pm 0.25}$ & $51.22_{\pm 0.52}$ & $43.62$ & $42.88$ \\
C-100-N-Coarse Clean & $35_{\pm 39}$ & $97$ & $1.015_{\pm 0.018}$ & $1.030_{\pm 0.019}$ & $0.656$ & $0.605$ & $28.02_{\pm 3.55}$ & $22.99_{\pm 0.32}$ & $21.44$ & $19.24$ & $94_{\pm 5}$ & $97$ & $1.023_{\pm 0.016}$ & $1.030_{\pm 0.019}$ & $0.605$ & $0.605$ & $22.76_{\pm 0.29}$ & $22.99_{\pm 0.32}$ & $19.32$ & $19.24$ \\
C-100-N-Coarse Noisy & $8_{\pm 1}$ & $37$ & $1.422_{\pm 0.007}$ & $1.857_{\pm 0.091}$ & $1.220$ & $1.152$ & $42.05_{\pm 0.57}$ & $45.86_{\pm 1.97}$ & $36.66$ & $33.58$ & $71_{\pm 38}$ & $35$ & $2.006_{\pm 0.356}$ & $1.837_{\pm 0.028}$ & $1.158$ & $1.152$ & $40.90_{\pm 0.56}$ & $46.34_{\pm 0.80}$ & $33.82$ & $33.54$ \\
C-100-N-Fine Clean & $96_{\pm 4}$ & $68$ & $1.501_{\pm 0.022}$ & $1.603_{\pm 0.025}$ & $1.055$ & $1.052$ & $33.79_{\pm 0.60}$ & $35.33_{\pm 0.38}$ & $29.26$ & $29.58$ & $88_{\pm 7}$ & $100$ & $1.510_{\pm 0.027}$ & $1.513_{\pm 0.021}$ & $1.053$ & $1.055$ & $33.61_{\pm 0.53}$ & $34.04_{\pm 0.48}$ & $29.38$ & $29.26$ \\
C-100-N-Fine Noisy & $8_{\pm 2}$ & $28$ & $2.419_{\pm 0.027}$ & $2.993_{\pm 0.044}$ & $2.083$ & $2.002$ & $59.54_{\pm 1.09}$ & $62.96_{\pm 0.83}$ & $52.96$ & $50.36$ & $81_{\pm 30}$ & $31$ & $3.095_{\pm 0.286}$ & $3.111_{\pm 0.085}$ & $2.059$ & $2.004$ & $58.60_{\pm 0.42}$ & $63.27_{\pm 1.00}$ & $50.62$ & $50.26$ \\
Income  & $6_{\pm 1}$ & $10$ & $0.393_{\pm 0.001}$ & $0.409_{\pm 0.004}$ & $0.386$ & $0.385$ & $17.85_{\pm 0.10}$ & $17.97_{\pm 0.15}$ & $17.70$ & $17.50$ & $7_{\pm 2}$ & $17$ & $0.396_{\pm 0.004}$ & $0.510_{\pm 0.012}$ & $0.385$ & $0.389$ & $17.77_{\pm 0.07}$ & $18.95_{\pm 0.23}$ & $17.72$ & $17.32$ \\
Public Coverage  & $8_{\pm 2}$ & $13$ & $0.543_{\pm 0.001}$ & $0.548_{\pm 0.003}$ & $0.538$ & $0.538$ & $27.42_{\pm 0.20}$ & $27.56_{\pm 0.13}$ & $27.21$ & $27.01$ & $10_{\pm 4}$ & $26$ & $0.545_{\pm 0.002}$ & $0.577_{\pm 0.006}$ & $0.538$ & $0.541$ & $27.27_{\pm 0.10}$ & $28.19_{\pm 0.23}$ & $27.04$ & $26.86$ \\
Mobility  & $9_{\pm 2}$ & $17$ & $0.472_{\pm 0.001}$ & $0.482_{\pm 0.004}$ & $0.469$ & $0.468$ & $21.49_{\pm 0.15}$ & $21.49_{\pm 0.17}$ & $21.25$ & $21.07$ & $13_{\pm 4}$ & $45$ & $0.478_{\pm 0.006}$ & $0.684_{\pm 0.015}$ & $0.468$ & $0.485$ & $21.21_{\pm 0.08}$ & $23.42_{\pm 0.56}$ & $21.19$ & $21.03$ \\
Employment  & $8_{\pm 2}$ & $12$ & $0.380_{\pm 0.000}$ & $0.382_{\pm 0.001}$ & $0.377$ & $0.377$ & $17.89_{\pm 0.10}$ & $17.92_{\pm 0.07}$ & $17.78$ & $17.69$ & $9_{\pm 4}$ & $17$ & $0.381_{\pm 0.001}$ & $0.384_{\pm 0.001}$ & $0.377$ & $0.377$ & $17.78_{\pm 0.05}$ & $18.02_{\pm 0.08}$ & $17.74$ & $17.65$ \\
Travel Time  & $8_{\pm 1}$ & $15$ & $0.597_{\pm 0.001}$ & $0.626_{\pm 0.004}$ & $0.593$ & $0.591$ & $35.56_{\pm 0.20}$ & $36.10_{\pm 0.27}$ & $35.19$ & $35.13$ & $10_{\pm 2}$ & $22$ & $0.603_{\pm 0.007}$ & $0.698_{\pm 0.011}$ & $0.592$ & $0.592$ & $35.42_{\pm 0.20}$ & $37.12_{\pm 0.21}$ & $35.28$ & $35.03$ \\
Collab  & $36_{\pm 6}$ & $132$ & $0.466_{\pm 0.015}$ & $0.883_{\pm 0.101}$ & $0.470$ & $0.405$ & $20.78_{\pm 1.02}$ & $20.10_{\pm 1.59}$ & $22.00$ & $19.60$ & $108_{\pm 71}$ & $258$ & $0.722_{\pm 0.272}$ & $1.568_{\pm 0.137}$ & $0.408$ & $0.415$ & $17.93_{\pm 1.10}$ & $20.90_{\pm 1.31}$ & $19.60$ & $17.60$ \\
Reddit-5k  & $13_{\pm 3}$ & $53$ & $1.099_{\pm 0.010}$ & $1.585_{\pm 0.084}$ & $1.101$ & $1.080$ & $47.04_{\pm 1.28}$ & $51.30_{\pm 1.45}$ & $46.49$ & $45.69$ & $17_{\pm 7}$ & $30$ & $1.124_{\pm 0.026}$ & $1.206_{\pm 0.034}$ & $1.099$ & $1.087$ & $45.47_{\pm 0.75}$ & $49.25_{\pm 1.80}$ & $46.09$ & $45.09$ \\
Reddit-12k  & $13_{\pm 3}$ & $40$ & $1.394_{\pm 0.009}$ & $1.582_{\pm 0.031}$ & $1.366$ & $1.339$ & $51.21_{\pm 0.64}$ & $54.14_{\pm 1.30}$ & $50.34$ & $50.42$ & $18_{\pm 6}$ & $18$ & $1.419_{\pm 0.023}$ & $1.423_{\pm 0.024}$ & $1.356$ & $1.355$ & $50.41_{\pm 0.50}$ & $51.95_{\pm 1.47}$ & $49.92$ & $49.58$ \\
\bottomrule
\end{tabular}


==> tables/extra/test.tex <==
\begin{tabular}{llllllll}
\toprule
 & Raw & Cal & WA & WA+Cal & Ens & Ens+Cal & WA+Cal+Ens \\
\midrule
C10 Aggregate & $0.711 \pm 0.019$ & $0.680 \pm 0.006$ & $0.633 \pm 0.003$ & $0.592 \pm 0.004$ & $0.566$ & $0.559$ & $2.300$ \\
C10 Clean & $0.414 \pm 0.009$ & $0.311 \pm 0.007$ & $0.312 \pm 0.008$ & $0.271 \pm 0.005$ & $0.252$ & $0.240$ & $0.233$ \\
C10 Random1 & $1.015 \pm 0.012$ & $0.996 \pm 0.005$ & $0.940 \pm 0.005$ & $0.955 \pm 0.121$ & $0.884$ & $2.252$ & $2.300$ \\
C10 Random2 & $1.034 \pm 0.007$ & $1.016 \pm 0.006$ & $0.962 \pm 0.004$ & $0.939 \pm 0.004$ & $0.907$ & $2.275$ & $2.302$ \\
C10 Random3 & $1.007 \pm 0.006$ & $0.991 \pm 0.009$ & $0.940 \pm 0.004$ & $0.913 \pm 0.004$ & $0.876$ & $0.873$ & $2.302$ \\
C10 Worst & $1.512 \pm 0.013$ & $1.498 \pm 0.011$ & $1.462 \pm 0.005$ & $1.556 \pm 0.300$ & $1.414$ & $1.414$ & $1.585$ \\
C100-C Clean & $0.907 \pm 0.006$ & $0.715 \pm 0.005$ & $0.708 \pm 0.010$ & $0.628 \pm 0.004$ & $0.608$ & $0.585$ & $0.554$ \\
C100-C Noisy & $1.238 \pm 0.013$ & $1.222 \pm 0.013$ & $1.113 \pm 0.006$ & $1.091 \pm 0.006$ & $1.042$ & $1.044$ & $1.019$ \\
C100-F Clean & $1.506 \pm 0.019$ & $1.362 \pm 0.016$ & $1.320 \pm 0.013$ & $1.361 \pm 0.417$ & $1.141$ & $1.123$ & $1.905$ \\
C100-F Noisy & $2.415 \pm 0.020$ & $2.370 \pm 0.019$ & $2.163 \pm 0.015$ & $2.449 \pm 0.867$ & $2.033$ & $2.040$ & $2.744$ \\
\bottomrule
\end{tabular}


==> tables/extra/training_setup.tex <==
\begin{tabular}{ll}
\toprule
Dataset & CIFAR-10/100-N \\
\midrule
Model & ResNet-18-D \\
Pre-trained & True \\
Optimizer & \makecell[tl]{SGD\\(momentum=0.9)} \\
LR & 0.1 \\
Weight Decay & 5e-4 \\
Scheduler & CosineAnnealing \\
Epochs & 100 \\
Batch Size & 500 \\
Augmentation & \makecell[tl]{RandomCrop\\+ HorizontalFlip} \\
\bottomrule
\end{tabular}


==> tables/loss.tex <==
\multirow{3}{*}{\makecell[l]{C-10-N\\Clean}} & CE & $100$ &  & $0.433 _{\pm 0.009}$ & $0.233$ & $96$ &  & $9.82 _{\pm 0.27}$ & $8.24$\\
 & SOP & $100$ &  & $0.430 _{\pm 0.008}$ & $0.235$ & $88$ &  & $9.71 _{\pm 0.20}$ & $8.00$\\
 & ELR & $100$ &  & $0.422 _{\pm 0.012}$ & $0.232$ & $100$ &  & $9.44 _{\pm 0.22}$ & $7.92$\\
\midrule
\multirow{3}{*}{\makecell[l]{C-10-N\\Aggregate}} & CE & $53$ &  & $0.977 _{\pm 0.030}$ & $0.543$ & $58$ &  & $22.21 _{\pm 0.62}$ & $15.74$\\
 & SOP & $94$ &  & $1.084 _{\pm 0.017}$ & $0.541$ & $98$ &  & $17.86 _{\pm 0.23}$ & $15.56$\\
 & ELR & $50$ &  & $0.938 _{\pm 0.031}$ & $0.541$ & $88$ &  & $19.11 _{\pm 0.30}$ & $15.52$\\
\midrule
\multirow{3}{*}{\makecell[l]{C-10-N\\Random1}} & CE & $31$ &  & $1.189 _{\pm 0.017}$ & $0.859$ & $67$ &  & $31.58 _{\pm 0.51}$ & $23.50$\\
 & SOP & $91$ &  & $1.813 _{\pm 0.022}$ & $0.851$ & $87$ &  & $26.89 _{\pm 0.31}$ & $23.14$\\
 & ELR & $31$ &  & $1.175 _{\pm 0.041}$ & $0.864$ & $91$ &  & $29.59 _{\pm 0.46}$ & $23.56$\\
\midrule
\multirow{3}{*}{\makecell[l]{C-10-N\\Random2}} & CE & $30$ &  & $1.189 _{\pm 0.037}$ & $0.888$ & $74$ &  & $31.15 _{\pm 0.38}$ & $24.12$\\
 & SOP & $77$ &  & $1.877 _{\pm 0.029}$ & $0.883$ & $97$ &  & $27.33 _{\pm 0.27}$ & $24.16$\\
 & ELR & $31$ &  & $1.217 _{\pm 0.024}$ & $0.893$ & $54$ &  & $33.34 _{\pm 0.47}$ & $24.50$\\
\midrule
\multirow{3}{*}{\makecell[l]{C-10-N\\Random3}} & CE & $32$ &  & $1.179 _{\pm 0.027}$ & $0.864$ & $38$ &  & $32.39 _{\pm 0.68}$ & $23.44$\\
 & SOP & $98$ &  & $1.787 _{\pm 0.014}$ & $0.851$ & $55$ &  & $29.04 _{\pm 0.68}$ & $22.96$\\
 & ELR & $32$ &  & $1.187 _{\pm 0.038}$ & $0.866$ & $56$ &  & $32.63 _{\pm 0.55}$ & $23.32$\\
\midrule
\multirow{3}{*}{\makecell[l]{C-10-N\\Worst}} & CE & $25$ &  & $1.643 _{\pm 0.019}$ & $1.399$ & $24$ &  & $49.67 _{\pm 0.74}$ & $42.88$\\
 & SOP & $20$ &  & $1.733 _{\pm 0.022}$ & $1.413$ & $39$ &  & $50.48 _{\pm 0.87}$ & $42.78$\\
 & ELR & $26$ &  & $1.685 _{\pm 0.031}$ & $1.397$ & $34$ &  & $51.50 _{\pm 0.63}$ & $42.48$\\
\midrule
\midrule
\multirow{3}{*}{\makecell[l]{C-100-N-C\\Clean}} & CE & $100$ &  & $1.040 _{\pm 0.019}$ & $0.606$ & $72$ &  & $24.39 _{\pm 0.43}$ & $19.52$\\
 & SOP & $100$ &  & $1.039 _{\pm 0.026}$ & $0.608$ & $65$ &  & $25.40 _{\pm 0.66}$ & $19.78$\\
 & ELR & $100$ &  & $1.039 _{\pm 0.011}$ & $0.605$ & $93$ &  & $23.11 _{\pm 0.23}$ & $19.24$\\
\midrule
\multirow{3}{*}{\makecell[l]{C-100-N-C\\Noisy}} & CE & $32$ &  & $1.744 _{\pm 0.049}$ & $1.150$ & $38$ &  & $45.45 _{\pm 0.98}$ & $33.54$\\
 & SOP & $32$ &  & $1.740 _{\pm 0.035}$ & $1.145$ & $28$ &  & $44.31 _{\pm 0.82}$ & $33.94$\\
 & ELR & $32$ &  & $1.794 _{\pm 0.040}$ & $1.152$ & $51$ &  & $44.95 _{\pm 0.69}$ & $33.60$\\
\midrule
\midrule
\multirow{3}{*}{\makecell[l]{C-100-N-F\\Clean}} & CE & $75$ &  & $1.567 _{\pm 0.019}$ & $1.063$ & $95$ &  & $33.86 _{\pm 0.53}$ & $29.94$\\
 & SOP & $71$ &  & $1.597 _{\pm 0.028}$ & $1.061$ & $97$ &  & $33.73 _{\pm 0.37}$ & $29.56$\\
 & ELR & $69$ &  & $1.624 _{\pm 0.013}$ & $1.068$ & $87$ &  & $34.34 _{\pm 0.26}$ & $29.66$\\
\midrule
\multirow{3}{*}{\makecell[l]{C-100-N-F\\Noisy}} & CE & $27$ &  & $3.015 _{\pm 0.079}$ & $1.994$ & $32$ &  & $63.53 _{\pm 0.55}$ & $50.26$\\
 & SOP & $29$ &  & $3.051 _{\pm 0.053}$ & $1.997$ & $31$ &  & $62.72 _{\pm 0.62}$ & $50.54$\\
 & ELR & $25$ &  & $2.903 _{\pm 0.077}$ & $1.997$ & $29$ &  & $63.73 _{\pm 0.82}$ & $50.50$\\
\midrule


==> tables/main.tex <==
\multirow{3}{*}{\makecell[l]{C-10-N\\Clean}} & Naive & $90$ & $_{\pm 9}$ & $0.435 _{\pm 0.012}$ & $0.234$ & \textcolor{green!70!black}{$-$ $0.201 _{\pm 0.012}$} & $92$ & $_{\pm 5}$ & $9.75 _{\pm 0.24}$ & $8.30$ & \textcolor{green!70!black}{$-$ $1.45 _{\pm 0.24}$}\\
 & Post-hoc & $100$ &  & $0.433 _{\pm 0.009}$ & $0.233$ & \textcolor{green!70!black}{$-$ $0.200 _{\pm 0.009}$} & $96$ &  & $9.82 _{\pm 0.27}$ & $8.24$ & \textcolor{green!70!black}{$-$ $1.58 _{\pm 0.27}$}\\
 & $\Delta$ & $+$ $10$ & $_{\pm 9}$ & \textcolor{green!70!black}{$-$ $0.001 _{\pm 0.005}$} & \textcolor{green!70!black}{$-$ $0.001$} &  & $+$ $4$ & $_{\pm 5}$ & \textcolor{red!70!black}{$+$ $0.07 _{\pm 0.10}$} & \textcolor{green!70!black}{$-$ $0.06$} & \\
\midrule
\multirow{3}{*}{\makecell[l]{C-10-N\\Aggregate}} & Naive & $10$ & $_{\pm 3}$ & $0.722 _{\pm 0.018}$ & $0.608$ & \textcolor{green!70!black}{$-$ $0.114 _{\pm 0.018}$} & $94$ & $_{\pm 6}$ & $19.20 _{\pm 0.39}$ & $15.88$ & \textcolor{green!70!black}{$-$ $3.33 _{\pm 0.39}$}\\
 & Post-hoc & $53$ &  & $0.977 _{\pm 0.030}$ & $0.543$ & \textcolor{green!70!black}{$-$ $0.434 _{\pm 0.030}$} & $58$ &  & $22.21 _{\pm 0.62}$ & $15.74$ & \textcolor{green!70!black}{$-$ $6.47 _{\pm 0.62}$}\\
 & $\Delta$ & $+$ $43$ & $_{\pm 3}$ & \textcolor{red!70!black}{$+$ $0.255 _{\pm 0.027}$} & \textcolor{green!70!black}{$-$ $0.065$} &  & $-$ $36$ & $_{\pm 6}$ & \textcolor{red!70!black}{$+$ $3.00 _{\pm 0.73}$} & \textcolor{green!70!black}{$-$ $0.14$} & \\
\midrule
\multirow{3}{*}{\makecell[l]{C-10-N\\Random1}} & Naive & $8$ & $_{\pm 2}$ & $1.009 _{\pm 0.008}$ & $0.916$ & \textcolor{green!70!black}{$-$ $0.093 _{\pm 0.008}$} & $22$ & $_{\pm 32}$ & $28.63 _{\pm 0.57}$ & $24.80$ & \textcolor{green!70!black}{$-$ $3.83 _{\pm 0.57}$}\\
 & Post-hoc & $31$ &  & $1.189 _{\pm 0.017}$ & $0.859$ & \textcolor{green!70!black}{$-$ $0.330 _{\pm 0.017}$} & $67$ &  & $31.58 _{\pm 0.51}$ & $23.50$ & \textcolor{green!70!black}{$-$ $8.08 _{\pm 0.51}$}\\
 & $\Delta$ & $+$ $23$ & $_{\pm 2}$ & \textcolor{red!70!black}{$+$ $0.181 _{\pm 0.018}$} & \textcolor{green!70!black}{$-$ $0.057$} &  & $+$ $44$ & $_{\pm 32}$ & \textcolor{red!70!black}{$+$ $2.95 _{\pm 0.95}$} & \textcolor{green!70!black}{$-$ $1.30$} & \\
\midrule
\multirow{3}{*}{\makecell[l]{C-10-N\\Random2}} & Naive & $10$ & $_{\pm 1}$ & $1.040 _{\pm 0.008}$ & $0.931$ & \textcolor{green!70!black}{$-$ $0.108 _{\pm 0.008}$} & $14$ & $_{\pm 6}$ & $29.90 _{\pm 0.42}$ & $25.44$ & \textcolor{green!70!black}{$-$ $4.47 _{\pm 0.42}$}\\
 & Post-hoc & $30$ &  & $1.189 _{\pm 0.037}$ & $0.888$ & \textcolor{green!70!black}{$-$ $0.301 _{\pm 0.037}$} & $74$ &  & $31.15 _{\pm 0.38}$ & $24.12$ & \textcolor{green!70!black}{$-$ $7.02 _{\pm 0.38}$}\\
 & $\Delta$ & $+$ $20$ & $_{\pm 1}$ & \textcolor{red!70!black}{$+$ $0.150 _{\pm 0.038}$} & \textcolor{green!70!black}{$-$ $0.043$} &  & $+$ $60$ & $_{\pm 6}$ & \textcolor{red!70!black}{$+$ $1.24 _{\pm 0.56}$} & \textcolor{green!70!black}{$-$ $1.32$} & \\
\midrule
\multirow{3}{*}{\makecell[l]{C-10-N\\Random3}} & Naive & $9$ & $_{\pm 2}$ & $1.005 _{\pm 0.014}$ & $0.910$ & \textcolor{green!70!black}{$-$ $0.095 _{\pm 0.014}$} & $24$ & $_{\pm 30}$ & $28.96 _{\pm 0.65}$ & $24.86$ & \textcolor{green!70!black}{$-$ $4.10 _{\pm 0.65}$}\\
 & Post-hoc & $32$ &  & $1.179 _{\pm 0.027}$ & $0.864$ & \textcolor{green!70!black}{$-$ $0.315 _{\pm 0.027}$} & $38$ &  & $32.39 _{\pm 0.68}$ & $23.44$ & \textcolor{green!70!black}{$-$ $8.95 _{\pm 0.68}$}\\
 & $\Delta$ & $+$ $23$ & $_{\pm 2}$ & \textcolor{red!70!black}{$+$ $0.174 _{\pm 0.031}$} & \textcolor{green!70!black}{$-$ $0.046$} &  & $+$ $14$ & $_{\pm 30}$ & \textcolor{red!70!black}{$+$ $3.43 _{\pm 1.03}$} & \textcolor{green!70!black}{$-$ $1.42$} & \\
\midrule
\multirow{3}{*}{\makecell[l]{C-10-N\\Worst}} & Naive & $8$ & $_{\pm 2}$ & $1.511 _{\pm 0.008}$ & $1.437$ & \textcolor{green!70!black}{$-$ $0.073 _{\pm 0.008}$} & $10$ & $_{\pm 3}$ & $46.84 _{\pm 0.56}$ & $44.30$ & \textcolor{green!70!black}{$-$ $2.54 _{\pm 0.56}$}\\
 & Post-hoc & $25$ &  & $1.643 _{\pm 0.019}$ & $1.399$ & \textcolor{green!70!black}{$-$ $0.245 _{\pm 0.019}$} & $24$ &  & $49.67 _{\pm 0.74}$ & $42.88$ & \textcolor{green!70!black}{$-$ $6.79 _{\pm 0.74}$}\\
 & $\Delta$ & $+$ $17$ & $_{\pm 2}$ & \textcolor{red!70!black}{$+$ $0.133 _{\pm 0.018}$} & \textcolor{green!70!black}{$-$ $0.039$} &  & $+$ $14$ & $_{\pm 3}$ & \textcolor{red!70!black}{$+$ $2.83 _{\pm 0.94}$} & \textcolor{green!70!black}{$-$ $1.42$} & \\
\midrule
\midrule
\multirow{3}{*}{\makecell[l]{C-100-N-C\\Clean}} & Naive & $33$ & $_{\pm 35}$ & $1.011 _{\pm 0.014}$ & $0.669$ & \textcolor{green!70!black}{$-$ $0.342 _{\pm 0.014}$} & $91$ & $_{\pm 4}$ & $23.12 _{\pm 0.40}$ & $19.36$ & \textcolor{green!70!black}{$-$ $3.76 _{\pm 0.40}$}\\
 & Post-hoc & $100$ &  & $1.040 _{\pm 0.019}$ & $0.606$ & \textcolor{green!70!black}{$-$ $0.435 _{\pm 0.019}$} & $72$ &  & $24.39 _{\pm 0.43}$ & $19.52$ & \textcolor{green!70!black}{$-$ $4.87 _{\pm 0.43}$}\\
 & $\Delta$ & $+$ $67$ & $_{\pm 35}$ & \textcolor{red!70!black}{$+$ $0.029 _{\pm 0.023}$} & \textcolor{green!70!black}{$-$ $0.063$} &  & $-$ $19$ & $_{\pm 4}$ & \textcolor{red!70!black}{$+$ $1.27 _{\pm 0.26}$} & \textcolor{red!70!black}{$+$ $0.16$} & \\
\midrule
\multirow{3}{*}{\makecell[l]{C-100-N-C\\Noisy}} & Naive & $8$ & $_{\pm 2}$ & $1.431 _{\pm 0.008}$ & $1.234$ & \textcolor{green!70!black}{$-$ $0.198 _{\pm 0.008}$} & $40$ & $_{\pm 41}$ & $41.42 _{\pm 0.45}$ & $34.42$ & \textcolor{green!70!black}{$-$ $7.00 _{\pm 0.45}$}\\
 & Post-hoc & $32$ &  & $1.744 _{\pm 0.049}$ & $1.150$ & \textcolor{green!70!black}{$-$ $0.594 _{\pm 0.049}$} & $38$ &  & $45.45 _{\pm 0.98}$ & $33.54$ & \textcolor{green!70!black}{$-$ $11.91 _{\pm 0.98}$}\\
 & $\Delta$ & $+$ $24$ & $_{\pm 2}$ & \textcolor{red!70!black}{$+$ $0.313 _{\pm 0.048}$} & \textcolor{green!70!black}{$-$ $0.084$} &  & $-$ $2$ & $_{\pm 41}$ & \textcolor{red!70!black}{$+$ $4.03 _{\pm 1.13}$} & \textcolor{green!70!black}{$-$ $0.88$} & \\
\midrule
\midrule
\multirow{3}{*}{\makecell[l]{C-100-N-F\\Clean}} & Naive & $93$ & $_{\pm 5}$ & $1.508 _{\pm 0.017}$ & $1.065$ & \textcolor{green!70!black}{$-$ $0.443 _{\pm 0.017}$} & $88$ & $_{\pm 5}$ & $33.83 _{\pm 0.37}$ & $29.90$ & \textcolor{green!70!black}{$-$ $3.93 _{\pm 0.37}$}\\
 & Post-hoc & $75$ &  & $1.567 _{\pm 0.019}$ & $1.063$ & \textcolor{green!70!black}{$-$ $0.504 _{\pm 0.019}$} & $95$ &  & $33.86 _{\pm 0.53}$ & $29.94$ & \textcolor{green!70!black}{$-$ $3.92 _{\pm 0.53}$}\\
 & $\Delta$ & $-$ $18$ & $_{\pm 5}$ & \textcolor{red!70!black}{$+$ $0.059 _{\pm 0.014}$} & \textcolor{green!70!black}{$-$ $0.002$} &  & $+$ $7$ & $_{\pm 5}$ & \textcolor{red!70!black}{$+$ $0.03 _{\pm 0.31}$} & \textcolor{red!70!black}{$+$ $0.04$} & \\
\midrule
\multirow{3}{*}{\makecell[l]{C-100-N-F\\Noisy}} & Naive & $7$ & $_{\pm 2}$ & $2.416 _{\pm 0.022}$ & $2.129$ & \textcolor{green!70!black}{$-$ $0.287 _{\pm 0.022}$} & $91$ & $_{\pm 7}$ & $58.68 _{\pm 0.49}$ & $51.34$ & \textcolor{green!70!black}{$-$ $7.34 _{\pm 0.49}$}\\
 & Post-hoc & $27$ &  & $3.015 _{\pm 0.079}$ & $1.994$ & \textcolor{green!70!black}{$-$ $1.021 _{\pm 0.079}$} & $32$ &  & $63.53 _{\pm 0.55}$ & $50.26$ & \textcolor{green!70!black}{$-$ $13.27 _{\pm 0.55}$}\\
 & $\Delta$ & $+$ $20$ & $_{\pm 2}$ & \textcolor{red!70!black}{$+$ $0.598 _{\pm 0.075}$} & \textcolor{green!70!black}{$-$ $0.135$} &  & $-$ $59$ & $_{\pm 7}$ & \textcolor{red!70!black}{$+$ $4.85 _{\pm 0.60}$} & \textcolor{green!70!black}{$-$ $1.08$} & \\
\midrule
\midrule
\multirow{3}{*}{Income} & Naive & $5$ & $_{\pm 1}$ & $0.393 _{\pm 0.001}$ & $0.388$ & \textcolor{green!70!black}{$-$ $0.005 _{\pm 0.001}$} & $7$ & $_{\pm 2}$ & $17.84 _{\pm 0.15}$ & $17.62$ & \textcolor{green!70!black}{$-$ $0.22 _{\pm 0.15}$}\\
 & Post-hoc & $11$ &  & $0.421 _{\pm 0.007}$ & $0.385$ & \textcolor{green!70!black}{$-$ $0.036 _{\pm 0.007}$} & $19$ &  & $19.21 _{\pm 0.14}$ & $17.40$ & \textcolor{green!70!black}{$-$ $1.81 _{\pm 0.14}$}\\
 & $\Delta$ & $+$ $6$ & $_{\pm 1}$ & \textcolor{red!70!black}{$+$ $0.028 _{\pm 0.006}$} & \textcolor{green!70!black}{$-$ $0.003$} &  & $+$ $12$ & $_{\pm 2}$ & \textcolor{red!70!black}{$+$ $1.37 _{\pm 0.22}$} & \textcolor{green!70!black}{$-$ $0.22$} & \\
\midrule
\multirow{3}{*}{\makecell[l]{Public\\Coverage}} & Naive & $10$ & $_{\pm 2}$ & $0.544 _{\pm 0.001}$ & $0.538$ & \textcolor{green!70!black}{$-$ $0.006 _{\pm 0.001}$} & $12$ & $_{\pm 3}$ & $27.52 _{\pm 0.24}$ & $27.25$ & \textcolor{green!70!black}{$-$ $0.28 _{\pm 0.24}$}\\
 & Post-hoc & $18$ &  & $0.554 _{\pm 0.002}$ & $0.538$ & \textcolor{green!70!black}{$-$ $0.016 _{\pm 0.002}$} & $22$ &  & $27.96 _{\pm 0.21}$ & $27.02$ & \textcolor{green!70!black}{$-$ $0.94 _{\pm 0.21}$}\\
 & $\Delta$ & $+$ $8$ & $_{\pm 2}$ & \textcolor{red!70!black}{$+$ $0.010 _{\pm 0.002}$} & \textcolor{green!70!black}{$-$ $0.000$} &  & $+$ $10$ & $_{\pm 3}$ & \textcolor{red!70!black}{$+$ $0.44 _{\pm 0.25}$} & \textcolor{green!70!black}{$-$ $0.22$} & \\
\midrule
\multirow{3}{*}{Mobility} & Naive & $6$ & $_{\pm 2}$ & $0.474 _{\pm 0.002}$ & $0.471$ & \textcolor{green!70!black}{$-$ $0.003 _{\pm 0.002}$} & $13$ & $_{\pm 5}$ & $21.43 _{\pm 0.18}$ & $21.17$ & \textcolor{green!70!black}{$-$ $0.26 _{\pm 0.18}$}\\
 & Post-hoc & $14$ &  & $0.476 _{\pm 0.003}$ & $0.468$ & \textcolor{green!70!black}{$-$ $0.008 _{\pm 0.003}$} & $11$ &  & $21.40 _{\pm 0.17}$ & $21.24$ & \textcolor{green!70!black}{$-$ $0.16 _{\pm 0.17}$}\\
 & $\Delta$ & $+$ $8$ & $_{\pm 2}$ & \textcolor{red!70!black}{$+$ $0.002 _{\pm 0.003}$} & \textcolor{green!70!black}{$-$ $0.003$} &  & $-$ $2$ & $_{\pm 5}$ & \textcolor{green!70!black}{$-$ $0.03 _{\pm 0.22}$} & \textcolor{red!70!black}{$+$ $0.07$} & \\
\midrule
\multirow{3}{*}{Employment} & Naive & $8$ & $_{\pm 1}$ & $0.380 _{\pm 0.000}$ & $0.378$ & \textcolor{green!70!black}{$-$ $0.003 _{\pm 0.000}$} & $14$ & $_{\pm 4}$ & $17.94 _{\pm 0.08}$ & $17.72$ & \textcolor{green!70!black}{$-$ $0.22 _{\pm 0.08}$}\\
 & Post-hoc & $15$ &  & $0.383 _{\pm 0.001}$ & $0.377$ & \textcolor{green!70!black}{$-$ $0.006 _{\pm 0.001}$} & $30$ &  & $18.27 _{\pm 0.12}$ & $17.83$ & \textcolor{green!70!black}{$-$ $0.43 _{\pm 0.12}$}\\
 & $\Delta$ & $+$ $7$ & $_{\pm 1}$ & \textcolor{red!70!black}{$+$ $0.003 _{\pm 0.001}$} & \textcolor{green!70!black}{$-$ $0.000$} &  & $+$ $16$ & $_{\pm 4}$ & \textcolor{red!70!black}{$+$ $0.33 _{\pm 0.16}$} & \textcolor{red!70!black}{$+$ $0.11$} & \\
\midrule
\multirow{3}{*}{Travel Time} & Naive & $6$ & $_{\pm 2}$ & $0.597 _{\pm 0.002}$ & $0.596$ & \textcolor{green!70!black}{$-$ $0.001 _{\pm 0.002}$} & $9$ & $_{\pm 1}$ & $35.77 _{\pm 0.34}$ & $35.44$ & \textcolor{green!70!black}{$-$ $0.32 _{\pm 0.34}$}\\
 & Post-hoc & $15$ &  & $0.626 _{\pm 0.003}$ & $0.591$ & \textcolor{green!70!black}{$-$ $0.035 _{\pm 0.003}$} & $16$ &  & $36.40 _{\pm 0.20}$ & $35.23$ & \textcolor{green!70!black}{$-$ $1.17 _{\pm 0.20}$}\\
 & $\Delta$ & $+$ $8$ & $_{\pm 2}$ & \textcolor{red!70!black}{$+$ $0.029 _{\pm 0.003}$} & \textcolor{green!70!black}{$-$ $0.005$} &  & $+$ $7$ & $_{\pm 1}$ & \textcolor{red!70!black}{$+$ $0.64 _{\pm 0.42}$} & \textcolor{green!70!black}{$-$ $0.21$} & \\
\midrule
\midrule
\multirow{3}{*}{FMoW} & Naive & $2$ & $_{\pm 0}$ & $1.583 _{\pm 0.014}$ & $1.494$ & \textcolor{green!70!black}{$-$ $0.089 _{\pm 0.014}$} & $15$ & $_{\pm 19}$ & $43.20 _{\pm 0.46}$ & $37.95$ & \textcolor{green!70!black}{$-$ $5.24 _{\pm 0.46}$}\\
 & Post-hoc & $50$ &  & $2.831 _{\pm 0.053}$ & $1.305$ & \textcolor{green!70!black}{$-$ $1.526 _{\pm 0.053}$} & $48$ &  & $43.18 _{\pm 0.55}$ & $34.93$ & \textcolor{green!70!black}{$-$ $8.24 _{\pm 0.55}$}\\
 & $\Delta$ & $+$ $48$ & $_{\pm 0}$ & \textcolor{red!70!black}{$+$ $1.248 _{\pm 0.062}$} & \textcolor{green!70!black}{$-$ $0.189$} &  & $+$ $33$ & $_{\pm 19}$ & \textcolor{green!70!black}{$-$ $0.02 _{\pm 0.80}$} & \textcolor{green!70!black}{$-$ $3.02$} & \\
\midrule
\midrule
\multirow{3}{*}{Yelp} & Naive & $2$ & $_{\pm 1}$ & $0.908 _{\pm 0.008}$ & $0.841$ & \textcolor{green!70!black}{$-$ $0.067 _{\pm 0.008}$} & $9$ & $_{\pm 8}$ & $39.41 _{\pm 0.76}$ & $36.18$ & \textcolor{green!70!black}{$-$ $3.23 _{\pm 0.76}$}\\
 & Post-hoc & $3$ &  & $0.990 _{\pm 0.044}$ & $0.824$ & \textcolor{green!70!black}{$-$ $0.166 _{\pm 0.044}$} & $3$ &  & $40.28 _{\pm 1.29}$ & $36.14$ & \textcolor{green!70!black}{$-$ $4.14 _{\pm 1.29}$}\\
 & $\Delta$ & $+$ $1$ & $_{\pm 1}$ & \textcolor{red!70!black}{$+$ $0.082 _{\pm 0.040}$} & \textcolor{green!70!black}{$-$ $0.017$} &  & $-$ $6$ & $_{\pm 8}$ & \textcolor{red!70!black}{$+$ $0.87 _{\pm 1.16}$} & \textcolor{green!70!black}{$-$ $0.04$} & \\
\midrule
\midrule
\multirow{3}{*}{Collab} & Naive & $52$ & $_{\pm 18}$ & $0.492 _{\pm 0.044}$ & $0.439$ & \textcolor{green!70!black}{$-$ $0.053 _{\pm 0.044}$} & $75$ & $_{\pm 28}$ & $20.65 _{\pm 1.06}$ & $20.40$ & \textcolor{green!70!black}{$-$ $0.25 _{\pm 1.06}$}\\
 & Post-hoc & $163$ &  & $1.075 _{\pm 0.122}$ & $0.404$ & \textcolor{green!70!black}{$-$ $0.671 _{\pm 0.122}$} & $152$ &  & $20.95 _{\pm 1.26}$ & $18.80$ & \textcolor{green!70!black}{$-$ $2.15 _{\pm 1.26}$}\\
 & $\Delta$ & $+$ $111$ & $_{\pm 18}$ & \textcolor{red!70!black}{$+$ $0.583 _{\pm 0.146}$} & \textcolor{green!70!black}{$-$ $0.035$} &  & $+$ $77$ & $_{\pm 28}$ & \textcolor{red!70!black}{$+$ $0.30 _{\pm 1.31}$} & \textcolor{green!70!black}{$-$ $1.60$} & \\
\midrule
\multirow{3}{*}{Reddit-5k} & Naive & $16$ & $_{\pm 3}$ & $1.150 _{\pm 0.020}$ & $1.099$ & \textcolor{green!70!black}{$-$ $0.051 _{\pm 0.020}$} & $13$ & $_{\pm 5}$ & $47.70 _{\pm 0.97}$ & $46.69$ & \textcolor{green!70!black}{$-$ $1.00 _{\pm 0.97}$}\\
 & Post-hoc & $44$ &  & $1.416 _{\pm 0.063}$ & $1.085$ & \textcolor{green!70!black}{$-$ $0.331 _{\pm 0.063}$} & $50$ &  & $50.55 _{\pm 1.69}$ & $45.89$ & \textcolor{green!70!black}{$-$ $4.66 _{\pm 1.69}$}\\
 & $\Delta$ & $+$ $28$ & $_{\pm 3}$ & \textcolor{red!70!black}{$+$ $0.266 _{\pm 0.068}$} & \textcolor{green!70!black}{$-$ $0.014$} &  & $+$ $37$ & $_{\pm 5}$ & \textcolor{red!70!black}{$+$ $2.86 _{\pm 2.39}$} & \textcolor{green!70!black}{$-$ $0.80$} & \\
\midrule
\multirow{3}{*}{Reddit-12k} & Naive & $16$ & $_{\pm 3}$ & $1.405 _{\pm 0.011}$ & $1.367$ & \textcolor{green!70!black}{$-$ $0.038 _{\pm 0.011}$} & $17$ & $_{\pm 4}$ & $51.78 _{\pm 1.05}$ & $50.34$ & \textcolor{green!70!black}{$-$ $1.45 _{\pm 1.05}$}\\
 & Post-hoc & $41$ &  & $1.585 _{\pm 0.023}$ & $1.346$ & \textcolor{green!70!black}{$-$ $0.239 _{\pm 0.023}$} & $64$ &  & $55.85 _{\pm 0.97}$ & $51.26$ & \textcolor{green!70!black}{$-$ $4.59 _{\pm 0.97}$}\\
 & $\Delta$ & $+$ $25$ & $_{\pm 3}$ & \textcolor{red!70!black}{$+$ $0.180 _{\pm 0.027}$} & \textcolor{green!70!black}{$-$ $0.021$} &  & $+$ $47$ & $_{\pm 4}$ & \textcolor{red!70!black}{$+$ $4.07 _{\pm 1.59}$} & \textcolor{red!70!black}{$+$ $0.92$} & \\
\midrule


==> tables/main/all.tex <==
\multirow{3}{*}{\makecell[l]{C-10-N\\Clean}} & Naive & $90$ & $_{\pm 9}$ & $0.435 _{\pm 0.012}$ & $0.234$ & $0.201 _{\pm 0.012}$ & $92$ & $_{\pm 5}$ & $9.75 _{\pm 0.24}$ & $8.30$ & $1.45 _{\pm 0.24}$\\
 & Post-hoc & $100$ &  & $0.433 _{\pm 0.009}$ & $0.233$ & $0.200 _{\pm 0.009}$ & $96$ &  & $9.82 _{\pm 0.27}$ & $8.24$ & $1.58 _{\pm 0.27}$\\
 & Gain & $-10$ & $_{\pm 9}$ & \textcolor{green!70!black}{$0.001 _{\pm 0.005}$} & \textcolor{green!70!black}{$0.001$} &  & $-4$ & $_{\pm 5}$ & \textcolor{red!70!black}{$-0.07 _{\pm 0.10}$} & \textcolor{green!70!black}{$0.06$} & \\
\midrule
\multirow{3}{*}{\makecell[l]{C-10-N\\Aggregate}} & Naive & $10$ & $_{\pm 3}$ & $0.722 _{\pm 0.018}$ & $0.608$ & $0.114 _{\pm 0.018}$ & $94$ & $_{\pm 6}$ & $19.20 _{\pm 0.39}$ & $15.88$ & $3.33 _{\pm 0.39}$\\
 & Post-hoc & $53$ &  & $0.977 _{\pm 0.030}$ & $0.543$ & $0.434 _{\pm 0.030}$ & $58$ &  & $22.21 _{\pm 0.62}$ & $15.74$ & $6.47 _{\pm 0.62}$\\
 & Gain & $-43$ & $_{\pm 3}$ & \textcolor{red!70!black}{$-0.255 _{\pm 0.027}$} & \textcolor{green!70!black}{$0.065$} &  & $36$ & $_{\pm 6}$ & \textcolor{red!70!black}{$-3.00 _{\pm 0.73}$} & \textcolor{green!70!black}{$0.14$} & \\
\midrule
\multirow{3}{*}{\makecell[l]{C-10-N\\Random1}} & Naive & $8$ & $_{\pm 2}$ & $1.009 _{\pm 0.008}$ & $0.916$ & $0.093 _{\pm 0.008}$ & $22$ & $_{\pm 32}$ & $28.63 _{\pm 0.57}$ & $24.80$ & $3.83 _{\pm 0.57}$\\
 & Post-hoc & $31$ &  & $1.189 _{\pm 0.017}$ & $0.859$ & $0.330 _{\pm 0.017}$ & $67$ &  & $31.58 _{\pm 0.51}$ & $23.50$ & $8.08 _{\pm 0.51}$\\
 & Gain & $-23$ & $_{\pm 2}$ & \textcolor{red!70!black}{$-0.181 _{\pm 0.018}$} & \textcolor{green!70!black}{$0.057$} &  & $-44$ & $_{\pm 32}$ & \textcolor{red!70!black}{$-2.95 _{\pm 0.95}$} & \textcolor{green!70!black}{$1.30$} & \\
\midrule
\multirow{3}{*}{\makecell[l]{C-10-N\\Random2}} & Naive & $10$ & $_{\pm 1}$ & $1.040 _{\pm 0.008}$ & $0.931$ & $0.108 _{\pm 0.008}$ & $14$ & $_{\pm 6}$ & $29.90 _{\pm 0.42}$ & $25.44$ & $4.47 _{\pm 0.42}$\\
 & Post-hoc & $30$ &  & $1.189 _{\pm 0.037}$ & $0.888$ & $0.301 _{\pm 0.037}$ & $74$ &  & $31.15 _{\pm 0.38}$ & $24.12$ & $7.02 _{\pm 0.38}$\\
 & Gain & $-20$ & $_{\pm 1}$ & \textcolor{red!70!black}{$-0.150 _{\pm 0.038}$} & \textcolor{green!70!black}{$0.043$} &  & $-60$ & $_{\pm 6}$ & \textcolor{red!70!black}{$-1.24 _{\pm 0.56}$} & \textcolor{green!70!black}{$1.32$} & \\
\midrule
\multirow{3}{*}{\makecell[l]{C-10-N\\Random3}} & Naive & $9$ & $_{\pm 2}$ & $1.005 _{\pm 0.014}$ & $0.910$ & $0.095 _{\pm 0.014}$ & $24$ & $_{\pm 30}$ & $28.96 _{\pm 0.65}$ & $24.86$ & $4.10 _{\pm 0.65}$\\
 & Post-hoc & $32$ &  & $1.179 _{\pm 0.027}$ & $0.864$ & $0.315 _{\pm 0.027}$ & $38$ &  & $32.39 _{\pm 0.68}$ & $23.44$ & $8.95 _{\pm 0.68}$\\
 & Gain & $-23$ & $_{\pm 2}$ & \textcolor{red!70!black}{$-0.174 _{\pm 0.031}$} & \textcolor{green!70!black}{$0.046$} &  & $-14$ & $_{\pm 30}$ & \textcolor{red!70!black}{$-3.43 _{\pm 1.03}$} & \textcolor{green!70!black}{$1.42$} & \\
\midrule
\multirow{3}{*}{\makecell[l]{C-10-N\\Worst}} & Naive & $8$ & $_{\pm 2}$ & $1.511 _{\pm 0.008}$ & $1.437$ & $0.073 _{\pm 0.008}$ & $10$ & $_{\pm 3}$ & $46.84 _{\pm 0.56}$ & $44.30$ & $2.54 _{\pm 0.56}$\\
 & Post-hoc & $25$ &  & $1.643 _{\pm 0.019}$ & $1.399$ & $0.245 _{\pm 0.019}$ & $24$ &  & $49.67 _{\pm 0.74}$ & $42.88$ & $6.79 _{\pm 0.74}$\\
 & Gain & $-17$ & $_{\pm 2}$ & \textcolor{red!70!black}{$-0.133 _{\pm 0.018}$} & \textcolor{green!70!black}{$0.039$} &  & $-14$ & $_{\pm 3}$ & \textcolor{red!70!black}{$-2.83 _{\pm 0.94}$} & \textcolor{green!70!black}{$1.42$} & \\
\midrule
\midrule
\multirow{3}{*}{\makecell[l]{C-100-N-C\\Clean}} & Naive & $33$ & $_{\pm 35}$ & $1.011 _{\pm 0.014}$ & $0.669$ & $0.342 _{\pm 0.014}$ & $91$ & $_{\pm 4}$ & $23.12 _{\pm 0.40}$ & $19.36$ & $3.76 _{\pm 0.40}$\\
 & Post-hoc & $100$ &  & $1.040 _{\pm 0.019}$ & $0.606$ & $0.435 _{\pm 0.019}$ & $72$ &  & $24.39 _{\pm 0.43}$ & $19.52$ & $4.87 _{\pm 0.43}$\\
 & Gain & $-67$ & $_{\pm 35}$ & \textcolor{red!70!black}{$-0.029 _{\pm 0.023}$} & \textcolor{green!70!black}{$0.063$} &  & $19$ & $_{\pm 4}$ & \textcolor{red!70!black}{$-1.27 _{\pm 0.26}$} & \textcolor{red!70!black}{$-0.16$} & \\
\midrule
\multirow{3}{*}{\makecell[l]{C-100-N-C\\Noisy}} & Naive & $8$ & $_{\pm 2}$ & $1.431 _{\pm 0.008}$ & $1.234$ & $0.198 _{\pm 0.008}$ & $40$ & $_{\pm 41}$ & $41.42 _{\pm 0.45}$ & $34.42$ & $7.00 _{\pm 0.45}$\\
 & Post-hoc & $32$ &  & $1.744 _{\pm 0.049}$ & $1.150$ & $0.594 _{\pm 0.049}$ & $38$ &  & $45.45 _{\pm 0.98}$ & $33.54$ & $11.91 _{\pm 0.98}$\\
 & Gain & $-24$ & $_{\pm 2}$ & \textcolor{red!70!black}{$-0.313 _{\pm 0.048}$} & \textcolor{green!70!black}{$0.084$} &  & $2$ & $_{\pm 41}$ & \textcolor{red!70!black}{$-4.03 _{\pm 1.13}$} & \textcolor{green!70!black}{$0.88$} & \\
\midrule
\midrule
\multirow{3}{*}{\makecell[l]{C-100-N-F\\Clean}} & Naive & $93$ & $_{\pm 5}$ & $1.508 _{\pm 0.017}$ & $1.065$ & $0.443 _{\pm 0.017}$ & $88$ & $_{\pm 5}$ & $33.83 _{\pm 0.37}$ & $29.90$ & $3.93 _{\pm 0.37}$\\
 & Post-hoc & $75$ &  & $1.567 _{\pm 0.019}$ & $1.063$ & $0.504 _{\pm 0.019}$ & $95$ &  & $33.86 _{\pm 0.53}$ & $29.94$ & $3.92 _{\pm 0.53}$\\
 & Gain & $18$ & $_{\pm 5}$ & \textcolor{red!70!black}{$-0.059 _{\pm 0.014}$} & \textcolor{green!70!black}{$0.002$} &  & $-7$ & $_{\pm 5}$ & \textcolor{red!70!black}{$-0.03 _{\pm 0.31}$} & \textcolor{red!70!black}{$-0.04$} & \\
\midrule
\multirow{3}{*}{\makecell[l]{C-100-N-F\\Noisy}} & Naive & $7$ & $_{\pm 2}$ & $2.416 _{\pm 0.022}$ & $2.129$ & $0.287 _{\pm 0.022}$ & $91$ & $_{\pm 7}$ & $58.68 _{\pm 0.49}$ & $51.34$ & $7.34 _{\pm 0.49}$\\
 & Post-hoc & $27$ &  & $3.015 _{\pm 0.079}$ & $1.994$ & $1.021 _{\pm 0.079}$ & $32$ &  & $63.53 _{\pm 0.55}$ & $50.26$ & $13.27 _{\pm 0.55}$\\
 & Gain & $-20$ & $_{\pm 2}$ & \textcolor{red!70!black}{$-0.598 _{\pm 0.075}$} & \textcolor{green!70!black}{$0.135$} &  & $59$ & $_{\pm 7}$ & \textcolor{red!70!black}{$-4.85 _{\pm 0.60}$} & \textcolor{green!70!black}{$1.08$} & \\
\midrule
\midrule
\multirow{3}{*}{Income} & Naive & $5$ & $_{\pm 1}$ & $0.393 _{\pm 0.001}$ & $0.388$ & $0.005 _{\pm 0.001}$ & $7$ & $_{\pm 2}$ & $17.84 _{\pm 0.15}$ & $17.62$ & $0.22 _{\pm 0.15}$\\
 & Post-hoc & $11$ &  & $0.421 _{\pm 0.007}$ & $0.385$ & $0.036 _{\pm 0.007}$ & $19$ &  & $19.21 _{\pm 0.14}$ & $17.40$ & $1.81 _{\pm 0.14}$\\
 & Gain & $-6$ & $_{\pm 1}$ & \textcolor{red!70!black}{$-0.028 _{\pm 0.006}$} & \textcolor{green!70!black}{$0.003$} &  & $-12$ & $_{\pm 2}$ & \textcolor{red!70!black}{$-1.37 _{\pm 0.22}$} & \textcolor{green!70!black}{$0.22$} & \\
\midrule
\multirow{3}{*}{\makecell[l]{Public\\Coverage}} & Naive & $10$ & $_{\pm 2}$ & $0.544 _{\pm 0.001}$ & $0.538$ & $0.006 _{\pm 0.001}$ & $12$ & $_{\pm 3}$ & $27.52 _{\pm 0.24}$ & $27.25$ & $0.28 _{\pm 0.24}$\\
 & Post-hoc & $18$ &  & $0.554 _{\pm 0.002}$ & $0.538$ & $0.016 _{\pm 0.002}$ & $22$ &  & $27.96 _{\pm 0.21}$ & $27.02$ & $0.94 _{\pm 0.21}$\\
 & Gain & $-8$ & $_{\pm 2}$ & \textcolor{red!70!black}{$-0.010 _{\pm 0.002}$} & \textcolor{green!70!black}{$0.000$} &  & $-10$ & $_{\pm 3}$ & \textcolor{red!70!black}{$-0.44 _{\pm 0.25}$} & \textcolor{green!70!black}{$0.22$} & \\
\midrule
\multirow{3}{*}{Mobility} & Naive & $6$ & $_{\pm 2}$ & $0.474 _{\pm 0.002}$ & $0.471$ & $0.003 _{\pm 0.002}$ & $13$ & $_{\pm 5}$ & $21.43 _{\pm 0.18}$ & $21.17$ & $0.26 _{\pm 0.18}$\\
 & Post-hoc & $14$ &  & $0.476 _{\pm 0.003}$ & $0.468$ & $0.008 _{\pm 0.003}$ & $11$ &  & $21.40 _{\pm 0.17}$ & $21.24$ & $0.16 _{\pm 0.17}$\\
 & Gain & $-8$ & $_{\pm 2}$ & \textcolor{red!70!black}{$-0.002 _{\pm 0.003}$} & \textcolor{green!70!black}{$0.003$} &  & $2$ & $_{\pm 5}$ & \textcolor{green!70!black}{$0.03 _{\pm 0.22}$} & \textcolor{red!70!black}{$-0.07$} & \\
\midrule
\multirow{3}{*}{Employment} & Naive & $8$ & $_{\pm 1}$ & $0.380 _{\pm 0.000}$ & $0.378$ & $0.003 _{\pm 0.000}$ & $14$ & $_{\pm 4}$ & $17.94 _{\pm 0.08}$ & $17.72$ & $0.22 _{\pm 0.08}$\\
 & Post-hoc & $15$ &  & $0.383 _{\pm 0.001}$ & $0.377$ & $0.006 _{\pm 0.001}$ & $30$ &  & $18.27 _{\pm 0.12}$ & $17.83$ & $0.43 _{\pm 0.12}$\\
 & Gain & $-7$ & $_{\pm 1}$ & \textcolor{red!70!black}{$-0.003 _{\pm 0.001}$} & \textcolor{green!70!black}{$0.000$} &  & $-16$ & $_{\pm 4}$ & \textcolor{red!70!black}{$-0.33 _{\pm 0.16}$} & \textcolor{red!70!black}{$-0.11$} & \\
\midrule
\multirow{3}{*}{Travel Time} & Naive & $6$ & $_{\pm 2}$ & $0.597 _{\pm 0.002}$ & $0.596$ & $0.001 _{\pm 0.002}$ & $9$ & $_{\pm 1}$ & $35.77 _{\pm 0.34}$ & $35.44$ & $0.32 _{\pm 0.34}$\\
 & Post-hoc & $15$ &  & $0.626 _{\pm 0.003}$ & $0.591$ & $0.035 _{\pm 0.003}$ & $16$ &  & $36.40 _{\pm 0.20}$ & $35.23$ & $1.17 _{\pm 0.20}$\\
 & Gain & $-8$ & $_{\pm 2}$ & \textcolor{red!70!black}{$-0.029 _{\pm 0.003}$} & \textcolor{green!70!black}{$0.005$} &  & $-7$ & $_{\pm 1}$ & \textcolor{red!70!black}{$-0.64 _{\pm 0.42}$} & \textcolor{green!70!black}{$0.21$} & \\
\midrule
\midrule
\multirow{3}{*}{FMoW} & Naive & $2$ & $_{\pm 0}$ & $1.583 _{\pm 0.014}$ & $1.494$ & $0.089 _{\pm 0.014}$ & $15$ & $_{\pm 19}$ & $43.20 _{\pm 0.46}$ & $37.95$ & $5.24 _{\pm 0.46}$\\
 & Post-hoc & $50$ &  & $2.831 _{\pm 0.053}$ & $1.305$ & $1.526 _{\pm 0.053}$ & $48$ &  & $43.18 _{\pm 0.55}$ & $34.93$ & $8.24 _{\pm 0.55}$\\
 & Gain & $-48$ & $_{\pm 0}$ & \textcolor{red!70!black}{$-1.248 _{\pm 0.062}$} & \textcolor{green!70!black}{$0.189$} &  & $-33$ & $_{\pm 19}$ & \textcolor{green!70!black}{$0.02 _{\pm 0.80}$} & \textcolor{green!70!black}{$3.02$} & \\
\midrule
\midrule
\multirow{3}{*}{Yelp} & Naive & $2$ & $_{\pm 1}$ & $0.908 _{\pm 0.008}$ & $0.841$ & $0.067 _{\pm 0.008}$ & $9$ & $_{\pm 8}$ & $39.41 _{\pm 0.76}$ & $36.18$ & $3.23 _{\pm 0.76}$\\
 & Post-hoc & $3$ &  & $0.990 _{\pm 0.044}$ & $0.824$ & $0.166 _{\pm 0.044}$ & $3$ &  & $40.28 _{\pm 1.29}$ & $36.14$ & $4.14 _{\pm 1.29}$\\
 & Gain & $-1$ & $_{\pm 1}$ & \textcolor{red!70!black}{$-0.082 _{\pm 0.040}$} & \textcolor{green!70!black}{$0.017$} &  & $6$ & $_{\pm 8}$ & \textcolor{red!70!black}{$-0.87 _{\pm 1.16}$} & \textcolor{green!70!black}{$0.04$} & \\
\midrule
\midrule
\multirow{3}{*}{Collab} & Naive & $52$ & $_{\pm 18}$ & $0.492 _{\pm 0.044}$ & $0.439$ & $0.053 _{\pm 0.044}$ & $75$ & $_{\pm 28}$ & $20.65 _{\pm 1.06}$ & $20.40$ & $0.25 _{\pm 1.06}$\\
 & Post-hoc & $163$ &  & $1.075 _{\pm 0.122}$ & $0.404$ & $0.671 _{\pm 0.122}$ & $152$ &  & $20.95 _{\pm 1.26}$ & $18.80$ & $2.15 _{\pm 1.26}$\\
 & Gain & $-111$ & $_{\pm 18}$ & \textcolor{red!70!black}{$-0.583 _{\pm 0.146}$} & \textcolor{green!70!black}{$0.035$} &  & $-77$ & $_{\pm 28}$ & \textcolor{red!70!black}{$-0.30 _{\pm 1.31}$} & \textcolor{green!70!black}{$1.60$} & \\
\midrule
\multirow{3}{*}{Reddit-5k} & Naive & $16$ & $_{\pm 3}$ & $1.150 _{\pm 0.020}$ & $1.099$ & $0.051 _{\pm 0.020}$ & $13$ & $_{\pm 5}$ & $47.70 _{\pm 0.97}$ & $46.69$ & $1.00 _{\pm 0.97}$\\
 & Post-hoc & $44$ &  & $1.416 _{\pm 0.063}$ & $1.085$ & $0.331 _{\pm 0.063}$ & $50$ &  & $50.55 _{\pm 1.69}$ & $45.89$ & $4.66 _{\pm 1.69}$\\
 & Gain & $-28$ & $_{\pm 3}$ & \textcolor{red!70!black}{$-0.266 _{\pm 0.068}$} & \textcolor{green!70!black}{$0.014$} &  & $-37$ & $_{\pm 5}$ & \textcolor{red!70!black}{$-2.86 _{\pm 2.39}$} & \textcolor{green!70!black}{$0.80$} & \\
\midrule
\multirow{3}{*}{Reddit-12k} & Naive & $16$ & $_{\pm 3}$ & $1.405 _{\pm 0.011}$ & $1.367$ & $0.038 _{\pm 0.011}$ & $17$ & $_{\pm 4}$ & $51.78 _{\pm 1.05}$ & $50.34$ & $1.45 _{\pm 1.05}$\\
 & Post-hoc & $41$ &  & $1.585 _{\pm 0.023}$ & $1.346$ & $0.239 _{\pm 0.023}$ & $64$ &  & $55.85 _{\pm 0.97}$ & $51.26$ & $4.59 _{\pm 0.97}$\\
 & Gain & $-25$ & $_{\pm 3}$ & \textcolor{red!70!black}{$-0.180 _{\pm 0.027}$} & \textcolor{green!70!black}{$0.021$} &  & $-47$ & $_{\pm 4}$ & \textcolor{red!70!black}{$-4.07 _{\pm 1.59}$} & \textcolor{red!70!black}{$-0.92$} & \\
\midrule


==> tables/main/cherry.tex <==
\multirow{3}{*}{\makecell[l]{C-10-N\\Clean}} & Naive & $90$ & $_{\pm 9}$ & $0.435 _{\pm 0.012}$ & $0.234$ & $0.201 _{\pm 0.012}$ & $92$ & $_{\pm 5}$ & $9.75 _{\pm 0.24}$ & $8.30$ & $1.45 _{\pm 0.24}$\\
 & Post-hoc & $100$ &  & $0.433 _{\pm 0.009}$ & $0.233$ & $0.200 _{\pm 0.009}$ & $96$ &  & $9.82 _{\pm 0.27}$ & $8.24$ & $1.58 _{\pm 0.27}$\\
 & Gain & $-10$ & $_{\pm 9}$ & \textcolor{green!70!black}{$0.001 _{\pm 0.005}$} & \textcolor{green!70!black}{$0.001$} &  & $-4$ & $_{\pm 5}$ & \textcolor{red!70!black}{$-0.07 _{\pm 0.10}$} & \textcolor{green!70!black}{$0.06$} & \\
\midrule
\multirow{3}{*}{\makecell[l]{C-10-N\\Aggregate}} & Naive & $10$ & $_{\pm 3}$ & $0.722 _{\pm 0.018}$ & $0.608$ & $0.114 _{\pm 0.018}$ & $94$ & $_{\pm 6}$ & $19.20 _{\pm 0.39}$ & $15.88$ & $3.33 _{\pm 0.39}$\\
 & Post-hoc & $53$ &  & $0.977 _{\pm 0.030}$ & $0.543$ & $0.434 _{\pm 0.030}$ & $58$ &  & $22.21 _{\pm 0.62}$ & $15.74$ & $6.47 _{\pm 0.62}$\\
 & Gain & $-43$ & $_{\pm 3}$ & \textcolor{red!70!black}{$-0.255 _{\pm 0.027}$} & \textcolor{green!70!black}{$0.065$} &  & $36$ & $_{\pm 6}$ & \textcolor{red!70!black}{$-3.00 _{\pm 0.73}$} & \textcolor{green!70!black}{$0.14$} & \\
\midrule
\multirow{3}{*}{\makecell[l]{C-10-N\\Random1}} & Naive & $8$ & $_{\pm 2}$ & $1.009 _{\pm 0.008}$ & $0.916$ & $0.093 _{\pm 0.008}$ & $22$ & $_{\pm 32}$ & $28.63 _{\pm 0.57}$ & $24.80$ & $3.83 _{\pm 0.57}$\\
 & Post-hoc & $31$ &  & $1.189 _{\pm 0.017}$ & $0.859$ & $0.330 _{\pm 0.017}$ & $67$ &  & $31.58 _{\pm 0.51}$ & $23.50$ & $8.08 _{\pm 0.51}$\\
 & Gain & $-23$ & $_{\pm 2}$ & \textcolor{red!70!black}{$-0.181 _{\pm 0.018}$} & \textcolor{green!70!black}{$0.057$} &  & $-44$ & $_{\pm 32}$ & \textcolor{red!70!black}{$-2.95 _{\pm 0.95}$} & \textcolor{green!70!black}{$1.30$} & \\
\midrule
\multirow{3}{*}{\makecell[l]{C-10-N\\Worst}} & Naive & $8$ & $_{\pm 2}$ & $1.511 _{\pm 0.008}$ & $1.437$ & $0.073 _{\pm 0.008}$ & $10$ & $_{\pm 3}$ & $46.84 _{\pm 0.56}$ & $44.30$ & $2.54 _{\pm 0.56}$\\
 & Post-hoc & $25$ &  & $1.643 _{\pm 0.019}$ & $1.399$ & $0.245 _{\pm 0.019}$ & $24$ &  & $49.67 _{\pm 0.74}$ & $42.88$ & $6.79 _{\pm 0.74}$\\
 & Gain & $-17$ & $_{\pm 2}$ & \textcolor{red!70!black}{$-0.133 _{\pm 0.018}$} & \textcolor{green!70!black}{$0.039$} &  & $-14$ & $_{\pm 3}$ & \textcolor{red!70!black}{$-2.83 _{\pm 0.94}$} & \textcolor{green!70!black}{$1.42$} & \\
\midrule
\midrule
\multirow{3}{*}{\makecell[l]{C-100-N-F\\Clean}} & Naive & $93$ & $_{\pm 5}$ & $1.508 _{\pm 0.017}$ & $1.065$ & $0.443 _{\pm 0.017}$ & $88$ & $_{\pm 5}$ & $33.83 _{\pm 0.37}$ & $29.90$ & $3.93 _{\pm 0.37}$\\
 & Post-hoc & $75$ &  & $1.567 _{\pm 0.019}$ & $1.063$ & $0.504 _{\pm 0.019}$ & $95$ &  & $33.86 _{\pm 0.53}$ & $29.94$ & $3.92 _{\pm 0.53}$\\
 & Gain & $18$ & $_{\pm 5}$ & \textcolor{red!70!black}{$-0.059 _{\pm 0.014}$} & \textcolor{green!70!black}{$0.002$} &  & $-7$ & $_{\pm 5}$ & \textcolor{red!70!black}{$-0.03 _{\pm 0.31}$} & \textcolor{red!70!black}{$-0.04$} & \\
\midrule
\multirow{3}{*}{\makecell[l]{C-100-N-F\\Noisy}} & Naive & $7$ & $_{\pm 2}$ & $2.416 _{\pm 0.022}$ & $2.129$ & $0.287 _{\pm 0.022}$ & $91$ & $_{\pm 7}$ & $58.68 _{\pm 0.49}$ & $51.34$ & $7.34 _{\pm 0.49}$\\
 & Post-hoc & $27$ &  & $3.015 _{\pm 0.079}$ & $1.994$ & $1.021 _{\pm 0.079}$ & $32$ &  & $63.53 _{\pm 0.55}$ & $50.26$ & $13.27 _{\pm 0.55}$\\
 & Gain & $-20$ & $_{\pm 2}$ & \textcolor{red!70!black}{$-0.598 _{\pm 0.075}$} & \textcolor{green!70!black}{$0.135$} &  & $59$ & $_{\pm 7}$ & \textcolor{red!70!black}{$-4.85 _{\pm 0.60}$} & \textcolor{green!70!black}{$1.08$} & \\
\midrule
\midrule
\multirow{3}{*}{FMoW} & Naive & $2$ & $_{\pm 0}$ & $1.583 _{\pm 0.014}$ & $1.494$ & $0.089 _{\pm 0.014}$ & $15$ & $_{\pm 19}$ & $43.20 _{\pm 0.46}$ & $37.95$ & $5.24 _{\pm 0.46}$\\
 & Post-hoc & $50$ &  & $2.831 _{\pm 0.053}$ & $1.305$ & $1.526 _{\pm 0.053}$ & $48$ &  & $43.18 _{\pm 0.55}$ & $34.93$ & $8.24 _{\pm 0.55}$\\
 & Gain & $-48$ & $_{\pm 0}$ & \textcolor{red!70!black}{$-1.248 _{\pm 0.062}$} & \textcolor{green!70!black}{$0.189$} &  & $-33$ & $_{\pm 19}$ & \textcolor{green!70!black}{$0.02 _{\pm 0.80}$} & \textcolor{green!70!black}{$3.02$} & \\
\midrule
\midrule
\multirow{3}{*}{Yelp} & Naive & $2$ & $_{\pm 1}$ & $0.908 _{\pm 0.008}$ & $0.841$ & $0.067 _{\pm 0.008}$ & $9$ & $_{\pm 8}$ & $39.41 _{\pm 0.76}$ & $36.18$ & $3.23 _{\pm 0.76}$\\
 & Post-hoc & $3$ &  & $0.990 _{\pm 0.044}$ & $0.824$ & $0.166 _{\pm 0.044}$ & $3$ &  & $40.28 _{\pm 1.29}$ & $36.14$ & $4.14 _{\pm 1.29}$\\
 & Gain & $-1$ & $_{\pm 1}$ & \textcolor{red!70!black}{$-0.082 _{\pm 0.040}$} & \textcolor{green!70!black}{$0.017$} &  & $6$ & $_{\pm 8}$ & \textcolor{red!70!black}{$-0.87 _{\pm 1.16}$} & \textcolor{green!70!black}{$0.04$} & \\
\midrule
\midrule
\multirow{3}{*}{Income} & Naive & $5$ & $_{\pm 1}$ & $0.393 _{\pm 0.001}$ & $0.388$ & $0.005 _{\pm 0.001}$ & $7$ & $_{\pm 2}$ & $17.84 _{\pm 0.15}$ & $17.62$ & $0.22 _{\pm 0.15}$\\
 & Post-hoc & $11$ &  & $0.421 _{\pm 0.007}$ & $0.385$ & $0.036 _{\pm 0.007}$ & $19$ &  & $19.21 _{\pm 0.14}$ & $17.40$ & $1.81 _{\pm 0.14}$\\
 & Gain & $-6$ & $_{\pm 1}$ & \textcolor{red!70!black}{$-0.028 _{\pm 0.006}$} & \textcolor{green!70!black}{$0.003$} &  & $-12$ & $_{\pm 2}$ & \textcolor{red!70!black}{$-1.37 _{\pm 0.22}$} & \textcolor{green!70!black}{$0.22$} & \\
\midrule
\multirow{3}{*}{\makecell[l]{Public\\Coverage}} & Naive & $10$ & $_{\pm 2}$ & $0.544 _{\pm 0.001}$ & $0.538$ & $0.006 _{\pm 0.001}$ & $12$ & $_{\pm 3}$ & $27.52 _{\pm 0.24}$ & $27.25$ & $0.28 _{\pm 0.24}$\\
 & Post-hoc & $18$ &  & $0.554 _{\pm 0.002}$ & $0.538$ & $0.016 _{\pm 0.002}$ & $22$ &  & $27.96 _{\pm 0.21}$ & $27.02$ & $0.94 _{\pm 0.21}$\\
 & Gain & $-8$ & $_{\pm 2}$ & \textcolor{red!70!black}{$-0.010 _{\pm 0.002}$} & \textcolor{green!70!black}{$0.000$} &  & $-10$ & $_{\pm 3}$ & \textcolor{red!70!black}{$-0.44 _{\pm 0.25}$} & \textcolor{green!70!black}{$0.22$} & \\
\midrule
\multirow{3}{*}{Travel Time} & Naive & $6$ & $_{\pm 2}$ & $0.597 _{\pm 0.002}$ & $0.596$ & $0.001 _{\pm 0.002}$ & $9$ & $_{\pm 1}$ & $35.77 _{\pm 0.34}$ & $35.44$ & $0.32 _{\pm 0.34}$\\
 & Post-hoc & $15$ &  & $0.626 _{\pm 0.003}$ & $0.591$ & $0.035 _{\pm 0.003}$ & $16$ &  & $36.40 _{\pm 0.20}$ & $35.23$ & $1.17 _{\pm 0.20}$\\
 & Gain & $-8$ & $_{\pm 2}$ & \textcolor{red!70!black}{$-0.029 _{\pm 0.003}$} & \textcolor{green!70!black}{$0.005$} &  & $-7$ & $_{\pm 1}$ & \textcolor{red!70!black}{$-0.64 _{\pm 0.42}$} & \textcolor{green!70!black}{$0.21$} & \\
\midrule
\midrule
\multirow{3}{*}{Collab} & Naive & $52$ & $_{\pm 18}$ & $0.492 _{\pm 0.044}$ & $0.439$ & $0.053 _{\pm 0.044}$ & $75$ & $_{\pm 28}$ & $20.65 _{\pm 1.06}$ & $20.40$ & $0.25 _{\pm 1.06}$\\
 & Post-hoc & $163$ &  & $1.075 _{\pm 0.122}$ & $0.404$ & $0.671 _{\pm 0.122}$ & $152$ &  & $20.95 _{\pm 1.26}$ & $18.80$ & $2.15 _{\pm 1.26}$\\
 & Gain & $-111$ & $_{\pm 18}$ & \textcolor{red!70!black}{$-0.583 _{\pm 0.146}$} & \textcolor{green!70!black}{$0.035$} &  & $-77$ & $_{\pm 28}$ & \textcolor{red!70!black}{$-0.30 _{\pm 1.31}$} & \textcolor{green!70!black}{$1.60$} & \\
\midrule
\multirow{3}{*}{Reddit-5k} & Naive & $16$ & $_{\pm 3}$ & $1.150 _{\pm 0.020}$ & $1.099$ & $0.051 _{\pm 0.020}$ & $13$ & $_{\pm 5}$ & $47.70 _{\pm 0.97}$ & $46.69$ & $1.00 _{\pm 0.97}$\\
 & Post-hoc & $44$ &  & $1.416 _{\pm 0.063}$ & $1.085$ & $0.331 _{\pm 0.063}$ & $50$ &  & $50.55 _{\pm 1.69}$ & $45.89$ & $4.66 _{\pm 1.69}$\\
 & Gain & $-28$ & $_{\pm 3}$ & \textcolor{red!70!black}{$-0.266 _{\pm 0.068}$} & \textcolor{green!70!black}{$0.014$} &  & $-37$ & $_{\pm 5}$ & \textcolor{red!70!black}{$-2.86 _{\pm 2.39}$} & \textcolor{green!70!black}{$0.80$} & \\
\midrule
\multirow{3}{*}{Reddit-12k} & Naive & $16$ & $_{\pm 3}$ & $1.405 _{\pm 0.011}$ & $1.367$ & $0.038 _{\pm 0.011}$ & $17$ & $_{\pm 4}$ & $51.78 _{\pm 1.05}$ & $50.34$ & $1.45 _{\pm 1.05}$\\
 & Post-hoc & $41$ &  & $1.585 _{\pm 0.023}$ & $1.346$ & $0.239 _{\pm 0.023}$ & $64$ &  & $55.85 _{\pm 0.97}$ & $51.26$ & $4.59 _{\pm 0.97}$\\
 & Gain & $-25$ & $_{\pm 3}$ & \textcolor{red!70!black}{$-0.180 _{\pm 0.027}$} & \textcolor{green!70!black}{$0.021$} &  & $-47$ & $_{\pm 4}$ & \textcolor{red!70!black}{$-4.07 _{\pm 1.59}$} & \textcolor{red!70!black}{$-0.92$} & \\
\midrule


==> tables/main/naive_vs_posthoc/cifar.tex <==
\multirow{3}{*}{\makecell[l]{C-10-N\\Clean}}&Greedy&&$90$&$_{\pm 9}$&$0.435 _{\pm 0.012}$&$0.234$&$0.201 _{\pm 0.012}$&&$92$&$_{\pm 5}$&$9.75 _{\pm 0.24}$&$8.30$&$1.45 _{\pm 0.24}$\\
&Post-hoc&&$100$ & &$0.433 _{\pm 0.009}$&$0.233$&$0.200 _{\pm 0.009}$&&$96$ & &$9.82 _{\pm 0.27}$&$8.24$&$1.58 _{\pm 0.27}$\\
&$\Delta$&&\textcolor{red!70!black}{$\uparrow 10$}&\textcolor{red!70!black}{$_{\pm 9}$}&\textcolor{green!70!black}{$\downarrow 0.001 _{\pm 0.005}$}&\textcolor{green!70!black}{$\downarrow 0.001$}&--&&\textcolor{red!70!black}{$\uparrow 4$}&\textcolor{red!70!black}{$_{\pm 5}$}&\textcolor{red!70!black}{$\uparrow 0.07 _{\pm 0.10}$}&\textcolor{green!70!black}{$\downarrow 0.06$}&--\\
\midrule
\multirow{3}{*}{\makecell[l]{C-10-N\\Aggregate}}&Greedy&&$10$&$_{\pm 3}$&$0.722 _{\pm 0.018}$&$0.608$&$0.114 _{\pm 0.018}$&&$94$&$_{\pm 6}$&$19.20 _{\pm 0.39}$&$15.88$&$3.33 _{\pm 0.39}$\\
&Post-hoc&&$53$ & &$0.977 _{\pm 0.030}$&$0.543$&$0.434 _{\pm 0.030}$&&$58$ & &$22.21 _{\pm 0.62}$&$15.74$&$6.47 _{\pm 0.62}$\\
&$\Delta$&&\textcolor{red!70!black}{$\uparrow 43$}&\textcolor{red!70!black}{$_{\pm 3}$}&\textcolor{red!70!black}{$\uparrow 0.255 _{\pm 0.027}$}&\textcolor{green!70!black}{$\downarrow 0.065$}&--&&\textcolor{green!70!black}{$\downarrow 36$}&\textcolor{green!70!black}{$_{\pm 6}$}&\textcolor{red!70!black}{$\uparrow 3.00 _{\pm 0.73}$}&\textcolor{green!70!black}{$\downarrow 0.14$}&--\\
\midrule
\multirow{3}{*}{\makecell[l]{C-10-N\\Random1}}&Greedy&&$8$&$_{\pm 2}$&$1.009 _{\pm 0.008}$&$0.916$&$0.093 _{\pm 0.008}$&&$22$&$_{\pm 32}$&$28.63 _{\pm 0.57}$&$24.80$&$3.83 _{\pm 0.57}$\\
&Post-hoc&&$31$ & &$1.189 _{\pm 0.017}$&$0.859$&$0.330 _{\pm 0.017}$&&$67$ & &$31.58 _{\pm 0.51}$&$23.50$&$8.08 _{\pm 0.51}$\\
&$\Delta$&&\textcolor{red!70!black}{$\uparrow 23$}&\textcolor{red!70!black}{$_{\pm 2}$}&\textcolor{red!70!black}{$\uparrow 0.181 _{\pm 0.018}$}&\textcolor{green!70!black}{$\downarrow 0.057$}&--&&\textcolor{red!70!black}{$\uparrow 44$}&\textcolor{red!70!black}{$_{\pm 32}$}&\textcolor{red!70!black}{$\uparrow 2.95 _{\pm 0.95}$}&\textcolor{green!70!black}{$\downarrow 1.30$}&--\\
\midrule
\multirow{3}{*}{\makecell[l]{C-10-N\\Worst}}&Greedy&&$8$&$_{\pm 2}$&$1.511 _{\pm 0.008}$&$1.437$&$0.073 _{\pm 0.008}$&&$10$&$_{\pm 3}$&$46.84 _{\pm 0.56}$&$44.30$&$2.54 _{\pm 0.56}$\\
&Post-hoc&&$25$ & &$1.643 _{\pm 0.019}$&$1.399$&$0.245 _{\pm 0.019}$&&$24$ & &$49.67 _{\pm 0.74}$&$42.88$&$6.79 _{\pm 0.74}$\\
&$\Delta$&&\textcolor{red!70!black}{$\uparrow 17$}&\textcolor{red!70!black}{$_{\pm 2}$}&\textcolor{red!70!black}{$\uparrow 0.133 _{\pm 0.018}$}&\textcolor{green!70!black}{$\downarrow 0.039$}&--&&\textcolor{red!70!black}{$\uparrow 14$}&\textcolor{red!70!black}{$_{\pm 3}$}&\textcolor{red!70!black}{$\uparrow 2.83 _{\pm 0.94}$}&\textcolor{green!70!black}{$\downarrow 1.42$}&--\\
\midrule
\midrule
\multirow{3}{*}{\makecell[l]{C-100-N-F\\Clean}}&Greedy&&$93$&$_{\pm 5}$&$1.508 _{\pm 0.017}$&$1.065$&$0.443 _{\pm 0.017}$&&$88$&$_{\pm 5}$&$33.83 _{\pm 0.37}$&$29.90$&$3.93 _{\pm 0.37}$\\
&Post-hoc&&$75$ & &$1.567 _{\pm 0.019}$&$1.063$&$0.504 _{\pm 0.019}$&&$95$ & &$33.86 _{\pm 0.53}$&$29.94$&$3.92 _{\pm 0.53}$\\
&$\Delta$&&\textcolor{green!70!black}{$\downarrow 18$}&\textcolor{green!70!black}{$_{\pm 5}$}&\textcolor{red!70!black}{$\uparrow 0.059 _{\pm 0.014}$}&\textcolor{green!70!black}{$\downarrow 0.002$}&--&&\textcolor{red!70!black}{$\uparrow 7$}&\textcolor{red!70!black}{$_{\pm 5}$}&\textcolor{red!70!black}{$\uparrow 0.03 _{\pm 0.31}$}&\textcolor{red!70!black}{$\uparrow 0.04$}&--\\
\midrule
\multirow{3}{*}{\makecell[l]{C-100-N-F\\Noisy}}&Greedy&&$7$&$_{\pm 2}$&$2.416 _{\pm 0.022}$&$2.129$&$0.287 _{\pm 0.022}$&&$91$&$_{\pm 7}$&$58.68 _{\pm 0.49}$&$51.34$&$7.34 _{\pm 0.49}$\\
&Post-hoc&&$27$ & &$3.015 _{\pm 0.079}$&$1.994$&$1.021 _{\pm 0.079}$&&$32$ & &$63.53 _{\pm 0.55}$&$50.26$&$13.27 _{\pm 0.55}$\\
&$\Delta$&&\textcolor{red!70!black}{$\uparrow 20$}&\textcolor{red!70!black}{$_{\pm 2}$}&\textcolor{red!70!black}{$\uparrow 0.598 _{\pm 0.075}$}&\textcolor{green!70!black}{$\downarrow 0.135$}&--&&\textcolor{green!70!black}{$\downarrow 59$}&\textcolor{green!70!black}{$_{\pm 7}$}&\textcolor{red!70!black}{$\uparrow 4.85 _{\pm 0.60}$}&\textcolor{green!70!black}{$\downarrow 1.08$}&--\\


==> tables/main/naive_vs_posthoc/real.tex <==
\multirow{3}{*}{FMoW}&Greedy&&$2$&$_{\pm 0}$&$1.583 _{\pm 0.014}$&$1.494$&$0.089 _{\pm 0.014}$&&$15$&$_{\pm 19}$&$43.20 _{\pm 0.46}$&$37.95$&$5.24 _{\pm 0.46}$\\
&Post-hoc&&$50$ & &$2.831 _{\pm 0.053}$&$1.305$&$1.526 _{\pm 0.053}$&&$48$ & &$43.18 _{\pm 0.55}$&$34.93$&$8.24 _{\pm 0.55}$\\
&$\Delta$&&\textcolor{red!70!black}{$\uparrow 48$}&\textcolor{red!70!black}{$_{\pm 0}$}&\textcolor{red!70!black}{$\uparrow 1.248 _{\pm 0.062}$}&\textcolor{green!70!black}{$\downarrow 0.189$}&--&&\textcolor{red!70!black}{$\uparrow 33$}&\textcolor{red!70!black}{$_{\pm 19}$}&\textcolor{green!70!black}{$\downarrow 0.02 _{\pm 0.80}$}&\textcolor{green!70!black}{$\downarrow 3.02$}&--\\
\midrule
\multirow{3}{*}{Yelp}&Greedy&&$2$&$_{\pm 1}$&$0.908 _{\pm 0.008}$&$0.841$&$0.067 _{\pm 0.008}$&&$9$&$_{\pm 8}$&$39.41 _{\pm 0.76}$&$36.18$&$3.23 _{\pm 0.76}$\\
&Post-hoc&&$3$ & &$0.990 _{\pm 0.044}$&$0.824$&$0.166 _{\pm 0.044}$&&$3$ & &$40.28 _{\pm 1.29}$&$36.14$&$4.14 _{\pm 1.29}$\\
&$\Delta$&&\textcolor{red!70!black}{$\uparrow 1$}&\textcolor{red!70!black}{$_{\pm 1}$}&\textcolor{red!70!black}{$\uparrow 0.082 _{\pm 0.040}$}&\textcolor{green!70!black}{$\downarrow 0.017$}&--&&\textcolor{green!70!black}{$\downarrow 6$}&\textcolor{green!70!black}{$_{\pm 8}$}&\textcolor{red!70!black}{$\uparrow 0.87 _{\pm 1.16}$}&\textcolor{green!70!black}{$\downarrow 0.04$}&--\\
\midrule
\multirow{3}{*}{Income}&Greedy&&$5$&$_{\pm 1}$&$0.393 _{\pm 0.001}$&$0.388$&$0.005 _{\pm 0.001}$&&$7$&$_{\pm 2}$&$17.84 _{\pm 0.15}$&$17.62$&$0.22 _{\pm 0.15}$\\
&Post-hoc&&$11$ & &$0.421 _{\pm 0.007}$&$0.385$&$0.036 _{\pm 0.007}$&&$19$ & &$19.21 _{\pm 0.14}$&$17.40$&$1.81 _{\pm 0.14}$\\
&$\Delta$&&\textcolor{red!70!black}{$\uparrow 6$}&\textcolor{red!70!black}{$_{\pm 1}$}&\textcolor{red!70!black}{$\uparrow 0.028 _{\pm 0.006}$}&\textcolor{green!70!black}{$\downarrow 0.003$}&--&&\textcolor{red!70!black}{$\uparrow 12$}&\textcolor{red!70!black}{$_{\pm 2}$}&\textcolor{red!70!black}{$\uparrow 1.37 _{\pm 0.22}$}&\textcolor{green!70!black}{$\downarrow 0.22$}&--\\
\midrule
\multirow{3}{*}{\makecell[l]{Public\\Coverage}}&Greedy&&$10$&$_{\pm 2}$&$0.544 _{\pm 0.001}$&$0.538$&$0.006 _{\pm 0.001}$&&$12$&$_{\pm 3}$&$27.52 _{\pm 0.24}$&$27.25$&$0.28 _{\pm 0.24}$\\
&Post-hoc&&$18$ & &$0.554 _{\pm 0.002}$&$0.538$&$0.016 _{\pm 0.002}$&&$22$ & &$27.96 _{\pm 0.21}$&$27.02$&$0.94 _{\pm 0.21}$\\
&$\Delta$&&\textcolor{red!70!black}{$\uparrow 8$}&\textcolor{red!70!black}{$_{\pm 2}$}&\textcolor{red!70!black}{$\uparrow 0.010 _{\pm 0.002}$}&\textcolor{green!70!black}{$\downarrow 0.000$}&--&&\textcolor{red!70!black}{$\uparrow 10$}&\textcolor{red!70!black}{$_{\pm 3}$}&\textcolor{red!70!black}{$\uparrow 0.44 _{\pm 0.25}$}&\textcolor{green!70!black}{$\downarrow 0.22$}&--\\
\midrule
\multirow{3}{*}{\makecell[l]{Travel\\Time}}&Greedy&&$6$&$_{\pm 2}$&$0.597 _{\pm 0.002}$&$0.596$&$0.001 _{\pm 0.002}$&&$9$&$_{\pm 1}$&$35.77 _{\pm 0.34}$&$35.44$&$0.32 _{\pm 0.34}$\\
&Post-hoc&&$15$ & &$0.626 _{\pm 0.003}$&$0.591$&$0.035 _{\pm 0.003}$&&$16$ & &$36.40 _{\pm 0.20}$&$35.23$&$1.17 _{\pm 0.20}$\\
&$\Delta$&&\textcolor{red!70!black}{$\uparrow 8$}&\textcolor{red!70!black}{$_{\pm 2}$}&\textcolor{red!70!black}{$\uparrow 0.029 _{\pm 0.003}$}&\textcolor{green!70!black}{$\downarrow 0.005$}&--&&\textcolor{red!70!black}{$\uparrow 7$}&\textcolor{red!70!black}{$_{\pm 1}$}&\textcolor{red!70!black}{$\uparrow 0.64 _{\pm 0.42}$}&\textcolor{green!70!black}{$\downarrow 0.21$}&--\\
\midrule
\multirow{3}{*}{Collab}&Greedy&&$52$&$_{\pm 18}$&$0.492 _{\pm 0.044}$&$0.439$&$0.053 _{\pm 0.044}$&&$75$&$_{\pm 28}$&$20.65 _{\pm 1.06}$&$20.40$&$0.25 _{\pm 1.06}$\\
&Post-hoc&&$163$ & &$1.075 _{\pm 0.122}$&$0.404$&$0.671 _{\pm 0.122}$&&$152$ & &$20.95 _{\pm 1.26}$&$18.80$&$2.15 _{\pm 1.26}$\\
&$\Delta$&&\textcolor{red!70!black}{$\uparrow 111$}&\textcolor{red!70!black}{$_{\pm 18}$}&\textcolor{red!70!black}{$\uparrow 0.583 _{\pm 0.146}$}&\textcolor{green!70!black}{$\downarrow 0.035$}&--&&\textcolor{red!70!black}{$\uparrow 77$}&\textcolor{red!70!black}{$_{\pm 28}$}&\textcolor{red!70!black}{$\uparrow 0.30 _{\pm 1.31}$}&\textcolor{green!70!black}{$\downarrow 1.60$}&--\\
\midrule
\multirow{3}{*}{Reddit-5k}&Greedy&&$15$&$_{\pm 4}$&$1.154 _{\pm 0.022}$&$1.101$&$0.053 _{\pm 0.022}$&&$13$&$_{\pm 5}$&$47.42 _{\pm 0.64}$&$47.09$&$0.33 _{\pm 0.64}$\\
&Post-hoc&&$44$ & &$1.448 _{\pm 0.058}$&$1.085$&$0.362 _{\pm 0.058}$&&$45$ & &$50.75 _{\pm 1.83}$&$45.49$&$5.26 _{\pm 1.83}$\\
&$\Delta$&&\textcolor{red!70!black}{$\uparrow 29$}&\textcolor{red!70!black}{$_{\pm 4}$}&\textcolor{red!70!black}{$\uparrow 0.294 _{\pm 0.059}$}&\textcolor{green!70!black}{$\downarrow 0.015$}&--&&\textcolor{red!70!black}{$\uparrow 32$}&\textcolor{red!70!black}{$_{\pm 5}$}&\textcolor{red!70!black}{$\uparrow 3.33 _{\pm 2.05}$}&\textcolor{green!70!black}{$\downarrow 1.60$}&--\\
\midrule
\multirow{3}{*}{Reddit-12k}&Greedy&&$16$&$_{\pm 3}$&$1.405 _{\pm 0.011}$&$1.367$&$0.038 _{\pm 0.011}$&&$17$&$_{\pm 4}$&$51.78 _{\pm 1.05}$&$50.34$&$1.45 _{\pm 1.05}$\\
&Post-hoc&&$41$ & &$1.585 _{\pm 0.023}$&$1.346$&$0.239 _{\pm 0.023}$&&$64$ & &$55.85 _{\pm 0.97}$&$51.26$&$4.59 _{\pm 0.97}$\\
&$\Delta$&&\textcolor{red!70!black}{$\uparrow 25$}&\textcolor{red!70!black}{$_{\pm 3}$}&\textcolor{red!70!black}{$\uparrow 0.180 _{\pm 0.027}$}&\textcolor{green!70!black}{$\downarrow 0.021$}&--&&\textcolor{red!70!black}{$\uparrow 47$}&\textcolor{red!70!black}{$_{\pm 4}$}&\textcolor{red!70!black}{$\uparrow 4.07 _{\pm 1.59}$}&\textcolor{red!70!black}{$\uparrow 0.92$}&--\\


==> tables/min/err.tex <==
\begin{tabular}{llllllll}
\toprule
 & Raw & Cal & WA & WA+Cal & Ens & Ens+Cal & WA+Cal+Ens \\
\midrule
C10 Aggregate & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
C10 Clean & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
C10 Random1 & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
C10 Random2 & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
C10 Random3 & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
C10 Worst & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
C100-C Clean & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
C100-C Noisy & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
C100-F Clean & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
C100-F Noisy & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
Employment  & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
Income  & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
Mobility  & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
Public Coverage  & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
Travel Time  & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
\bottomrule
\end{tabular}


==> tables/min/nll.tex <==
\begin{tabular}{llllllll}
\toprule
 & Raw & Cal & WA & WA+Cal & Ens & Ens+Cal & WA+Cal+Ens \\
\midrule
C10 Aggregate & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
C10 Clean & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
C10 Random1 & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
C10 Random2 & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
C10 Random3 & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
C10 Worst & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
C100-C Clean & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
C100-C Noisy & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
C100-F Clean & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
C100-F Noisy & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
Employment  & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
Income  & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
Mobility  & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
Public Coverage  & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
Travel Time  & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan $\pm$ nan & nan & nan & nan \\
\bottomrule
\end{tabular}


==> tables/min_err.tex <==
\begin{tabular}{lllllll}
\toprule
 & Raw & Cal & Ens & WA & WA+Cal & WA+Cal+Ens \\
\midrule
C10 Aggregate & $0.188 \pm 0.002$ & $0.188 \pm 0.001$ & $0.161$ & $0.168 \pm 0.003$ & $0.168 \pm 0.003$ & $0.158$ \\
C10 Clean & $0.094 \pm 0.003$ & $0.094 \pm 0.003$ & $0.078$ & $0.088 \pm 0.003$ & $0.088 \pm 0.003$ & $0.078$ \\
C10 Random1 & $0.286 \pm 0.003$ & $0.283 \pm 0.003$ & $0.240$ & $0.248 \pm 0.001$ & $0.248 \pm 0.002$ & $0.244$ \\
C10 Random2 & $0.292 \pm 0.004$ & $0.287 \pm 0.003$ & $0.248$ & $0.254 \pm 0.003$ & $0.254 \pm 0.002$ & $0.242$ \\
C10 Random3 & $0.285 \pm 0.002$ & $0.281 \pm 0.003$ & $0.241$ & $0.248 \pm 0.002$ & $0.248 \pm 0.002$ & $0.235$ \\
C10 Worst & $0.467 \pm 0.005$ & $0.464 \pm 0.004$ & $0.429$ & $0.440 \pm 0.003$ & $0.496 \pm 0.157$ & $0.488$ \\
C100-C Clean & $0.223 \pm 0.002$ & $0.222 \pm 0.002$ & $0.188$ & $0.204 \pm 0.001$ & $0.204 \pm 0.002$ & $0.182$ \\
C100-C Noisy & $0.391 \pm 0.004$ & $0.389 \pm 0.004$ & $0.333$ & $0.343 \pm 0.003$ & $0.343 \pm 0.004$ & $0.321$ \\
C100-F Clean & $0.337 \pm 0.001$ & $0.339 \pm 0.001$ & $0.292$ & $0.327 \pm 0.003$ & $0.330 \pm 0.005$ & $0.330$ \\
C100-F Noisy & $0.585 \pm 0.004$ & $0.583 \pm 0.004$ & $0.508$ & $0.530 \pm 0.003$ & $0.589 \pm 0.162$ & $0.634$ \\
\bottomrule
\end{tabular}


==> tables/min_nll.tex <==
\begin{tabular}{lllllll}
\toprule
 & Raw & Cal & Ens & WA & WA+Cal & WA+Cal+Ens \\
\midrule
C10 Aggregate & $0.711 \pm 0.019$ & $0.680 \pm 0.006$ & $0.566$ & $0.633 \pm 0.003$ & $0.592 \pm 0.004$ & $2.300$ \\
C10 Clean & $0.414 \pm 0.009$ & $0.311 \pm 0.007$ & $0.252$ & $0.312 \pm 0.008$ & $0.271 \pm 0.005$ & $0.233$ \\
C10 Random1 & $1.015 \pm 0.012$ & $0.996 \pm 0.005$ & $0.884$ & $0.940 \pm 0.005$ & $0.955 \pm 0.121$ & $2.300$ \\
C10 Random2 & $1.034 \pm 0.007$ & $1.016 \pm 0.006$ & $0.907$ & $0.962 \pm 0.004$ & $0.939 \pm 0.004$ & $2.302$ \\
C10 Random3 & $1.007 \pm 0.006$ & $0.991 \pm 0.009$ & $0.876$ & $0.940 \pm 0.004$ & $0.913 \pm 0.004$ & $2.302$ \\
C10 Worst & $1.512 \pm 0.013$ & $1.498 \pm 0.011$ & $1.414$ & $1.462 \pm 0.005$ & $1.556 \pm 0.300$ & $1.585$ \\
C100-C Clean & $0.907 \pm 0.006$ & $0.715 \pm 0.005$ & $0.608$ & $0.708 \pm 0.010$ & $0.628 \pm 0.004$ & $0.554$ \\
C100-C Noisy & $1.238 \pm 0.013$ & $1.222 \pm 0.013$ & $1.042$ & $1.113 \pm 0.006$ & $1.091 \pm 0.006$ & $1.019$ \\
C100-F Clean & $1.506 \pm 0.019$ & $1.362 \pm 0.016$ & $1.141$ & $1.320 \pm 0.013$ & $1.361 \pm 0.417$ & $1.905$ \\
C100-F Noisy & $2.415 \pm 0.020$ & $2.370 \pm 0.019$ & $2.033$ & $2.163 \pm 0.015$ & $2.449 \pm 0.867$ & $2.744$ \\
\bottomrule
\end{tabular}


==> tables/new_cifar.tex <==
Clean&0.435&0.234&$\bm{0.233}$&9.75&8.30&$\bm{8.24}$\\
Aggre&0.722&0.608&$\bm{0.543}$&19.20&15.88&$\bm{15.74}$\\
Rand1&1.009&0.916&$\bm{0.859}$&28.63&24.80&$\bm{23.50}$\\
Rand2&1.040&0.931&$\bm{0.888}$&29.91&25.44&$\bm{24.12}$\\
Rand3&1.005&0.910&$\bm{0.864}$&28.96&24.86&$\bm{23.44}$\\
Worst&1.511&1.437&$\bm{1.399}$&46.84&44.30&$\bm{42.88}$\\
Clean&1.011&0.669&$\bm{0.606}$&23.12&$\bm{19.36}$&19.52\\
Noisy&1.431&1.234&$\bm{1.150}$&41.42&34.42&$\bm{33.54}$\\
Clean&1.508&1.065&$\bm{1.063}$&33.83&$\bm{29.90}$&29.94\\
Noisy&2.416&2.129&$\bm{1.994}$&58.68&51.34&$\bm{50.26}$\\


==> tables/new_cifar10.tex <==
Clean&0.435&0.234&$\bm{0.233}$&9.75&8.30&$\bm{8.24}$\\
Aggre&0.722&0.608&$\bm{0.543}$&19.20&15.88&$\bm{15.74}$\\
Rand1&1.009&0.916&$\bm{0.859}$&28.63&24.80&$\bm{23.50}$\\
Rand2&1.040&0.931&$\bm{0.888}$&29.91&25.44&$\bm{24.12}$\\
Rand3&1.005&0.910&$\bm{0.864}$&28.96&24.86&$\bm{23.44}$\\
Worst&1.511&1.437&$\bm{1.399}$&46.84&44.30&$\bm{42.88}$\\


==> tables/new_cifar100_coarse.tex <==
Clean&1.011&0.669&$\bm{0.606}$&23.12&$\bm{19.36}$&19.52\\
Noisy&1.431&1.234&$\bm{1.150}$&41.42&34.42&$\bm{33.54}$\\


==> tables/new_cifar100_coarse_elr.tex <==
Clean&1.030&0.644&$\bm{0.605}$&23.07&19.28&$\bm{19.24}$\\
Noisy&1.415&1.228&$\bm{1.152}$&41.55&34.72&$\bm{33.60}$\\


==> tables/new_cifar100_coarse_sc.tex <==
Clean&1.011&0.786&$\bm{0.686}$&23.12&$\bm{21.30}$&21.38\\
Noisy&1.431&1.330&$\bm{1.235}$&41.42&38.08&$\bm{35.87}$\\


==> tables/new_cifar100_coarse_sop.tex <==
Clean&1.018&0.623&$\bm{0.608}$&23.07&$\bm{19.18}$&19.78\\
Noisy&1.427&1.247&$\bm{1.145}$&41.39&34.32&$\bm{33.94}$\\


==> tables/new_cifar100_fine.tex <==
Clean&1.508&1.065&$\bm{1.063}$&33.83&$\bm{29.90}$&29.94\\
Noisy&2.416&2.129&$\bm{1.994}$&58.68&51.34&$\bm{50.26}$\\


==> tables/new_cifar100_fine_elr.tex <==
Clean&1.518&1.070&$\bm{1.068}$&34.05&29.68&$\bm{29.66}$\\
Noisy&2.432&2.130&$\bm{1.997}$&58.85&50.86&$\bm{50.50}$\\


==> tables/new_cifar100_fine_sc.tex <==
Clean&1.508&1.215&$\bm{1.205}$&33.83&$\bm{32.67}$&32.69\\
Noisy&2.416&2.289&$\bm{2.136}$&58.68&54.94&$\bm{53.18}$\\


==> tables/new_cifar100_fine_sop.tex <==
Clean&1.513&1.063&$\bm{1.061}$&33.79&$\bm{29.46}$&29.56\\
Noisy&2.415&2.118&$\bm{1.997}$&58.34&51.06&$\bm{50.54}$\\


==> tables/new_cifar10_elr.tex <==
Clean&0.421&0.233&$\bm{0.232}$&9.53&7.98&$\bm{7.92}$\\
Aggre&0.730&0.606&$\bm{0.541}$&19.02&$\bm{15.34}$&15.52\\
Rand1&1.019&0.921&$\bm{0.864}$&29.42&24.30&$\bm{23.56}$\\
Rand2&1.042&0.941&$\bm{0.893}$&29.79&26.12&$\bm{24.50}$\\
Rand3&1.004&0.912&$\bm{0.866}$&28.80&24.52&$\bm{23.32}$\\
Worst&1.508&1.444&$\bm{1.397}$&46.94&44.64&$\bm{42.48}$\\


==> tables/new_cifar10_sc.tex <==
Clean&0.435&$\bm{0.269}$&0.270&9.75&$\bm{9.09}$&9.10\\
Aggre&0.722&0.663&$\bm{0.585}$&19.20&17.08&$\bm{16.95}$\\
Rand1&1.009&0.968&$\bm{0.907}$&28.63&27.13&$\bm{24.84}$\\
Rand2&1.040&0.983&$\bm{0.935}$&29.91&27.60&$\bm{25.69}$\\
Rand3&1.005&0.963&$\bm{0.911}$&28.96&26.91&$\bm{25.09}$\\
Worst&1.511&1.483&$\bm{1.443}$&46.84&46.12&$\bm{44.14}$\\


==> tables/new_cifar10_sop.tex <==
Clean&0.425&0.236&$\bm{0.235}$&9.65&$\bm{7.96}$&8.00\\
Aggre&0.728&0.634&$\bm{0.541}$&18.03&15.58&$\bm{15.56}$\\
Rand1&1.025&0.925&$\bm{0.851}$&26.91&23.20&$\bm{23.14}$\\
Rand2&1.045&0.957&$\bm{0.883}$&27.39&$\bm{24.12}$&24.16\\
Rand3&1.016&0.921&$\bm{0.851}$&26.66&23.02&$\bm{22.96}$\\
Worst&1.514&1.447&$\bm{1.413}$&46.78&44.50&$\bm{42.78}$\\


==> tables/new_err.tex <==
C10 Clean&$\bm{9.75}$&$\bm{9.09}$&9.10&8.30&$\bm{8.24}$\\
C10 Aggre&$\bm{19.20}$&17.08&$\bm{16.95}$&15.88&$\bm{15.74}$\\
C10 Rand1&$\bm{28.63}$&27.13&$\bm{24.84}$&24.80&$\bm{23.50}$\\
C10 Worst&$\bm{46.84}$&46.12&$\bm{44.14}$&44.30&$\bm{42.88}$\\
C100 Clean&$\bm{33.83}$&$\bm{32.67}$&32.69&$\bm{29.90}$&29.94\\
C100 Noisy&$\bm{58.68}$&54.94&$\bm{53.18}$&51.34&$\bm{50.26}$\\
FMoW&$\bm{43.20}$&42.69&$\bm{39.92}$&37.95&$\bm{34.93}$\\


==> tables/new_fmow_ood.tex <==
FMoW (ID val & test)&1.583&1.627&$\bm{1.554}$&1.494&$\bm{1.305}$&43.20&42.69&$\bm{39.92}$&37.95&$\bm{34.93}$\\
FMoW (OOD val & test)&1.831&1.840&$\bm{1.788}$&1.700&$\bm{1.571}$&49.32&49.70&$\bm{46.75}$&46.74&$\bm{41.56}$\\


==> tables/new_nll.tex <==
C10 Clean&$\bm{0.435}$&$\bm{0.269}$&0.270&0.234&$\bm{0.233}$\\
C10 Aggre&$\bm{0.722}$&0.663&$\bm{0.585}$&0.608&$\bm{0.543}$\\
C10 Rand1&$\bm{1.009}$&0.968&$\bm{0.907}$&0.916&$\bm{0.859}$\\
C10 Worst&$\bm{1.511}$&1.483&$\bm{1.443}$&1.437&$\bm{1.399}$\\
C100 Clean&$\bm{1.508}$&1.215&$\bm{1.205}$&1.065&$\bm{1.063}$\\
C100 Noisy&$\bm{2.416}$&2.289&$\bm{2.136}$&2.129&$\bm{1.994}$\\
FMoW&$\bm{1.583}$&1.627&$\bm{1.554}$&1.494&$\bm{1.305}$\\


==> tables/new_nll_sc.tex <==
C10 Clean&$\bm{0.435}$&$\bm{0.269}$&0.270&0.234&$\bm{0.233}$\\
C10 Aggre&$\bm{0.722}$&0.663&$\bm{0.585}$&0.608&$\bm{0.543}$\\
C10 Rand1&$\bm{1.009}$&0.968&$\bm{0.907}$&0.916&$\bm{0.859}$\\
C10 Worst&$\bm{1.511}$&1.483&$\bm{1.443}$&1.437&$\bm{1.399}$\\
C100 Clean&$\bm{1.508}$&1.215&$\bm{1.205}$&1.065&$\bm{1.063}$\\
C100 Noisy&$\bm{2.416}$&2.289&$\bm{2.136}$&2.129&$\bm{1.994}$\\
FMoW&$\bm{1.583}$&1.627&$\bm{1.554}$&1.494&$\bm{1.305}$\\


==> tables/new_real.tex.tex <==
Yelp&0.908&0.890&$\bm{0.854}$&0.841&$\bm{0.824}$&39.41&38.02&$\bm{37.33}$&36.18&$\bm{36.14}$\\
\midrule
Income&0.393&0.390&$\bm{0.387}$&0.388&$\bm{0.385}$&17.84&17.69&$\bm{17.54}$&17.62&$\bm{17.40}$\\
Cover&0.544&0.540&$\bm{0.539}$&0.538&$\bm{0.538}$&27.52&27.31&$\bm{27.25}$&27.25&$\bm{27.02}$\\
Mobility&0.474&0.472&$\bm{0.471}$&0.471&$\bm{0.468}$&21.43&$\bm{21.38}$&21.42&$\bm{21.17}$&21.24\\
Employ&0.380&0.379&$\bm{0.378}$&0.378&$\bm{0.377}$&17.94&$\bm{17.77}$&17.80&$\bm{17.72}$&17.83\\
Travel&0.597&0.597&$\bm{0.593}$&0.596&$\bm{0.591}$&35.77&35.46&$\bm{35.35}$&35.44&$\bm{35.23}$\\
\midrule
Collab&0.492&0.475&$\bm{0.460}$&0.439&$\bm{0.404}$&20.65&21.58&$\bm{20.27}$&20.40&$\bm{18.80}$\\
Reddit-5k&1.154&1.112&$\bm{1.100}$&1.101&$\bm{1.085}$&47.42&48.35&$\bm{47.04}$&47.09&$\bm{45.49}$\\
Reddit-12k&1.405&1.381&$\bm{1.366}$&1.367&$\bm{1.346}$&51.78&$\bm{51.08}$&51.11&$\bm{50.34}$&51.26\\


==> tables/new_real_collab_reddit.tex <==
Collab&0.492&0.439&$\bm{0.404}$&20.65&20.40&$\bm{18.80}$\\
Reddit5&1.154&1.101&$\bm{1.085}$&47.42&47.09&$\bm{45.49}$\\
Reddit12&1.405&1.367&$\bm{1.346}$&51.78&$\bm{50.34}$&51.26\\


==> tables/new_real_fmow.tex <==
FMoW&1.583&1.494&$\bm{1.305}$&43.20&37.95&$\bm{34.93}$\\


==> tables/new_real_folktables.tex <==
Income&0.393&0.388&$\bm{0.385}$&17.84&17.62&$\bm{17.40}$\\
Cover&0.544&0.538&$\bm{0.538}$&27.52&27.25&$\bm{27.02}$\\
Mobility&0.474&0.471&$\bm{0.468}$&21.43&$\bm{21.17}$&21.24\\
Employ&0.380&0.378&$\bm{0.377}$&17.94&$\bm{17.72}$&17.83\\
Travel&0.597&0.596&$\bm{0.591}$&35.77&35.44&$\bm{35.23}$\\


==> tables/new_real_yelp.tex <==
Yelp&0.908&0.841&$\bm{0.824}$&39.41&36.18&$\bm{36.14}$\\


==> tables/new_sc.tex <==
C10 Clean&0.435&$\bm{0.269}$&0.270&9.75&$\bm{9.09}$&9.10\\
C10 Aggre&0.722&0.663&$\bm{0.585}$&19.20&17.08&$\bm{16.95}$\\
C10 Rand1&1.009&0.968&$\bm{0.907}$&28.63&27.13&$\bm{24.84}$\\
C10 Worst&1.511&1.483&$\bm{1.443}$&46.84&46.12&$\bm{44.14}$\\
C100 Clean&1.508&1.215&$\bm{1.205}$&33.83&$\bm{32.67}$&32.69\\
C100 Noisy&2.416&2.289&$\bm{2.136}$&58.68&54.94&$\bm{53.18}$\\
FMoW&1.583&1.627&$\bm{1.554}$&43.20&42.69&$\bm{39.92}$\\


==> tables/new_scec.tex <==
C10 Clean&0.435&0.234&$\bm{0.233}$&9.75&8.30&$\bm{8.24}$\\
C10 Aggre&0.722&0.608&$\bm{0.543}$&19.20&15.88&$\bm{15.74}$\\
C10 Rand1&1.009&0.916&$\bm{0.859}$&28.63&24.80&$\bm{23.50}$\\
C10 Worst&1.511&1.437&$\bm{1.399}$&46.84&44.30&$\bm{42.88}$\\
C100 Clean&1.508&1.065&$\bm{1.063}$&33.83&$\bm{29.90}$&29.94\\
C100 Noisy&2.416&2.129&$\bm{1.994}$&58.68&51.34&$\bm{50.26}$\\
FMoW&1.583&1.494&$\bm{1.305}$&43.20&37.95&$\bm{34.93}$\\


==> tables/noise_bench/datasets.tex <==
\begin{tabular}{llS[table-format=5]S[table-format=5]S[table-format=5]S[table-format=3]rc}
\toprule
Modality & Dataset & {Train Size} & {Val Size} & {Test Size} & {Classes} & Input Size & Units\\
\midrule
\multirow{4}{*}{Vision} & CIFAR-10 & 40000 & 5000 & 5000 & 10 & \numproduct{3x32x32} & \multirow{4}{*}{C $\times$ W $\times$ H}\\
 & CIFAR-100-N Coarse & 40000 & 5000 & 5000 & 20 & \numproduct{3x32x32} & \\
 & CIFAR-100-N Fine & 40000 & 5000 & 5000 & 100 & \numproduct{3x32x32} & \\
 & FMoW & 76863 & 11483 & 11327 & 62 & \numproduct{3x224x224} & \\
\midrule
\multirow{3}{*}{Graph} & Collab & 4000 & 500 & 500 & 3 & \num{74.49} / \num{2457.78} & \multirow{3}{*}{\makecell{nodes / edges \\ (avg.)}}\\
 & Reddit-5k & 4001 & 499 & 499 & 5 & \num{508.52} / \num{594.87} & \\
 & Reddit-12k & 9545 & 1192 & 1192 & 11 & \num{391.41} / \num{456.89} & \\
\midrule
\multirow{5}{*}{Tabular} & Income & 156533 & 19566 & 19566 & 2 & \num{816} & \multirow{5}{*}{features}\\
 & Public Coverage & 110844 & 13855 & 13855 & 2 & \num{88} & \\
 & Mobility & 64265 & 8032 & 8032 & 2 & \num{101} & \\
 & Employment & 303055 & 37881 & 37881 & 2 & \num{98} & \\
 & Travel Time & 138008 & 17250 & 17250 & 2 & \num{615} & \\
\bottomrule
\end{tabular}

==> tables/noise_bench/training_setup.tex <==
\begin{tabular}{ll}
\toprule
Dataset & CIFAR-10/100-N \\
\midrule
Model & ResNet-18-D \\
Pre-trained & True \\
Optimizer & \makecell[tl]{SGD\\(momentum=0.9)} \\
LR & 0.1 \\
Weight Decay & 5e-4 \\
Scheduler & CosineAnnealing \\
Epochs & 100 \\
Batch Size & 500 \\
Augmentation & \makecell[tl]{RandomCrop\\+ HorizontalFlip} \\
\bottomrule
\end{tabular}


==> tables/old_main.tex <==
\begin{tabular}{lllllllllllllllllllll}
\toprule
 & \multicolumn{10}{r}{Best Loss} & \multicolumn{10}{r}{Best Error} \\
 & \multicolumn{2}{r}{Epoch} & \multicolumn{2}{r}{Base Loss} & \multicolumn{2}{r}{Final Loss} & \multicolumn{2}{r}{Base Error} & \multicolumn{2}{r}{Final Error} & \multicolumn{2}{r}{Epoch} & \multicolumn{2}{r}{Base Loss} & \multicolumn{2}{r}{Final Loss} & \multicolumn{2}{r}{Base Error} & \multicolumn{2}{r}{Final Error} \\
 & Naive & Post-hoc & Naive & Post-hoc & Naive & Post-hoc & Naive & Post-hoc & Naive & Post-hoc & Naive & Post-hoc & Naive & Post-hoc & Naive & Post-hoc & Naive & Post-hoc & Naive & Post-hoc \\
\midrule
C-10-N Clean & $72_{\pm 35}$ & $101$ & $0.414_{\pm 0.009}$ & $0.423_{\pm 0.014}$ & $0.235$ & $0.229$ & $10.74_{\pm 1.93}$ & $9.51_{\pm 0.24}$ & $7.68$ & $7.56$ & $95_{\pm 4}$ & $100$ & $0.420_{\pm 0.013}$ & $0.422_{\pm 0.015}$ & $0.229$ & $0.229$ & $9.38_{\pm 0.24}$ & $9.53_{\pm 0.27}$ & $7.58$ & $7.56$ \\
C-10-N Aggregate & $11_{\pm 2}$ & $49$ & $0.713_{\pm 0.012}$ & $0.971_{\pm 0.029}$ & $0.589$ & $0.540$ & $21.66_{\pm 0.44}$ & $23.39_{\pm 0.53}$ & $18.00$ & $15.80$ & $93_{\pm 5}$ & $75$ & $1.098_{\pm 0.018}$ & $1.083_{\pm 0.017}$ & $0.549$ & $0.544$ & $19.01_{\pm 0.32}$ & $20.02_{\pm 0.25}$ & $15.58$ & $15.56$ \\
C-10-N Random1 & $12_{\pm 3}$ & $36$ & $1.016_{\pm 0.009}$ & $1.244_{\pm 0.021}$ & $0.890$ & $0.860$ & $28.84_{\pm 0.55}$ & $32.30_{\pm 1.04}$ & $25.06$ & $23.60$ & $34_{\pm 37}$ & $45$ & $1.218_{\pm 0.373}$ & $1.376_{\pm 0.050}$ & $0.867$ & $0.862$ & $28.54_{\pm 0.22}$ & $32.98_{\pm 1.48}$ & $23.92$ & $23.46$ \\
C-10-N Random2 & $10_{\pm 3}$ & $33$ & $1.030_{\pm 0.010}$ & $1.245_{\pm 0.038}$ & $0.921$ & $0.888$ & $29.40_{\pm 0.62}$ & $32.36_{\pm 1.29}$ & $26.16$ & $24.30$ & $24_{\pm 31}$ & $51$ & $1.149_{\pm 0.308}$ & $1.512_{\pm 0.017}$ & $0.904$ & $0.897$ & $29.22_{\pm 0.29}$ & $33.72_{\pm 0.61}$ & $25.26$ & $23.88$ \\
C-10-N Random3 & $9_{\pm 1}$ & $30$ & $1.007_{\pm 0.010}$ & $1.178_{\pm 0.028}$ & $0.899$ & $0.863$ & $29.18_{\pm 0.42}$ & $31.68_{\pm 0.86}$ & $25.96$ & $23.76$ & $25_{\pm 27}$ & $60$ & $1.127_{\pm 0.279}$ & $1.625_{\pm 0.035}$ & $0.871$ & $0.877$ & $28.70_{\pm 0.18}$ & $32.43_{\pm 0.71}$ & $24.40$ & $23.30$ \\
C-10-N Worst & $9_{\pm 2}$ & $27$ & $1.508_{\pm 0.007}$ & $1.678_{\pm 0.018}$ & $1.425$ & $1.398$ & $46.97_{\pm 0.55}$ & $50.44_{\pm 1.29}$ & $44.04$ & $43.16$ & $11_{\pm 3}$ & $34$ & $1.514_{\pm 0.012}$ & $1.809_{\pm 0.036}$ & $1.415$ & $1.400$ & $46.70_{\pm 0.25}$ & $51.22_{\pm 0.52}$ & $43.62$ & $42.88$ \\
C-100-N-Coarse Clean & $35_{\pm 39}$ & $97$ & $1.015_{\pm 0.018}$ & $1.030_{\pm 0.019}$ & $0.656$ & $0.605$ & $28.02_{\pm 3.55}$ & $22.99_{\pm 0.32}$ & $21.44$ & $19.24$ & $94_{\pm 5}$ & $97$ & $1.023_{\pm 0.016}$ & $1.030_{\pm 0.019}$ & $0.605$ & $0.605$ & $22.76_{\pm 0.29}$ & $22.99_{\pm 0.32}$ & $19.32$ & $19.24$ \\
C-100-N-Coarse Noisy & $8_{\pm 1}$ & $37$ & $1.422_{\pm 0.007}$ & $1.857_{\pm 0.091}$ & $1.220$ & $1.152$ & $42.05_{\pm 0.57}$ & $45.86_{\pm 1.97}$ & $36.66$ & $33.58$ & $71_{\pm 38}$ & $35$ & $2.006_{\pm 0.356}$ & $1.837_{\pm 0.028}$ & $1.158$ & $1.152$ & $40.90_{\pm 0.56}$ & $46.34_{\pm 0.80}$ & $33.82$ & $33.54$ \\
C-100-N-Fine Clean & $96_{\pm 4}$ & $68$ & $1.501_{\pm 0.022}$ & $1.603_{\pm 0.025}$ & $1.055$ & $1.052$ & $33.79_{\pm 0.60}$ & $35.33_{\pm 0.38}$ & $29.26$ & $29.58$ & $88_{\pm 7}$ & $100$ & $1.510_{\pm 0.027}$ & $1.513_{\pm 0.021}$ & $1.053$ & $1.055$ & $33.61_{\pm 0.53}$ & $34.04_{\pm 0.48}$ & $29.38$ & $29.26$ \\
C-100-N-Fine Noisy & $8_{\pm 2}$ & $28$ & $2.419_{\pm 0.027}$ & $2.993_{\pm 0.044}$ & $2.083$ & $2.002$ & $59.54_{\pm 1.09}$ & $62.96_{\pm 0.83}$ & $52.96$ & $50.36$ & $81_{\pm 30}$ & $31$ & $3.095_{\pm 0.286}$ & $3.111_{\pm 0.085}$ & $2.059$ & $2.004$ & $58.60_{\pm 0.42}$ & $63.27_{\pm 1.00}$ & $50.62$ & $50.26$ \\
Income  & $6_{\pm 1}$ & $10$ & $0.393_{\pm 0.001}$ & $0.409_{\pm 0.004}$ & $0.386$ & $0.385$ & $17.85_{\pm 0.10}$ & $17.97_{\pm 0.15}$ & $17.70$ & $17.50$ & $7_{\pm 2}$ & $17$ & $0.396_{\pm 0.004}$ & $0.510_{\pm 0.012}$ & $0.385$ & $0.389$ & $17.77_{\pm 0.07}$ & $18.95_{\pm 0.23}$ & $17.72$ & $17.32$ \\
Public Coverage  & $8_{\pm 2}$ & $13$ & $0.543_{\pm 0.001}$ & $0.548_{\pm 0.003}$ & $0.538$ & $0.538$ & $27.42_{\pm 0.20}$ & $27.56_{\pm 0.13}$ & $27.21$ & $27.01$ & $10_{\pm 4}$ & $26$ & $0.545_{\pm 0.002}$ & $0.577_{\pm 0.006}$ & $0.538$ & $0.541$ & $27.27_{\pm 0.10}$ & $28.19_{\pm 0.23}$ & $27.04$ & $26.86$ \\
Mobility  & $9_{\pm 2}$ & $17$ & $0.472_{\pm 0.001}$ & $0.482_{\pm 0.004}$ & $0.469$ & $0.468$ & $21.49_{\pm 0.15}$ & $21.49_{\pm 0.17}$ & $21.25$ & $21.07$ & $13_{\pm 4}$ & $45$ & $0.478_{\pm 0.006}$ & $0.684_{\pm 0.015}$ & $0.468$ & $0.485$ & $21.21_{\pm 0.08}$ & $23.42_{\pm 0.56}$ & $21.19$ & $21.03$ \\
Employment  & $8_{\pm 2}$ & $12$ & $0.380_{\pm 0.000}$ & $0.382_{\pm 0.001}$ & $0.377$ & $0.377$ & $17.89_{\pm 0.10}$ & $17.92_{\pm 0.07}$ & $17.78$ & $17.69$ & $9_{\pm 4}$ & $17$ & $0.381_{\pm 0.001}$ & $0.384_{\pm 0.001}$ & $0.377$ & $0.377$ & $17.78_{\pm 0.05}$ & $18.02_{\pm 0.08}$ & $17.74$ & $17.65$ \\
Travel Time  & $8_{\pm 1}$ & $15$ & $0.597_{\pm 0.001}$ & $0.626_{\pm 0.004}$ & $0.593$ & $0.591$ & $35.56_{\pm 0.20}$ & $36.10_{\pm 0.27}$ & $35.19$ & $35.13$ & $10_{\pm 2}$ & $22$ & $0.603_{\pm 0.007}$ & $0.698_{\pm 0.011}$ & $0.592$ & $0.592$ & $35.42_{\pm 0.20}$ & $37.12_{\pm 0.21}$ & $35.28$ & $35.03$ \\
Collab  & $36_{\pm 6}$ & $132$ & $0.466_{\pm 0.015}$ & $0.883_{\pm 0.101}$ & $0.470$ & $0.405$ & $20.78_{\pm 1.02}$ & $20.10_{\pm 1.59}$ & $22.00$ & $19.60$ & $108_{\pm 71}$ & $258$ & $0.722_{\pm 0.272}$ & $1.568_{\pm 0.137}$ & $0.408$ & $0.415$ & $17.93_{\pm 1.10}$ & $20.90_{\pm 1.31}$ & $19.60$ & $17.60$ \\
Reddit-5k  & $13_{\pm 3}$ & $53$ & $1.099_{\pm 0.010}$ & $1.585_{\pm 0.084}$ & $1.101$ & $1.080$ & $47.04_{\pm 1.28}$ & $51.30_{\pm 1.45}$ & $46.49$ & $45.69$ & $17_{\pm 7}$ & $30$ & $1.124_{\pm 0.026}$ & $1.206_{\pm 0.034}$ & $1.099$ & $1.087$ & $45.47_{\pm 0.75}$ & $49.25_{\pm 1.80}$ & $46.09$ & $45.09$ \\
Reddit-12k  & $13_{\pm 3}$ & $40$ & $1.394_{\pm 0.009}$ & $1.582_{\pm 0.031}$ & $1.366$ & $1.339$ & $51.21_{\pm 0.64}$ & $54.14_{\pm 1.30}$ & $50.34$ & $50.42$ & $18_{\pm 6}$ & $18$ & $1.419_{\pm 0.023}$ & $1.423_{\pm 0.024}$ & $1.356$ & $1.355$ & $50.41_{\pm 0.50}$ & $51.95_{\pm 1.47}$ & $49.92$ & $49.58$ \\
\bottomrule
\end{tabular}


==> tables/prelim.tex <==
\multirow{3}{*}{Clean (0)}&TS&$\bm{0.114}$&0.117&$\bm{0.00}$&$\bm{0.00}$\\
&SWA&$\bm{0.106}$&0.126&0.66&$\bm{0.65}$\\
&Ens&$\bm{0.129}$&0.174&1.79&$\bm{1.77}$\\
\midrule
\multirow{3}{*}{Aggre (9)}&TS&$\bm{0.010}$&0.035&$\bm{0.00}$&$\bm{0.00}$\\
&SWA&$\bm{0.055}$&0.095&$\bm{2.13}$&2.26\\
&Ens&$\bm{0.146}$&0.154&2.45&$\bm{2.28}$\\
\midrule
\multirow{3}{*}{Rand1 (17)}&TS&0.006&$\bm{0.004}$&$\bm{0.00}$&$\bm{0.00}$\\
&SWA&$\bm{0.038}$&0.075&$\bm{1.50}$&3.79\\
&Ens&$\bm{0.118}$&0.122&4.51&$\bm{4.01}$\\
\midrule
\multirow{3}{*}{Worst (40)}&TS&$\bm{0.006}$&0.009&$\bm{0.00}$&$\bm{0.00}$\\
&SWA&$\bm{0.028}$&0.058&$\bm{0.72}$&2.70\\
&Ens&$\bm{0.089}$&0.094&$\bm{3.06}$&3.51\\


==> tables/prelim_cifar10.tex <==
\multirow{3}{*}{Clean (0)}&TS&0.114&$\bm{0.117}$&$\bm{0.00}$&$\bm{0.00}$\\
&SWA&0.106&$\bm{0.126}$&$\bm{0.66}$&0.65\\
&Ens&0.129&$\bm{0.174}$&$\bm{1.79}$&1.77\\
\midrule
\multirow{3}{*}{Aggre (9)}&TS&0.010&$\bm{0.035}$&$\bm{0.00}$&$\bm{0.00}$\\
&SWA&0.055&$\bm{0.095}$&2.13&$\bm{2.26}$\\
&Ens&0.146&$\bm{0.154}$&$\bm{2.45}$&2.28\\
\midrule
\multirow{3}{*}{Rand1 (17)}&TS&$\bm{0.006}$&0.004&$\bm{0.00}$&$\bm{0.00}$\\
&SWA&0.038&$\bm{0.075}$&1.50&$\bm{3.79}$\\
&Ens&0.118&$\bm{0.122}$&$\bm{4.51}$&4.01\\
\midrule
\multirow{3}{*}{Worst (40)}&TS&0.006&$\bm{0.009}$&$\bm{0.00}$&$\bm{0.00}$\\
&SWA&0.028&$\bm{0.058}$&0.72&$\bm{2.70}$\\
&Ens&0.089&$\bm{0.094}$&3.06&$\bm{3.51}$\\


==> tables/prelim_cifar100.tex <==
\multirow{3}{*}{Clean (0)}&TS&0.155&$\bm{0.157}$&$\bm{0.00}$&$\bm{0.00}$\\
&SWA&-0.017&$\bm{0.188}$&$\bm{1.16}$&1.13\\
&Ens&0.323&$\bm{0.375}$&$\bm{4.41}$&$\bm{4.41}$\\
\midrule
\multirow{3}{*}{Noisy (40)}&TS&0.006&$\bm{0.012}$&$\bm{0.00}$&$\bm{0.00}$\\
&SWA&0.132&$\bm{0.244}$&3.74&$\bm{5.49}$\\
&Ens&0.353&$\bm{0.386}$&5.80&$\bm{7.74}$\\


==> tables/test.tex <==
\begin{tabular}{llllllll}
\toprule
 & Raw & Cal & WA & WA+Cal & Ens & Ens+Cal & WA+Cal+Ens \\
\midrule
C10 Aggregate & $0.711 \pm 0.019$ & $0.680 \pm 0.006$ & $0.633 \pm 0.003$ & $0.592 \pm 0.004$ & $0.566$ & $0.559$ & $2.300$ \\
C10 Clean & $0.414 \pm 0.009$ & $0.311 \pm 0.007$ & $0.312 \pm 0.008$ & $0.271 \pm 0.005$ & $0.252$ & $0.240$ & $0.233$ \\
C10 Random1 & $1.015 \pm 0.012$ & $0.996 \pm 0.005$ & $0.940 \pm 0.005$ & $0.955 \pm 0.121$ & $0.884$ & $2.252$ & $2.300$ \\
C10 Random2 & $1.034 \pm 0.007$ & $1.016 \pm 0.006$ & $0.962 \pm 0.004$ & $0.939 \pm 0.004$ & $0.907$ & $2.275$ & $2.302$ \\
C10 Random3 & $1.007 \pm 0.006$ & $0.991 \pm 0.009$ & $0.940 \pm 0.004$ & $0.913 \pm 0.004$ & $0.876$ & $0.873$ & $2.302$ \\
C10 Worst & $1.512 \pm 0.013$ & $1.498 \pm 0.011$ & $1.462 \pm 0.005$ & $1.556 \pm 0.300$ & $1.414$ & $1.414$ & $1.585$ \\
C100-C Clean & $0.907 \pm 0.006$ & $0.715 \pm 0.005$ & $0.708 \pm 0.010$ & $0.628 \pm 0.004$ & $0.608$ & $0.585$ & $0.554$ \\
C100-C Noisy & $1.238 \pm 0.013$ & $1.222 \pm 0.013$ & $1.113 \pm 0.006$ & $1.091 \pm 0.006$ & $1.042$ & $1.044$ & $1.019$ \\
C100-F Clean & $1.506 \pm 0.019$ & $1.362 \pm 0.016$ & $1.320 \pm 0.013$ & $1.361 \pm 0.417$ & $1.141$ & $1.123$ & $1.905$ \\
C100-F Noisy & $2.415 \pm 0.020$ & $2.370 \pm 0.019$ & $2.163 \pm 0.015$ & $2.449 \pm 0.867$ & $2.033$ & $2.040$ & $2.744$ \\
\bottomrule
\end{tabular}


==> tables/training_setup.tex <==
\begin{tabular}{ll}
\toprule
Dataset & CIFAR-10/100-N \\
\midrule
Model & ResNet-18-D \\
Pre-trained & True \\
Optimizer & \makecell[tl]{SGD\\(momentum=0.9)} \\
LR & 0.1 \\
Weight Decay & 5e-4 \\
Scheduler & CosineAnnealing \\
Epochs & 100 \\
Batch Size & 500 \\
Augmentation & \makecell[tl]{RandomCrop\\+ HorizontalFlip} \\
\bottomrule
\end{tabular}

